First-order Temporal Logic on Finite Traces: Semantic Properties, Decidable Fragments, and Applications

Formalisms based on temporal logics interpreted over finite strict linear orders, known in the literature as finite traces, have been used for temporal specification in automated planning, process modelling, (runtime) verification and synthesis of programs, as well as in knowledge representation and reasoning. In this paper, we focus on first-order temporal logic on finite traces. We first investigate preservation of equivalences and satisfiability of formulas between finite and infinite traces, by providing a set of semantic and syntactic conditions to guarantee when the distinction between reasoning in the two cases can be blurred. Moreover, we show that the satisfiability problem on finite traces for several decidable fragments of first-order temporal logic is ExpSpace-complete, as in the infinite trace case, while it decreases to NExpTime when finite traces bounded in the number of instants are considered. This leads also to new complexity results for temporal description logics over finite traces. Finally, we investigate applications to planning and verification, in particular by establishing connections with the notions of insensitivity to infiniteness and safety from the literature.

==> 10-proofs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage
\appendix

 

  
\section{Proofs for Section~\ref{sec:tdlf-to-tdl}}
\label{sec:appA}
%\nb{M: Change title to `Section $n$'? (cf. Appendix C)}

%\subsection{$\TALCf$ is in \ExpSpace}

\LemmaModels*
\begin{proof}
%(Sketch)
%\nb{M: Removed `Sketch'} O: Ok thanks
$\psi_{f}$ is satisfied in $\Imf$
iff there is 
  $k>0$ such that, for all $d\in\Delta$, it holds that: 
$d\not\in E^{\Imc_{j}}$, for all $j \in[0, k)$; and
$d\in E^{\Imc_{i}}$, for all $i \in[k, \infty)$.
That is,
$\Imf = \FEImf'$,
%$\Imf = \FImf'$,
for some finite trace $\Fmf$ and some infinite trace $\Imf'$.
 \end{proof}



%~ \begin{proof}
%~ ($\Rightarrow$) Let $\Imf$ be s.t. $\Imf,0 \mdl \psi_{f}$. Then $E^{\I_{0}} = \eset$, and for every $n > 0$ we have that: $\Imf,n \models E \sqsubseteq \Next E$, and there is a $k > 0$ s.t. $\Imf,{k} \mdl \top \sqs E$, i.e.,$E^{\I_{k}} = \Delta^{\Imf}$. Moreover, for all $n$, $0 < n < k$, $\Imf,n \mdl \top \sqs \lnot E$, i.e., $E^{\I_{n}} = \eset$.  Finally, since $E^{\I_{k}} = \Delta^{\Imf}$ and $E^{\I_{n}} \sbs E^{\I_{n+1}}$ for all $n > 0$, we have $E^{\I_{n}} = \Delta^{\Imf}$ for all $n \geq k$. It is immediate to find a finite trace $\Fmf = (\Delta, (\Fmc_{n})_{n \in [0, k - 1]})$ and an infinite trace $\Imf' = (\Delta, (\Imc'_{n})_{n \in [0,\infty)})$ s.t. $\Imf$ is of the form $\FImf'$.
  
%~ ($\Leftarrow$) Let $\Imf$ be an infinite trace of the form $\FImf'$, for some finite trace $\Fmf= (\Delta, (\Fmc_n)_{n \in [0, l]})$ and some infinite trace $\Imf' = (\Delta, (\Imc'_n)_{n \in [0, \infty)})$ . By definition:
%~ \[
%~ E^{\I_{n}} =
	%~ \begin{cases}
		%~ \emptyset, & \text{for all $n \in [0, l]$} \\
		%~ \Delta, & \text{for all $n \in [l + 1, \infty)$}
	%~ \end{cases} \\
%~ \]
%~ Clearly, $\Imf,0 \mdl \B (E \sqsubseteq \Next E)$, since: for every
%~ $n$, $0 \leq n \leq l$, $\eset = E^{\I_{n}} \sbs E^{\I_{n+1}}$; while
%~ for every $n > l$,
%~ $\Delta^{\Imf} = E^{\I_{n}} \sbs E^{\I_{n+1}} = \Delta^{\Imf}$. By definition, we also have that $\Imf, 0 \mdl \top \sqs \lnot E$. Moreover, $\Imf, l + 1 \mdl \top \sqs E$, and
%~ thanks to the fact that $E^{\I_{n}} = \eset$, for all $n$,
%~ $0 \leq n \leq l$, the following holds as well:
%~ $\Imf,n \mdl \top \sqs \lnot E$. 
%~ Therefore, we can conclude that
%~ $\Imf,0 \mdl (\top \sqs \lnot E) \Until (\top \sqs E)$, and thus $\Imf,0 \mdl \psi_{f}$.
%~ \end{proof}

%\nb{O: I removed the proof of lemma 1 because I think 
%it is a very straightforward lemma. \\ M: But in \cite{DegEtAl} 
%they give a sketch of a similar proof, and in our Section 5.2 we prove the analogous Lemma. 
%I would keep it, even if in a very short form, for ``symmetry'' reasons}
%\nb{O:  I added a  sketch. More than that I would find strange in a paper}
%\nb{M: Great, thanks!}

\LemmaTranslation*
\begin{proof}
%\nb{M: Changed, check} O: I did. Thanks!
Let
$\Fmf = (\Delta^\Fmf, (\Fmc_n)_{n \in [0, l]})$
be a finite trace
%with length $k$
and let
%\Imf be an infinite trace
$\FEImf = (\Delta^{\FImf}, (\FImc_n)_{n \in [0, \infty)})$
be an end extension of $\Fmf$. 
%We show that
%%$\Fmf,0 \mdl \p$ iff $\FImf,0 \mdl \p\tr$.
%$\Fmf \mdl \p$ iff $\FImf \mdl \p\tr$.
%
%Firstly, we prove, by induction on concepts $C$ occurring in $\p$, that for all $n \in [0, k - 1]$,
%and for all $d \in \Delta$:
%\[
%d \in C^{\F_{n}} \text{ if and only if } d \in (C\tr)^{\FImc_{n}}. \label{eq:conc} \tag{$\ast$}
%\]
%For the base case $C = A \in \NC$, this is an immediate consequence of the definitions of $\FImf$ and $\cdot\tr$. 
%Assume the lemma holds for $C_1$ and $C_2$. 
%The inductive cases for boolean operators on concepts, $C = \lnot C_{1}$ 
%and $C = (C_{1} \sqcap C_{2})$, are straightforward. 
%We are  left with the cases below.
%
%\noindent
%\newline 
%$C = \exists R.C_{1}$. We have that  
%$d \in (\exists R.C_{1})^{\Fmc_{n}}$ iff there is $d' \in C_{1}^{\Fmc_{n}}$ 
%such that $(d,d')\in R^{\Fmc_{n}}$. By i.h. and definition of $\FImf$ this happens 
%iff  $d' \in (C_{1}\tr)^{\FImc_{n}}$ and $(d,d')\in R^{\FImc_{n}}$, which 
%means that $d \in (\exists R.(C_{1}\tr))^{\FImc_{n}}$. 
%By definition of $\cdot\tr$, $d \in ((\exists R.C_{1})\tr)^{\FImc_{n}}$.
%
%\noindent
%\newline
%$C = C_{1} \Until C_{2}$. 
%We have that  
%$d \in (C_{1} \Until C_{2})^{\F_{n}}$ iff, for some $m \in (n,k -1]$, 
%  $d \in C_{2}^{\F_{m}}$ and, for all $i \in (n,m)$, 
%  $d \in C_{1}^{\F_{i}}$. By i.h. and definition of $\FImf$ this happens 
%iff  $d \in (C_{2}\tr)^{\FImc_{m}}$ and, for all $i \in (n,m)$, 
%  $d \in (C_{1}\tr)^{\FImc_{i}}$. 
%%$a \in \{ d \in \Delta \mid \exists h \in (i, k) \colon d \in C_{2}^{\FImc_{h}} 
%%\land \forall j \in (i,h) \colon d \in C_{1}^{\FImc_{j}} \}$. 
%Since $E^{\FImc_{n}} = \eset$ iff $n \in [0, k - 1]$,    %this is equivalent to: 
%%$a \in \{ d \in \Delta \mid \exists h \in (i, \infty) \colon d \in 
%%(C_{2}\tr)^{\FImc_{h}} \cap (\lnot E)^{\FImc_{h}} \land \forall j \in (i,h) \colon d \in C_{1}^{\FImc_{j}} \}$ iff 
%$d \in (C_{1}\tr \Until (C_{2}\tr \sqcap \lnot E))^{\FImc_{n}}$. By definition of $\cdot\tr$,  
% $d \in ((C_{1} \Until C_{2})\tr)^{\FImc_{n}}$.\\
%
Firstly, we prove, by induction on subformulas $\psi$ of $\p$, that for all $n \in [0, l]$
and all assignments
%\nb{M: Changed to `all'}
$\assign$:
\[
\Fmf,n \mdl^{\assign} \psi \text{ iff } \FEImf,n \mdl^{\assign} \psi\tr.
\]
If $\psi = P(\bar{\tau})$, the statement follows immediately from the definition of $\FEImf$ and $\cdot\tr$.
%If $\psi = A(a)$ or $\psi = R(a,b)$, with $A \in \NC$ and $R \in \NR$, the statements 
%follow immediately from the definitions of $\FImf$ and $\cdot\tr$. If $\psi = C_{1} \sqs C_{2}$, 
%we apply what has already been shown above.
%
The proof of the inductive cases $\psi = \lnot \chi$, $\psi = (\chi \land \zeta)$, and $\psi = \exists x \chi$ is straightforward. The remaining case is proved as follows.

\noindent
\newline 
$\psi = (\chi \Until \zeta)$.
We have that  
$\Fmf, n \mdl^{\assign} \chi \Until \zeta$
iff there is $m \in (n, l]$ such that
$\Fmf, m \models^{\assign} \zeta$
and for all
$i \in (n,m)$, $\Fmf,i \models^{\assign} \chi$. 
By i.h. and definition of $\FEImf$ this happens iff there is
$m \in (n, l]$ s.t. $\FEImf, m \models^{\assign} \zeta\tr$
and for all
$i \in (n,m)$, $\FEImf,i \models^{\assign} \chi\tr$.
Since
$E^{\FEImc_{j}} = \eset$ for all $j \in [0, l]$,   
this means that
$\FEImf, n \mdl^{\assign} \chi\tr \Until (\zeta\tr \land \forall x \lnot E(x))$.
That is, 
$\FEImf, n \mdl^{\assign} (\chi \Until \zeta)\tr$ 
(recall that $\forall x \lnot E(x)=\psi_{f_1}$).
%\nb{O: added}

%$\Fmf, n \mdl^{\assign} (\psi_{1} \Until \psi_{2})$ iff 
%there is $m \in (n, k - 1]$ s.t. 
%$\Fmf,m \models \psi_{2} \text{ and for all } i \in (n,m)$, $\Fmf,i \models \psi_{1}$. 
%By i.h. and definition of $\FImf$ this happens
% iff  there is
%$m \in (n, k -1]$ s.t. $\FImf,m \models \psi_{2}\tr \text{ and for all } 
%  i \in (n,m)$, $\FImf,i \models \psi_{1}\tr$. Since $E^{\FImc_{n}} = \eset$ iff $n \in [0, k -1]$,   
%  %the previous step is equivalent to:
%%$\exists h \in (i, \infty) \colon \FImf,h \models \psi_{2}\tr \text{ and } \FImf,h \mdl \lnot (\top \sqs E), \text{ and } \forall j \in (i,h) \colon \FImf,j \models \psi_{1}\tr$, that is:
%%$\exists h \in (i, \infty) \colon \FImf,h \models \psi_{2}\tr \land \lnot (\top \sqs E), \text{ and } \forall j \in (i,h) \colon \FImf,j \models \psi_{1}\tr$.
%this means that,
%$\FImf,n \mdl \psi_{1}\tr \Until (\psi_{2}\tr \land \lnot (\top
%\sqs E))$ iff
%$\FImf,n \mdl (\psi_{1} \Until \psi_{2})\tr$.

\noindent
\newline 
Thus, in particular, we have:
$\Fmf \mdl \p$ iff $\FEImf \mdl \p\tr$.
%\nb{O: added $E$}
%
%\medskip
%\medskip
%($\Leftarrow$) Conversely, suppose that for all extensions $\FImf$ of $\Fmf$, $\p\tr$ 
%is satisfiable on $\FImf$. The proof that $\Fmf,0 \mdl \p$ follows in a way analogous 
%to the ($\Rightarrow$) direction.
\end{proof}



\TheorFiniteChar*
\begin{proof} 
If
%\nb{O: Changed, end extension}
$\p$ is satisfied in some finite trace $\Fmf$, then (by Lemmas~\ref{lemma:finchar} 
and \ref{lemma:finextchar}) any end extension $\FEImf$ satisfies $\p\tr \land \psif$. Conversely, 
suppose that $\p\tr \land \psif$ is satisfied in some infinite trace $\Imf$. By Lemma~\ref{lemma:finchar}, 
%\nb{M: Changes using $\Imf = \FImf'$} O: thanks!
$\Imf = \FEImf'$, for some finite trace $\Fmf$ and some infinite trace $\Imf'$. 
Since $\FEImf' \mdl \p\tr$, by Lemma~\ref{lemma:finextchar}, we have that  $\Fmf \mdl \p$.
\end{proof}


%\input{4-hardness}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Proofs for   `Traces with at Most $k$ Time Points'}
%\label{sec:appB}
\input{5-fixed-fo}

\TheorTALCkBounded*
\begin{proof}
By Lemma~\ref{lem:qm}  
there is a model with at most $k$ time points 
iff there is a quasimodel  for $\varphi$   with a sequence of quasistates  (for $\varphi$) of length at most $k$. 
This means that   runs   have size at most $k$. Since each   run   
is a sequence of   types, the number of possible   runs   is 
bounded by $|\types{\varphi}|^k$. The correspondence between models and quasimodels 
(Lemma~\ref{lem:qm}) maps each   run  to 
a domain element. Thus, there is a model with domain size bounded by $|\types{\varphi}|^k$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proofs for Section~\ref{sec:dist}}
\label{sec:appC}

%\LemmaNot*
\begin{restatable}{lemma}{LemmaNot}\label{lemma:not}
  Let $\p$ be a $\QTLfr{}{}{}$ formula, and
  $Q, Q' \in \{ \exists, \forall \}$, with $Q \neq Q'$.  Then, $\p$ is
  $\finit{\Rightarrow}{Q}$ iff $\lnot \p$ is $\finit{\Leftarrow}{Q'}$.
%  and
%  \nb{A: why needed?}
%  $\lnot \p$ is $\finit{\Rightarrow}{Q}$ iff $\p$ is
%  $\finit{\Leftarrow}{Q'}$.
  Moreover, $\p$ is
  $\infinit{\Rightarrow}{Q}$ iff $\lnot \p$ is
  $\infinit{\Leftarrow}{Q'}$.
%  and
%  \nb{A: why needed? \\ Used in proofs of Lemma 12 and Th. 18 (+ maybe in future discussion in Verification Section, I don't know). Not necessary though, we can safely remove it}
%  $\lnot \p$ is
%  $\infinit{\Rightarrow}{Q}$ iff $\p$ is $\infinit{\Leftarrow}{Q'}$.
\end{restatable}
%
\begin{proof}
  Suppose that $\p$ is $\finit{\Rightarrow}{Q}$, i.e.:
  $\forall \Fmf ( \Fmf \mdl^{\assign} \p \Rightarrow Q \Imf \in
  \Ext(\Fmf).\Imf \mdl^{\assign} \p )$, for all assignments $\assign$.
  This is equivalent to:
  $\forall \Fmf ( Q' \Imf \in \Ext(\Fmf).\Imf \mdl^{\assign} \lnot \p
  \Rightarrow \Fmf \mdl^{\assign} \lnot \p )$, for all assignments
  $\assign$.  That is, $\lnot\p$ is $\finit{\Leftarrow}{Q'}$.  The
  remaining case is analogous.
\end{proof}


%O: transformed into a remark because it is clear from the definition
%~ \TheorFiniteInfinite*
%~ \begin{proof}
%~ Straightforward, from the definitions of
%~ $\infinit{\Rightarrow}{\exists}$
%~ and
%~ $\finit{\Rightarrow}{\exists}$.
%~ \end{proof}


%\Lemmaequconj*
\begin{restatable}{lemma}{Lemmaequconj}\label{lemma:equconj}
  Let $\p$ and $\psi$ be $\QTLfr{}{}{}$ formulas.  If
  $\p \land \lnot \psi$ and $\psi \land \lnot \p$ are
  $\finit{\Rightarrow}{\exists}$, then $\equivinf{\p}{\psi}$ implies
  $\equivfin{\p}{\psi}$.  Moreover, if $\p \land \lnot \psi$ and
  $\psi \land \lnot \p$ are $\infinit{\Rightarrow}{\exists}$, then
  $\equivfin{\p}{\psi}$ implies $\equivinf{\p}{\psi}$.
\end{restatable}
%
\begin{proof}
  Suppose that $\p \land \lnot \psi$ and $\psi \land \lnot \p$ are
  $\finit{\Rightarrow}{\exists}$.  We have $\equivinf{\p}{\psi}$ iff
  $\p \land \lnot \psi$
%  not $\satinf{\p \land \lnot \psi}$
  and $\psi \land \lnot \p$
  are not $\QTLfr{i}{}{}$ satisfiable.
%  and
%  not
%%  \nb{O: remove sat notation? }
%  $\satinf{\psi \land \lnot \p}$.
  Assume $\equivinf{\p}{\psi}$.
%  \nb{O: added}
  By $\finit{\Rightarrow}{\exists}$, the previous step implies:
  $\p \land \lnot \psi$
%  is not $\QTLfr{f}{}{}$ satisfiable
%  not
%  $\satfin{\p \land \lnot \psi}$
  and
  $\psi \land \lnot \p$
  are not $\QTLfr{f}{}{}$ satisfiable,
%  not
%  $\satfin{\psi \land \lnot \p}$,
  which is equivalent to
  $\equivfin{\p}{\psi}$.
  Moreover, suppose that $\p \land \lnot \psi$
  and $\psi \land \lnot \p$ are $\infinit{\Rightarrow}{\exists}$.  We
  have that $\equivfin{\p}{\psi}$ iff
  $\p \land \lnot \psi$
%  is not $\QTLfr{f}{}{}$ satisfiable
%  not
%  $\satfin{\p \land \lnot \psi}$
  and
  $\psi \land \lnot \p$
  are not $\QTLfr{f}{}{}$ satisfiable
%  not
%  $\satfin{\psi \land \lnot \p}$.
  If $\equivfin{\p}{\psi}$,
%  \nb{O: added}
  by $\infinit{\Rightarrow}{\exists}$
  we have %the previous step implies:
  $\p \land \lnot \psi$
  and
  $\psi \land \lnot \p$
  are not $\QTLfr{i}{}{}$ satisfiable.
%  not
%  $\satinf{\p \land \lnot \psi}$
%  and
%  not
%  $\satinf{\psi \land \lnot \p}$.
  Thus, $\equivinf{\p}{\psi}$.
\end{proof}


%\Theoremequfininf*
%\begin{proof}
%We have that
%$\equivfin{\p}{\psi}$
%iff
%$\lnot \satfin{\p \land \lnot \psi} \land \lnot \satfin{\psi \land \lnot \p}$.
%By
%$\infinit{\Rightarrow}{\exists}$,
%the previous step implies:
%$\lnot \satinf{\p \land \lnot \psi} \land \lnot \satinf{\psi \land \lnot \p}$.
%Equivalently,
%$\equivinf{\p}{\psi}$.
%\end{proof}
%
%
%
%\Theoremequinffin*
%\begin{proof}
%We have
%$\equivinf{\p}{\psi}$
%iff
%$\lnot \satinf{\p \land \lnot \psi} \land \lnot \satinf{\psi \land \lnot \p}$.
%By
%$\finit{\Rightarrow}{\exists}$,
%the previous step implies:
%$\lnot \satfin{\p \land \lnot \psi} \land \lnot \satfin{\psi \land \lnot \p}$,
%which is equivalent to
%$\equivfin{\p}{\psi}$.
%\end{proof}

 
%\Lemmaarrowexists*
\begin{restatable}{lemma}{Lemmaarrowexists}\label{lemma:arrowexists}
  Let $\p$ and $\psi$ be $\QTLfr{}{}{}$ formulas.  If $\p$ and $\psi$
  are $\finit{}{\exists}$ or $\finit{}{\forall}$, then
  $\p \land \lnot \psi$ and $\psi \land \lnot \p$ are
  $\finit{\Rightarrow}{\exists}$.  Moreover, if $\p$ and $\psi$ are
  $\infinit{}{\exists}$ or $\infinit{}{\forall}$, then
  $\p \land \lnot \psi$ and $\psi \land \lnot \p$ are
  $\infinit{\Rightarrow}{\exists}$.
\end{restatable}
%
\begin{proof}
  %\nb{M: Changed proof and added ref. Lemma~\ref{lemma:not} O: ok thanks}
  Suppose that $\p$ and $\psi$ are $\finit{}{\exists}$ (the
  case for $\finit{}{\forall}$ is similar), and let
  $\chi \in \{ \p, \psi \}$.
%  
%  For all assignments $\assign$, we have
%  $\forall \Fmf (\Fmf \mdl^{\assign} \chi \Rightarrow \exists \Imf \in
%  \Ext(\Fmf). \Imf \mdl^{\assign} \chi)$ and
%  $\forall \Fmf (\Fmf \not \mdl^{\assign} \chi \Rightarrow \forall
%  \Imf \in \Ext(\Fmf). \Imf \not \mdl^{\assign} \chi$.  The latter is
%  equivalent to:
%  $\forall \Fmf (\Fmf \mdl^{\assign} \lnot \chi \Rightarrow \forall
%  \Imf \in \Ext(\Fmf). \Imf \mdl^{\assign} \lnot \chi)$, which in turn
%  implies
%  $\forall \Fmf (\Fmf \mdl^{\assign} \lnot \chi \Rightarrow \exists
%  \Imf \in \Ext(\Fmf). \Imf \mdl^{\assign} \lnot \chi)$.  Thus, we
%  have that both $\chi$ and $\lnot \chi$ are
%  $\finit{\Rightarrow}{\exists}$.
%  
  Since, in particular, $\chi$ is $\finit{\Leftarrow}{\exists}$, by
  Lemma~\ref{lemma:not} we have that $\lnot \chi$ is also
  $\finit{\Rightarrow}{\forall}$, and thus
  $\finit{\Rightarrow}{\exists}$.
  %
  Thus, we have that both $\chi$ and $\lnot \chi$ are
  $\finit{\Rightarrow}{\exists}$.
  Suppose now, towards a
  contradiction, that $\p \land \lnot \psi$ is not
  $\finit{\Rightarrow}{\exists}$.  This means that there is a finite
  trace $\Fmf$ such that $\Fmf \mdl^{\assign} \p$ and
  $\Fmf \not \mdl^{\assign} \psi$, and for all $\Imf \in \Ext(\Fmf)$:
  $\Imf \not \mdl^{\assign} \p$ or $\Imf \mdl^{\assign} \psi$.  Given
  that $\p$ is $\finit{\Rightarrow}{\exists}$, there is a
  $\Imf' \in \Ext(\Fmf)$ such that $\Imf' \mdl^{\assign} \p$.  Also,
  since $\psi$ is $\finit{\Leftarrow}{\exists}$, we have that for all
  $\Imf \in \Ext(\Fmf)$, $\Imf \not \mdl^{\assign} \psi$.  Consider
  now an arbitrary $\Imf \in \Ext(\Fmf)$: if
  $\Imf \mdl^{\assign} \psi$, we have a contradiction from the fact
  that for all $\Imf \in \Ext(\Fmf)$, $\Imf \not \mdl^{\assign} \psi$.
  Then, for all $\Imf \in \Ext(\Fmf)$, we have
  $\Imf \not \mdl^{\assign} \p$, which contradicts the fact that there
  is a $\Imf' \in \Ext(\Fmf)$
%  \nb{O: seems it should be $\Ext(\Fmf)$}
  such that $\Imf' \mdl^{\assign} \p$.
  This absurd shows that $\p \land \lnot \psi$ is
  $\finit{\Rightarrow}{\exists}$ (the proof for $\psi \land \lnot \p$
  is analogous).
  
  Moreover, suppose $\p$ and $\psi$ are $\infinit{}{\exists}$ (the case for
  $\infinit{}{\forall}$ is similar), and again let
  $\chi \in \{ \p, \psi \}$.
%  
%  Then, for all assignments $\assign$, we
%  have both
%  $\forall \Imf (\Imf \mdl^{\assign} \chi \Rightarrow \exists \Fmf \in
%  \Pre(\Imf). \Fmf \mdl^{\assign} \chi)$ and
%  $\forall \Imf (\Imf \not \mdl^{\assign} \chi \Rightarrow \forall
%  \Fmf \in \Pre(\Imf). \Fmf \not \mdl^{\assign} \chi$.  The latter is
%  equivalent to:
%  $\forall \Imf (\Imf \mdl^{\assign} \lnot \chi \Rightarrow \forall
%  \Fmf \in \Pre(\Imf). \Fmf \mdl^{\assign} \lnot \chi)$, which in turn
%  implies
%  $\forall \Imf (\Imf \mdl^{\assign} \lnot \chi \Rightarrow \exists
%  \Fmf \in \Pre(\Imf). \Fmf \mdl^{\assign} \lnot \chi)$.  Thus, we
%  have that both $\chi$ and $\lnot \chi$ are
%  $\infinit{\Rightarrow}{\exists}$.
%
  Since, in particular, $\chi$ is
  $\infinit{\Leftarrow}{\exists}$,
  by Lemma~\ref{lemma:not} we have that $\lnot \chi$ is also
  $\infinit{\Rightarrow}{\forall}$,
  and thus
  $\infinit{\Rightarrow}{\exists}$.
  %
  Thus, we have that both $\chi$ and $\lnot \chi$ are
  $\infinit{\Rightarrow}{\exists}$.
  Suppose now, towards a
  contradiction, that $\p \land \lnot \psi$ is not
  $\infinit{\Rightarrow}{\exists}$.  We have that there is an infinite
  trace $\Imf$ and an assignment $\assign$ such that $\Imf \mdl^{\assign} \p$ and
  $\Imf \mdl^{\assign} \lnot \psi$, and for all $\Fmf \in \Pre(\Imf)$:
  $\Fmf \not \mdl^{\assign} \p$ or $\Fmf \mdl^{\assign} \psi$.  Since
  $\p$ is $\infinit{\Rightarrow}{\exists}$, there is a
  $\Fmf' \in \Pre(\Imf)$ such that $\Fmf' \mdl^{\assign} \p$.
  Moreover, since $\lnot \psi$ is $\infinit{\Rightarrow}{\forall}$, we have
  that for all $\Fmf \in \Pre(\Imf)$, $\Fmf \mdl^{\assign} \lnot \psi$.
  Given an arbitrary $\Fmf \in \Pre(\Imf)$, if
  $\Fmf \mdl^{\assign} \psi$, we contradict the fact that for all
  $\Fmf \in \Pre(\Imf)$, $\Fmf \not \mdl^{\assign} \psi$.  Thus, for
  all $\Fmf \in \Pre(\Imf)$, we have $\Fmf \not \mdl^{\assign} \p$,
  contradicting the fact that there is a $\Fmf' \in \Pre(\Imf)$ such
  that $\Fmf' \mdl^{\assign} \p$.  This absurd proves that
  $\p \land \lnot \psi$ is $\infinit{\Rightarrow}{\exists}$ (the proof
  for $\psi \land \lnot \p$ is analogous).
\end{proof}


\Theoremusonlyif*
\begin{proof}
  %({\bf point 1}) It 
  Points (1) and (2) follow from Lemma~\ref{lemma:equconj} and
  Lemma~\ref{lemma:arrowexists}.  We provide also a direct proof.
  Assume $\p$ and $\psi$ to be $\finit{}{\exists}$ (the proof for
  $\finit{}{\forall}$ is analogous).  Given an assignment $\assign$,
  let $\Fmf$ be a finite trace such that $\Fmf \mdl^{\assign} \p$.  By
  $\finit{}{\exists}$, there is an infinite trace
  % $\Imf$ such that $\Imf = \FImf'$, for some infinite trace $\Imf'$,
  % and $\Imf \mdl \p$.
  $\Imf \in \Ext(\Fmf)$ such that $\Imf \mdl^{\assign} \p$ Since
  $\equivinf{\p}{\psi}$, we have that $\Imf \mdl^{\assign} \psi$.  By
  $\finit{}{\exists}$, $\Fmf \models^{\assign} \psi$.  
   The converse
   direction can be obtained analogously, by swapping $\p$ and $\psi$.

   %({\bf point 2}) 
   We now show Point~(3). 
   Given a finite trace $\Fmf$ and an assignment
   $\assign$, suppose that $\Fmf \mdl^{\assign} \p$.  Since $\p$
   is $\finit{\Rightarrow}{\exists}$, we have that for some
   $\Imf \in \Ext(\Fmf)$, $\Imf \mdl^{\assign} \p$.  By assumption,
   $\equivinf{\p}{\psi}$, so $\Imf \mdl^{\assign} \psi$.  As $\psi$ is
   $\infinit{\Rightarrow}{\forall}$, $\Imf \mdl^{\assign} \psi$
   implies that, for all $\Fmf' \in \Pre(\Imf)$,
   $\Fmf' \mdl^{\assign} \psi$.  Thus, in particular,
   $\Fmf \mdl^{\assign} \psi$.  The other direction can be obtained
     by swapping $\p$ and $\psi$.
%%% COMPLETE \infinit{\forall}{\forall}
%Now suppose that $\p$ and $\psi$ are $\infinit{\forall}{\forall}$, and let $\Fmf \models \p$. 
%\nb{M: Complete}
\end{proof}

% \begin{proof}  
%The result for~\ref{ins:degetal} can be seen as   a
%consequence of Theorem~\ref{theor:inschar}. 
%Given a finite trace \Fmf, if $\Fmf\models \p$ then, as $\p$ is   
%  insensitive~\ref{ins:degetal}, $\FEmf\models \p$. 
%  By assumption,  $\p\equiv_\Imf\psi$, so  $\FEmf\models \psi$. 
%  As  $\psi$ is   
%  insensitive~\ref{ins:degetal}, $\FEmf\models \psi$ implies $\Fmf\models \psi$. 
%  The converse direction can again be obtained by swapping $\p$ and $\psi$. 
%  \end{proof}



\Theoremusif*
\begin{proof}
  Points (1) and (2) follow again from Lemma~\ref{lemma:equconj} and
  Lemma~\ref{lemma:arrowexists}.  Here we give a direct proof as well.
  Suppose that $\p$ and $\psi$ are $\infinit{}{\exists}$ (the proof
  for for $\infinit{}{\forall}$ is analogous).  Given an assignment
  $\assign$, let \Imf be an infinite trace such that
  $\Imf \models^{\assign} \p$.  By $\infinit{}{\exists}$,
%there is $\Fmf$ such that $\Imf = \FImf'$ for some $\Imf'$, and $\Fmf \mdl \p$. 
  there is $\Fmf \in \Pre(\Imf)$ such that $\Fmf \mdl^{\assign} \p$.
  As $\equivfin{\p}{\psi}$, this means that
%there is $\Fmf$ such that $\Imf = \FImf'$ for some $\Imf'$, and $\Fmf \mdl \psi$.
  $\Fmf \mdl^{\assign} \psi$.  Since $\psi$ is $\infinit{}{\exists}$,
  we have $\Imf \mdl^{\assign} \psi$.  The converse direction is
  obtained analogously, by swapping $\p$ and $\psi$. %replacing $\p$ by $\psi$ and vice-versa.

  %({\bf point 2}) 
  We now show  Point~(3). 
  Let $\Imf$ be an infinite trace and $\assign$ be an
  assignment such that $\Imf \mdl^{\assign} \p$.  As $\p$ is
  $\infinit{\Rightarrow}{\exists}$, there is $\Fmf \in \Pre(\Imf)$
  such that $\Fmf \mdl^{\assign} \p$.  Given that
  $\equivfin{\p}{\psi}$, $\Fmf \mdl^{\assign} \psi$.  By
  $\finit{\Rightarrow}{\forall}$, for all $\Imf' \in \Ext(\Fmf)$:
  $\Imf' \mdl^{\assign} \psi$.  Therefore, we have also
  $\Imf \mdl^{\assign} \psi$.  The converse direction is obtained in a
  similar way by swapping $\p$ and $\psi$.
\end{proof}


%\begin{restatable}{lemma}{LemmaBoolean}\label{lem:bool}
%  \nb{M: merge with next Th.}  Let $\p$ be a non-temporal $\QTLfr{}{}{}$
%  formula. Then, for all finite traces
%  $\Fmf = (\Delta, (\Fmc)_{n \in [0, l]})$, all $n \in [0, l]$, and
%  all assignments $\assign$:
%\[
%	\exists \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \p \Leftrightarrow \forall \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \p.
%\]
%Moreover, for all infinite traces $\Imf$, all $n \in \Nbb$, and all assignments $\assign$:
%\[
%	\exists \Fmf \in \Prel{n}(\Imf). \Fmf, n \models^{\assign} \p \Leftrightarrow \forall \Fmf \in \Prel{n}(\Imf). \Fmf, n \models^{\assign} \p.
%\]
%\end{restatable}
%\begin{proof}
%By induction on non-temporal formulas.
%\end{proof}


\TheoremBoolean*
\begin{proof}
Clearly, assuming that $\p$ has no temporal operators, for any
finite/infinite trace 
%\nb{M: $\Tmf \to \Mmf$}
\Mmf,  $\Mmf$ satisfies $\p$ iff  
%$\p$ is satisfied at time point $0$. Since there are no 
%temporal operators, 
any extension/prefix of \Mmf satisfies $\p$. 
%~ Let $\p$ be a non-temporal $\QTLfr{}{}{}$ formula.
%~ Since there are no operators to interpret with respect to a different time point, we notice the following.
%~ For all finite traces
  %~ $\Fmf = (\Delta, (\Fmc)_{n \in [0, l]})$, all $n \in [0, l]$, and
  %~ all assignments $\assign$:
%~ \[
	%~ \exists \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \p \Leftrightarrow \forall \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \p.
%~ \]
%~ Moreover, for all infinite traces $\Imf$, all $n \in \Nbb$, and all assignments $\assign$:
%~ \[
	%~ \exists \Fmf \in \Prel{n}(\Imf). \Fmf, n \models^{\assign} \p \Leftrightarrow \forall \Fmf \in \Prel{n}(\Imf). \Fmf, n \models^{\assign} \p,
%~ \]
%~ where
%~ $\Prel{n}(\Imf) = \{ \Fmf = (\Delta, (\Fmc)_{m \in [0, l]}) \mid l \geq n \text{ and } \Imf = \Fmf \cdot \Imf', \text{ for some } $\Imf'$ \}$.
%~ Using this observation together with Lemma~\ref{lemma:not}, it is easy to prove by induction on non-temporal formulas $\p$ that for all $\Fmf = (\Delta, (\Fmc)_{n \in [0, l]})$, all $n \in [0,l]$, and all assignments $\assign$:
%~ \[
	%~ \Fmf, n \models^{\assign} \p \Leftrightarrow Q \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \p
%~ \]
%~ and
%~ \[
	%~ \Imf, n \models^{\assign} \p \Leftrightarrow \exists \Fmf \in \Prel{n}(\Imf). \Fmf, n \models^{\assign} \p,
%~ \]
%~ where $Q \in \{ \forall, \exists \}$.
%~ Therefore, in particular, a non-temporal formula $\p$ is
%~ $\finit{}{Q}$
%~ and
%~ $\infinit{}{Q}$.
\end{proof}

 

%\nb{O:showing lemmas}

In the proofs of Theorems~\ref{thm:diamond} and~\ref{thm:box} we use the following notation. 
Given a finite trace $\Fmf = (\Delta, \Fmc_{n \in [0, l]})$, we denote by  $\Fmf^{\omega}$ 
the extension of  \Fmf with the infinite trace 
$(\Fmf^l)^\omega$, where $\Fmf^l$ is the finite trace 
with only the last instant of \Fmf.
Also, given and assignment 
$\assign$ and an element $d$ of a domain $\Delta$ (of 
a finite or infinite trace), we write
 $\assign_d$ for the result of modifying $\assign$ so that 
  $x$ maps to $d$.
  The next lemma is useful to prove Theorem~\ref{thm:diamond}.
  %~ \begin{lemma}\label{lem:auxfinite}
%~ For all finite traces \Fmf, all  assignments \assign,
%~ and all $\D^+\forall$-formulas $\varphi$, 
 %~ $\Fmf\models^\assign \varphi$ iff 
%~ $\Fmf^{\omega}\models^\assign \varphi$.
%~ \end{lemma}
%~ \begin{proof} 
%~ The proof is by induction. 
%~ In the base case we have all non-temporal $\D^+\forall$-formulas.
%~ Assume that the lemma holds for a $\D^+\forall$-formula $\varphi$. 
%~ If $\Fmf\models^\assign \D^+\varphi$ then 
%~ there is $n\geq 0$ such that  $\Fmf,n\models^\assign \varphi$. 
%~ Let $\Fmf'$ be the suffix of \Fmf starting at $n$. %O: not very precise...
%~ By inductive hypothesis, $(\Fmf')^\omega\models \varphi$. 
%~ Then, by definition of $\Fmf'$,
%~ $\Fmf^\omega\models^\assign \D^+\varphi$.
%~ Conversely, if $\Fmf^\omega\models^\assign \D^+\varphi$ then 
%~ there is $n\geq 0$ such that  $\Fmf^\omega,n\models^\assign \varphi$. 
%~ By definition of $\Fmf^\omega$, there is a suffix 
%~ $\Fmf'$ of $\Fmf$ such that $(\Fmf')^\omega$
%~ corresponds to the suffix of $\Fmf^\omega$ starting at $n$. 
 %~ By inductive hypothesis, $\Fmf'\models \varphi$. 
 %~ As $\Fmf'$ is a suffix of  $\Fmf$, we have that
 %~ $\Fmf\models^\assign \D^+\varphi$.
 %~ Other cases can be proved 
%~ by straightforward applications of the inductive hypothesis. 
%~ %$\Fmf^{\omega}\models^\assign \varphi$.
%~ \end{proof}
\begin{lemma}\label{lem:aux3}
Let \Fmf be a finite trace and let $\Fmf'$ 
be a prefix of \Fmf.
For all  assignments \assign,
and all $\D$-formulas $\varphi$, 
if $\Fmf'\models^\assign \varphi$ then 
$\Fmf\models^\assign \varphi$ .
\end{lemma}
\begin{proof}
The proof is by induction. 
In the base case we have all non-temporal $\D$-formulas.
Assume that the lemma holds for a $\D$-formula $\varphi$. 
Let \Fmf be a finite trace, let $\Fmf'$ 
be a prefix of \Fmf and let \assign be an assignment.
If $\Fmf'\models^\assign \D\varphi$ then 
there is $n>0$ such that $\Fmf',n\models^\assign \varphi$.
As $\Fmf'$ is a prefix of \Fmf, we have that 
$\Fmf,n\models^\assign \varphi$.
This means that there is  $n>0$ such that $\Fmf,n\models^\assign \varphi$.
Thus,  $\Fmf\models^\assign \D\varphi$. Other cases can be proved 
by straightforward applications of the inductive hypothesis. 
\end{proof}


\TheoremDiamond*
\begin{proof}
  We first show that all $\D^{+}\forall$-formulas are $\finit{}{\forall}$.
  In Claim~\ref{cl:diamond1}, we show that all $\D^{+}\forall$-formulas are 
  $\finit{\Rightarrow}{\forall}$ (in fact for the $\Rightarrow$ 
  we can also allow $\D\varphi$ in the grammar).
  Then, in Claim~\ref{cl:diamond2}, 
  we show that all $\D^{+}\forall$-formulas are 
  $\finit{\Leftarrow}{\forall}$.
  
  %at all formulas generated by
  %the extension of the grammar rule for 
  %$\D^{+}\forall$-formulas with $\D\varphi$ is
  %$\finit{\Rightarrow}{\forall}$.
  % that $\D^{+}\forall$-formulas
  %extended with formulas of the form  $\D\varphi$.
  %\nb{A:and $\D^{+}\forall$-formulas?}
  %   are $\finit{\Rightarrow}{\forall}$,
  %which also implies that $\D^{+}$-formulas are
  %$\finit{\Rightarrow}{\forall}$ since disjunction is also in the
  %fragment of $\D$-formulas.
  %
\begin{claim}\label{cl:diamond1}
  For all finite traces \Fmf, all assignments \assign, and all
  $\D^{+}\forall$-formulas $\varphi$, if $\Fmf\models^\assign \varphi$ then, for
  all $\Imf\in\textit{Ext}(\Fmf)$, $\Imf \models^\assign \varphi$.
\end{claim}
\noindent\textit{Proof of Claim~\ref{cl:diamond1}}
The proof is by  induction. In the base case 
we have all non-temporal $\D^{+}\forall$-formulas (Theorem~\ref{thm:boolean}).
Assume that the claim holds for $\varphi$ and $\psi$, 
and there is a finite trace \Fmf and an assignment $\assign$ such that 
$\Fmf\models^\assign \varphi'$. We now argue that, 
for all $\Imf\in\textit{Ext}(\Fmf)$, 
$\Imf \models^\assign \varphi'$, where $\varphi'$ is as follows.
\begin{itemize}
\item For $\varphi'=\D\varphi$: by assumption 
$\Fmf\models^\assign \D\varphi$. 
This means that there is $n\in (0,l]$ such that 
$\Fmf,n\models^\assign  \varphi$. In other words,  
$\Fmf^n\models^\assign  \varphi$, 
where $\Fmf^n$ is the suffix of \Fmf starting from time point $n$. 
By the inductive hypothesis, if $\Fmf^n\models^\assign \varphi$
then, for all $\Imf\in\textit{Ext}(\Fmf^n)$, 
%we have that 
$\Imf \models^\assign \varphi$.
This implies that for all $\Imf\in\textit{Ext}(\Fmf)$, 
there is $n\in (0,\infty)$  such that 
$\Imf,n \models^\assign \varphi$. So, 
$\Imf \models^\assign \D\varphi$ for all $\Imf\in\textit{Ext}(\Fmf)$.
\item For $\varphi'=\forall x\varphi$: by assumption 
$\Fmf\models^\assign \forall x\varphi$. 
This means that for all $d\in\Delta$, $\Fmf\models^{\assign_d} \varphi[d]$, 
 where $\assign_d$ extends $\assign$ by mapping $x$ to $d$. 
By applying the inductive hypothesis on every $\varphi[d]$ with $d\in\Delta$,
we have that, for all $d\in\Delta$ and all $\Imf\in\textit{Ext}(\Fmf)$,
 $\Imf\models^{\assign_d} \varphi[d]$.
By semantics of $\forall$, for all $\Imf\in\textit{Ext}(\Fmf)$,
 $\Imf\models^\assign \forall x\varphi$. 
\item For $\varphi'=\exists x\varphi$: 
by assumption 
$\Fmf\models^\assign \exists x\varphi$. 
This means that there is $d\in\Delta$ such that 
$\Fmf\models^{\assign_d} \varphi[d]$, 
 where $\assign_d$ extends $\assign$ by mapping $x$ to $d$. 
By applying the inductive hypothesis,
we have that, for   all $\Imf\in\textit{Ext}(\Fmf)$,
 $\Imf\models^{\assign_d} \varphi[d]$.
By semantics of $\exists$, for all $\Imf\in\textit{Ext}(\Fmf)$,
 $\Imf\models^\assign \exists x\varphi$. 
\item The remaining cases  can 
be proved in a straightforward way  using the 
inductive hypothesis. 
\end{itemize}
 We observe that 
problematic formulas for this claim are, e.g., $\D \textit{last}$.  
This formula holds in any finite trace \Fmf 
 but it does not on any extension of \Fmf. 
  Claim~\ref{cl:diamond1}  
relies on the fact that the grammar rule for $\D$-formulas
does not allow $\textit{last}$. 
The boolean case $\varphi\vee\psi$ also relies 
on the fact that the claim is for $\D$-formulas, since, e.g., 
the formula $\D\B^{+} P(x)\vee \D\B^{+} Q(x)$
holds on any finite trace (with more than one time point) where $P(x)\vee Q(x)$ is satisfied 
in the last time point but there are extensions 
which do not satisfy $\D\B^{+} P(x)\vee \D\B^{+} Q(x)$. 
%In\nb{A: added} the following we show $\finit{\Leftarrow}{\forall}$. 

\begin{claim}\label{cl:diamond2}
For all finite traces \Fmf, all assignments \assign, and
all $\D^{+}\forall$-formulas
    $\varphi$,  if, 
for all $\Imf\in\textit{Ext}(\Fmf)$, 
%we have that 
$\Imf \models^\assign \varphi$ then 
$\Fmf\models^\assign \varphi$. 
\end{claim}
\noindent\textit{Proof of Claim~\ref{cl:diamond2}}
If, 
for all $\Imf\in\textit{Ext}(\Fmf)$, 
%we have that 
$\Imf \models^\assign \varphi$ then,
in particular, $\Fmf^\omega \models^\assign \varphi$. 
We show that 
$\Fmf^\omega \models^\assign \varphi$ implies $\Fmf\models^\assign \varphi$. 
The proof is by induction. 
In the base case we have all non-temporal $\D^+\forall$-formulas.
Assume that the lemma holds for a $\D^+\forall$-formula $\varphi$. 
%~ If $\Fmf\models^\assign \D^+\varphi$ then 
%~ there is $n\geq 0$ such that  $\Fmf,n\models^\assign \varphi$. 
%~ Let $\Fmf'$ be the suffix of \Fmf starting at $n$. %O: not very precise...
%~ By inductive hypothesis, $(\Fmf')^\omega\models \varphi$. 
%~ Then, by definition of $\Fmf'$,
%~ $\Fmf^\omega\models^\assign \D^+\varphi$.
\begin{itemize}
\item If $\Fmf^\omega\models^\assign \D^+\varphi$ then 
there is $n\geq 0$ such that  $\Fmf^\omega,n\models^\assign \varphi$. 
By definition of $\Fmf^\omega$, there is a suffix 
$\Fmf'$ of $\Fmf$ such that $\Fmf'^\omega$
corresponds to the suffix of $\Fmf^\omega$ starting at $n$. 
 By inductive hypothesis, $\Fmf'\models \varphi$. 
 As $\Fmf'$ is a suffix of  $\Fmf$, we have that
 $\Fmf\models^\assign \D^+\varphi$.
 \item If
$\Fmf^\omega\models^\assign \forall x\varphi$. 
This means that, for all $d\in\Delta$,
$\Fmf^\omega\models^\assign  \varphi[d]$. 
By the inductive hypothesis, for all $d\in\Delta$, $\Fmf\models^\assign  \varphi[d]$. 
So, 
$\Fmf\models^\assign \forall x\varphi$.
\item 
If
$\Fmf^\omega\models^\assign \exists x\varphi$. 
This means that there is $d\in\Delta$ such that 
$\Fmf^\omega\models^\assign  \varphi[d]$. 
By the inductive hypothesis,   $\Fmf\models^\assign  \varphi[d]$. 
This means that 
$\Fmf\models^\assign \exists x\varphi$.
\item The remaining cases  can 
be proved in a straightforward way   using the 
inductive hypothesis. 
\end{itemize}

%~ The proof is by  induction as in Claim~\ref{cl:diamond1}, with 
%~ all non-temporal  $\D^{+}\forall$-formulas in the base case (Theorem~\ref{thm:boolean}).
%~ Assume  that the claim holds for $\varphi$ and $\psi$. 
%~ \begin{itemize}
%~ \item The case for formulas of the form  $\D^{+}\varphi$ is as follows.
%~ Assume that given a $\D^{+}$-formula $\varphi$ and a finite trace $\Fmf = (\Delta, \Fmc_{n \in [0, l]})$
%~ we have that, for all $\Imf\in \textit{Ext}(\Fmf)$,  $\Imf\models^\assign\D^+ \varphi$.
%~ Assume to the contrary that $\Fmf\not\models^\assign \D^+\varphi$. 
%~ This means that, for all $n\in [0,l]$, $\Fmf,n\not\models^\assign \varphi$. 
%~ %Together with our assumption, 
%~ This implies that, for all $\Imf\in \textit{Ext}(\Fmf)$, 
 %~ $\Imf,l+1\models^\assign\D^+ \varphi$  (because 
%~ time points in \Fmf range in $[0, l]$). 
%~ So $\D^+ \varphi$ is valid in all infinite traces.
%~ %\nb{A: I don't see why. What about considering two cases, $\varphi\equiv\top$ and $\varphi\not\equiv\top$} 
%~ One can show with an inductive argument that, 
%~ for all $\D^{+}$-formulas $\varphi$, 
%~ if $\varphi$ is valid in all infinite traces then it is 
%~ valid in all finite traces: this holds for non-temporal 
%~ $\D^{+}$-formulas and, for formulas of the form $\D^+\varphi$ we know 
%~ that $\D^+\varphi$ is valid in all infinite traces iff $\varphi$ 
%~ is valid. The same holds for finite traces, $\D^+\varphi$ is valid in all 
%~ finite traces iff $\varphi$ is also valid.
%~ This contradicts our assumption that $\Fmf\not\models^\assign \D^+\varphi$. 
%~ Thus, $\Fmf\models^\assign \D^+\varphi$. 
%~ %by Lemma~\ref{lem:aux3};
%~ %The case for formulas of the form $\forall x\varphi$ is 
%~ \item Now, we consider formulas of the form  
%~ $\forall x\varphi$. 
%~ Let $\Fmf$ be a finite trace.
%~ % be  a finite trace and let 
%~ % $\Imf$ be an element of $\textit{Ext}(\Fmf)$.
 %~ Assume that, for all $\Imf\in\textit{Ext}(\Fmf)$, we have
  %~ $\Imf\models^\assign \forall x\varphi$. By semantics of $\forall$, 
 %~ we have that, for all $\Imf\in\textit{Ext}(\Fmf)$, 
 %~ and for all $d\in\Delta$, $\Imf\models^{\assign_d} \varphi[d]$, 
 %~ where $\assign_d$ extends $\assign$ by mapping $x$ to $d$. 
 %~ By applying the inductive hypothesis on every $\varphi[d]$ with $d\in\Delta$
 %~ we have that $\Fmf\models^{\assign_d} \varphi[d]$, for all $d\in\Delta$.
 %~ By semantics of $\forall$,  $\Fmf\models^\assign \forall x\varphi$.  
%~ %?? \nb{on going}
%~ \item The case for formulas of the form $\exists x\varphi$ is as follows. 
 %~ Assume that, for all $\Imf\in\textit{Ext}(\Fmf)$, we have
  %~ $\Imf\models^\assign \exists x\varphi$. 
  %~ By semantics of $\exists$, 
 %~ we have that, for all $\Imf\in\textit{Ext}(\Fmf)$, 
 %~ there is $d\in\Delta$ such that $\Imf\models^{\assign_d} \varphi[d]$, 
 %~ where $\assign_d$ extends $\assign$ by mapping $x$ to $d$. 
 %~ By applying the inductive hypothesis,
 %~ we have that $\Fmf\models^{\assign_d} \varphi[d]$.
 %~ By semantics of $\exists$,  $\Fmf\models^\assign \exists x\varphi$.  
%~ \item
%~ %by Lemma~\ref{lem:aux4}; 
%~ The case for formulas of the form $\varphi\vee \psi$ is as follows. 
%~ One can show that for all $\D^{+}$-formulas $\varphi$ and all finite traces $\Fmf$, 
%~ if $\Fmf\not\models \varphi$ then $\Fmf^\omega\not\models \varphi$: 
%~ this holds for all non-temporal formulas and if an eventuality is not 
%~ satisfied in \Fmf then, by definition of $\Fmf^\omega$, it will not be satisfied in  $\Fmf^\omega$.
%~ Assume that, 
 %~ for all $\Imf\in\textit{Ext}(\Fmf)$, 
%~ $\Imf \models^\assign \varphi\vee\psi$. 
%~ Suppose to the contrary that 
%~ $\Fmf\not\models^\assign \varphi\vee\psi$. 
%~ By the argument above, $\Fmf^\omega\not\models \varphi\vee\psi$. 
%~ Since $\Fmf^\omega\in\textit{Ext}(\Fmf)$,
%~ this contradicts our assumption that 
%~ for all $\Imf\in\textit{Ext}(\Fmf)$, $\Imf \models^\assign \varphi\vee\psi$. 
%~ Thus, $\Fmf\models^\assign \varphi\vee\psi$. 
%~ \item The remaining cases are a straightforward application 
%~ of the inductive hypothesis.
%~ \end{itemize}

\smallskip

We point out that this claim does not hold 
for $\D$-formulas (only for $\D^{+}$-formulas). 
To see this consider the formula $\D \top$, which holds 
in any infinite trace but not on a finite trace with 
only one time point. 

%~ \item 
%~ \end{itemize}

\medskip

We now show that all $\D$-formulas are $\infinit{}{\exists}$.  
In Claim~\ref{cl:diamond3}, we show that all $\D$-formulas 
are $\infinit{\Rightarrow}{\exists}$. 
Then, in Claim~\ref{cl:diamond4}, we show that all 
$\D$-formulas are $\infinit{\Leftarrow}{\exists}$. 

\begin{claim}\label{cl:diamond3}
For all infinite traces \Imf, all assignments \assign, and
all $\D$-formulas $\varphi$, if $\Imf\models^\assign \varphi$
then there is $\Fmf\in \textit{Pre}(\Imf)$ such that 
$\Fmf\models^\assign \varphi$.
\end{claim}
\noindent\textit{Proof of Claim~\ref{cl:diamond3}}
The proof is by   induction as in Claim~\ref{cl:diamond1}. 
In the base case 
we have all non-temporal $\D$-formulas (Theorem~\ref{thm:boolean}).
Assume that the claim holds for $\varphi$ and $\psi$.
\begin{itemize}
\item For formulas of the form $\D\varphi$ the argument is as follows. 
Let \Imf be  an infinite trace. 
By assumption $\Imf\models^\assign \D\varphi$. 
This means that there is $n\in (0,\infty)$ such that 
$\Imf,n\models^\assign  \varphi$. In other words,  
$\Imf^n\models^\assign  \varphi$, 
where $\Imf^n$ is the suffix of \Imf starting from time point $n$. 
By the inductive hypothesis, if $\Imf^n\models^\assign \varphi$
then  
there is $\Fmf\in \textit{Pre}(\Imf^n)$ such that
$\Fmf\models^\assign \D\varphi$. 
Then, there is $\Fmf'\in \textit{Pre}(\Imf)$ such that
$\Fmf'\models^\assign \D\varphi$. 
\item For formulas of the form $\exists x\varphi$ the argument is as follows. 
Let $\Imf  = (\Delta, \Imc_{n \in [0, \infty)})$ be  an infinite trace. 
By assumption $\Imf\models^\assign \exists x\varphi$. 
This means that there is $d\in\Delta$ such that 
$\Imf\models^\assign  \varphi[d]$.   
By the inductive hypothesis, if $\Imf\models^\assign \varphi[d]$
then  
there is $\Fmf\in \textit{Pre}(\Imf)$ such that
$\Fmf\models^\assign \varphi[d]$. 
So, $\Fmf\models^\assign \exists x\varphi$. 
\item  For formulas of the form $\varphi\wedge\psi$ the argument is as follows. 
Let \Imf be  an infinite trace. 
By assumption $\Imf\models^\assign \varphi\wedge\psi$. 
This means that $\Imf\models^\assign \varphi$ and 
$\Imf\models^\assign \psi$.   
By the inductive hypothesis,  
there are $\Fmf,\Fmf'\in \textit{Pre}(\Imf)$ such that
$\Fmf\models^\assign \varphi$ and $\Fmf'\models^\assign \psi$. 
By definition of $\Fmf$ and $\Fmf'$, 
 either $\Fmf'$ is a prefix of $\Fmf$ or vice versa. 
 Assume w.l.o.g. that $\Fmf'$ is a prefix of $\Fmf$.
By Lemma~\ref{lem:aux3}, if
$\Fmf'\models^\assign \psi$ then $\Fmf\models^\assign \psi$.
Then, $\Fmf\models^\assign \varphi$ and $\Fmf\models^\assign \psi$, 
and so, $\Fmf\models^\assign \varphi\wedge \psi$. 
\item The remaining cases are a straightforward application 
of the inductive hypothesis.
\end{itemize}

\begin{claim}\label{cl:diamond4}
For all infinite traces \Imf, all assignments \assign, and
all $\D$-formulas $\varphi$, if 
there is $\Fmf\in \textit{Pre}(\Imf)$ such that 
$\Fmf\models^\assign \varphi$ then 
 $\Imf\models^\assign \varphi$. 
\end{claim}
\noindent\textit{Proof of Claim~\ref{cl:diamond4}}
The proof is by   induction as in Claim~\ref{cl:diamond1}. 
In the base case 
we have all non-temporal $\D$-formulas (Theorem~\ref{thm:boolean}).
Assume that the claim holds for $\varphi$ and $\psi$.
\begin{itemize}
\item For formulas of the form $\D\varphi$ the argument is as follows. 
Let \Imf be  an infinite trace. 
By assumption there is $\Fmf\in \textit{Pre}(\Imf)$ such that
$\Fmf\models^\assign \D\varphi$. 
This means that there is $n\in (0,l]$ such that 
$\Fmf,n\models^\assign  \varphi$. In other words,  
$\Fmf^n\models^\assign  \varphi$, 
where $\Fmf^n$ is the suffix of \Fmf starting from time point $n$. 
By the inductive hypothesis, if $\Fmf^n\models^\assign \varphi$
then  
$\Imf^n \models^\assign \varphi$, 
where $\Imf^n$ is the suffix of \Imf starting from time point $n$. 
This implies that   
there is $n\in (0,\infty)$  such that 
$\Imf,n \models^\assign \varphi$. So, 
$\Imf \models^\assign \D\varphi$. 
\item For formulas of the form $\exists x\varphi$ the argument is as follows. 
Let $\Imf  = (\Delta, \Imc_{n \in [0, \infty)})$ be  an infinite trace. 
By assumption  there is $\Fmf\in \textit{Pre}(\Imf)$ such that
$\Fmf\models^\assign \exists x\varphi$. 
This means that there is $d\in\Delta$ such that 
$\Fmf\models^\assign  \varphi[d]$.   
By the inductive hypothesis, if $\Fmf\models^\assign \varphi[d]$
then  
$\Imf \models^\assign \varphi[d]$. 
So, $\Imf\models^\assign \exists x\varphi$. 
\item The remaining cases 
can be proved by a straightforward application 
of the inductive hypothesis. 
\end{itemize}
\end{proof}





The next lemmas are useful to prove Theorem~\ref{thm:box}.
%We observe that Lemma~\ref{lem:aux0} below
%does not hold for arbitrary 
%$\QTLfr{}{}{}$  formulas, e.g., it does not hold for   $\neg P(x)\wedge \B P(x)$.
 
%~ \begin{lemma}\label{lem:aux0}
%~ For all finite traces \Fmf, all infinite traces \Imf (sharing 
%~ the same domain of \Fmf),  all assignments \assign,
%~ and all $\B^{+}\exists$-formulas $\varphi$, 
%~ if $\Fmf\models^\assign \varphi$ and $\Imf\models^\assign \varphi$
%~ then $\FImf\models^\assign \varphi$.
%~ \end{lemma}

\begin{lemma}\label{lem:aux1}
Let \Fmf be a finite trace and let $\Fmf'$ 
be a prefix of \Fmf.
For all  assignments \assign,
and all $\B$-formulas $\varphi$, 
if $\Fmf'\not\models^\assign \varphi$  
then $\Fmf\not\models^\assign \varphi$.
\end{lemma}
\begin{proof}
The proof is by induction. 
In the base case we have all non-temporal $\B$-formulas.
Assume that the lemma holds for a $\B$-formula $\varphi$. 
Let \Fmf be a finite trace, let $\Fmf'$ 
be a prefix of \Fmf and let \assign be an assignment.
If $\Fmf'\not\models^\assign \B\varphi$  then 
there is $n>0$ such that $\Fmf',n\not\models^\assign \varphi$.
As $\Fmf'$ is a prefix of \Fmf, we have that 
$\Fmf,n\not\models^\assign \varphi$.
This means that there is  $n>0$ such that $\Fmf,n\not\models^\assign \varphi$.
Thus,  $\Fmf\not\models^\assign \B\varphi$. Other cases can be proved 
by straightforward applications of the inductive hypothesis. 
\end{proof}
\begin{lemma}\label{lem:aux11}
For all finite traces \Fmf, all infinite traces $\Imf\in \textit{Ext}(\Fmf)$,  
all assignments \assign,
and all $\B^{+}\exists$-formulas $\varphi$, 
if $\Fmf\models^\assign\B^+ \varphi$
then  $\Fmf^\omega\models^\assign \B^+\varphi$. 
\end{lemma}
\begin{proof}
The proof is by induction. 
In the base case we have all non-temporal $\B^{+}\exists$-formulas.
Assume that the lemma holds for $\varphi$ and $\psi$.
We now argue that if $\Fmf\models^\assign\B^+\B^+\varphi$
then  
%$(\Fmf)^\omega\models^\assign \B^+\varphi'$, where 
%$\varphi'$ is as follows. 
%For $\varphi'=\B^+\varphi$, we have  
$\Fmf^\omega\models^\assign \B^+\B^+\varphi$, by the 
inductive hypothesis and the semantics of $\B^+$. 
The remaining cases  can 
be proved in a straightforward way   using the 
inductive hypothesis. 
%For $\varphi'=\exists x\varphi$, 
\end{proof}

%~ \begin{lemma}\label{lem:aux2}
%~ For all finite traces \Fmf, all infinite traces $\Imf\in \textit{Ext}(\Fmf)$,  
%~ all assignments \assign,
%~ and all $\B^{+}$-formulas $\varphi$, 
%~ if $\Imf\models^\assign\forall x \varphi$
%~ then  $\Fmf\models^\assign \forall x\varphi$. 
%~ \end{lemma}
%~ \begin{lemma}\label{lem:aux}
%~ For all finite traces \Fmf, all infinite traces \Imf (sharing 
%~ the same domain of \Fmf),  all assignments \assign,
%~ and all $\B^{+}$-formulas $\varphi$, 
%~ if $\Fmf\models^\assign \B^{+}\varphi$ 
%~ then $\Fmf^{\omega}\models^\assign \B^{+}\varphi$.
%~ \end{lemma}

\newtheorem{claim2}{Claim} 

Recall that, given and assignment 
$\assign$ and an element $d$ of a domain $\Delta$ (of 
a finite or infinite trace), we write
 $\assign_d$ for the result of modifying $\assign$ so that 
  $x$ maps to $d$.
 
\TheoremBox*
\begin{proof}
We first show that all $\B^{+}\exists$-formulas are $\finit{}{\exists}$. 
In Claim~\ref{cl:box1} we show that all 
 $\B^{+}\exists$-formulas are $\finit{\Rightarrow}{\exists}$.
 Then, in Claim~\ref{cl:box2} we show that all 
 $\B^{+}\exists$-formulas are $\finit{\Leftarrow}{\exists}$. 
\begin{claim2}\label{cl:box1}
For all finite traces \Fmf, all assignments \assign, and
all $\B^{+}\exists$-formulas $\varphi$, if 
$\Fmf\models^\assign \varphi$ then there is $\Imf\in \textit{Ext}(\Fmf)$
such that $\Imf\models^\assign \varphi$.
\end{claim2}
\noindent\textit{Proof of Claim~\ref{cl:box1}}
We show that  $\Fmf\models^\assign \varphi$
implies $\Fmf^{\omega}\models^\assign \varphi$.
The proof is by   induction. In the base case 
we have all non-temporal $\B^{+}\exists$-formulas (Theorem~\ref{thm:boolean}).
Assume that the claim holds for $\varphi$. % and $\psi$, 
%and there is a finite trace \Fmf and an assignment $\assign$ such that 
%$\Fmf\models^\assign \varphi'$. We now argue that 
%$\Fmf^{\omega}\models^\assign \varphi'$, where $\varphi'$ is as follows.
\begin{itemize}
\item The case for  $\B^{+}\varphi$ is by Lemma~\ref{lem:aux11}.
%~ : by assumption 
%~ $\Fmf\models^\assign \B^{+}\varphi$. 
%~ This means that, for all $n\in [0,l]$,
%~ $\Fmf,n\models^\assign  \varphi$. In particular, 
%~ $\Fmf,l\models^\assign  \varphi$, 
%~ that is, $\Fmf^l\models^\assign  \varphi$.
%~ By the inductive hypothesis, $(\Fmf^l)^\omega\models^\assign  \varphi$. By definition of $(\Fmf^l)^\omega$,
%~ it follows that $(\Fmf^l)^\omega\models^\assign \B^+\varphi$.
%~ %As $\Fmf^l$ has only one time point, $\Fmf^l\models^\assign  \B^+\varphi$.
%~ As $(\Fmf^l)^\omega\models^\assign  \B^+\varphi$ and 
%~ $\Fmf\models^\assign \B^{+}\varphi$, 
%~ \textcolor{blue}{(...)}
%by Lemma~\ref{lem:aux0}, 
%$\Fmf^{\omega}\models^\assign \B^{+}\varphi$.
\item 
%For $\varphi'=\forall x\varphi$: 
%by assumption 
If $\Fmf\models^\assign \forall x\varphi$. 
This means that, for all $d\in\Delta$,
$\Fmf\models^\assign  \varphi[d]$. 
By the inductive hypothesis, for all $d\in\Delta$, $\Fmf^\omega\models^\assign  \varphi[d]$. 
So, 
$\Fmf^{\omega}\models^\assign \forall x\varphi$.
\item %For $\varphi'=\exists x\varphi$: by assumption 
If $\Fmf\models^\assign \exists x\varphi$. 
This means that there is $d\in\Delta$ such that 
$\Fmf\models^\assign  \varphi[d]$. 
By the inductive hypothesis,   $\Fmf^\omega\models^\assign  \varphi[d]$. 
This means that 
$\Fmf^{\omega}\models^\assign \exists x\varphi$.
\item The remaining cases  can 
be proved in a straightforward way   using the 
inductive hypothesis. 
\end{itemize} 
We observe that 
the problematic operator for this claim is $\B$, 
e.g., $\B\bot$ holds in a finite trace \Fmf with 
only one time point but it does not on any extension, 
in particular, not on $\Fmf^{\omega}$. This claim  
relies on the fact that the grammar rule for $\B^{+}$-formulas
does not allow the $\B$ operator. 

\medskip

%We now show that all  $\B^{+}$-formulas are $\finit{\Leftarrow}{\exists}$.
\begin{claim2}\label{cl:box2}
For all finite traces \Fmf, all assignments \assign, and
all $\B^{+}\exists$-formulas $\varphi$, if there exists $\Imf\in \textit{Ext}(\Fmf)$
such that  $\Imf\models^\assign \varphi$ then we have that 
 $\Fmf\models^\assign \varphi$.
\end{claim2}
\noindent\textit{Proof of Claim~\ref{cl:box2}}
The proof is by   induction, as in Claim~\ref{cl:box1}. 
In the base case 
we have all non-temporal $\B^{+}\exists$-formulas (Theorem~\ref{thm:boolean}).
Assume that the claim holds for $\varphi$ and $\psi$.
%The case for formulas of the form $\B^{+}\varphi$ is by Lemma~\ref{lem:aux1}
\begin{itemize}
\item For formulas of the form $\B^{+}\varphi$ the argument is as follows. 
Let $\Fmf = (\Delta, \Fmc_{n \in [0, l]})$ be  a finite trace and let 
 $\Imf$ be an element of $\textit{Ext}(\Fmf)$.
 Assume 
$\Imf\models^\assign \B^{+}\varphi$. 
%and let 
% $\Fmf = (\Delta, \Fmc_{n \in [0, l]})$  be an arbitrary element of $\textit{Pre}(\Imf)$.
If  $\Imf\models^\assign \B^{+}\varphi$ then, for all $n\in [0,\infty)$, 
$\Imf,n\models^\assign \varphi$. 
By applying the inductive hypothesis on every point in 
$[0,l]$, we have that, for all $n\in [0,l]$, 
$\Fmf,n\models^\assign \varphi$. So,
$\Fmf\models^\assign \B^{+}\varphi$.
\item The case for formulas of the form 
$\forall x\varphi$ is as follows. 
Let $\Fmf = (\Delta, \Fmc_{n \in [0, l]})$ be  a finite trace. 
 Assume that there is $\Imf\in\textit{Ext}(\Fmf)$ such that  
  $\Imf\models^\assign \forall x\varphi$. By semantics of $\forall$, 
 we have that, for all $d\in\Delta$, $\Imf\models^{\assign_d} \varphi[d]$. 
% where $\assign_d$ extends $\assign$ by mapping $x$ to $d$. 
 By applying the inductive hypothesis on every $\varphi[d]$ with $d\in\Delta$
 we have that $\Fmf\models^{\assign_d} \varphi[d]$, for all $d\in\Delta$.
 %By semantics of $\forall$, 
 So,  $\Fmf\models^\assign \forall x\varphi$.  
%The case for formulas of the form $\forall x\varphi$ is by Lemma~\ref{lem:aux2}; 
\item The case for formulas of the form 
$\exists x\varphi$ is as follows. 
Let $\Fmf = (\Delta, \Fmc_{n \in [0, l]})$ be  a finite trace.
 %
 Assume that there is $\Imf\in\textit{Ext}(\Fmf)$ such that 
  $\Imf\models^\assign \exists x\varphi$. By semantics of $\exists$, 
 there is  $d\in\Delta$ such that  $\Imf\models^{\assign_d} \varphi[d]$. 
% where $\assign_d$ extends $\assign$ by mapping $x$ to $d$. 
 By applying the inductive hypothesis, 
 we have that $\Fmf\models^{\assign_d} \varphi[d]$, for some $d\in\Delta$.
 %By semantics of $\exists$, 
 So,  $\Fmf\models^\assign \exists x\varphi$.  
\item The remaining cases are a straightforward application 
of the inductive hypothesis.
\end{itemize}

\medskip

We now show that all $\B$-formulas are $\infinit{}{\forall}$.  
In Claim~\ref{cl:box3}, we show that all $\B$-formulas 
are $\infinit{\Rightarrow}{\forall}$. 
Then, in Claim~\ref{cl:box4}, we show that all 
$\B$-formulas are $\infinit{\Leftarrow}{\forall}$. 


\begin{claim2}\label{cl:box3}
For all infinite traces \Imf, all assignments \assign, and
all $\B$-formulas $\varphi$, if $\Imf\models^\assign \varphi$
then, for all  $\Fmf\in \textit{Pre}(\Imf)$,
we have that  $\Fmf\models^\assign \varphi$. 
\end{claim2}
\noindent\textit{Proof of Claim~\ref{cl:box3}}
The proof is by   induction as in Claim~\ref{cl:box1}. 
In the base case 
we have all non-temporal $\B$-formulas (Theorem~\ref{thm:boolean}).
Assume that the claim holds for $\varphi$ and $\psi$.
\begin{itemize}
\item For formulas of the form $\B\varphi$ the argument is as follows. 
Let \Imf be  an infinite trace  such that
$\Imf\models^\assign \B\varphi$
and let 
 $\Fmf = (\Delta, \Fmc_{n \in [0, l]})$  be an arbitrary element of $\textit{Pre}(\Imf)$.
If  $\Imf\models^\assign \B\varphi$ then, for all $n\in (0,\infty)$, 
$\Imf,n\models^\assign \varphi$. 
By applying the inductive hypothesis on every point in 
$(0,l]$, we have that, for all $n\in (0,l]$, 
$\Fmf,n\models^\assign \varphi$. This means that
$\Fmf\models^\assign \B\varphi$.
 Since \Fmf was an arbitrary element of $\textit{Pre}(\Imf)$, 
 the argument holds for all  $\Fmf\in \textit{Pre}(\Imf)$. 
 %For all case here
\item The case for formulas of the form 
$\forall x\varphi$ is as follows. 
Let $\Imf  = (\Delta, \Imc_{n \in [0, \infty)})$ be  an infinite trace   
and let 
 $\Fmf$  be an arbitrary element of $\textit{Pre}(\Imf)$.
 Assume  $\Imf\models^\assign \forall x\varphi$. By semantics of $\forall$, 
 we have that, for all $d\in\Delta$, $\Imf\models^{\assign_d} \varphi[d]$.  
% where $\assign_d$ extends $\assign$ by mapping $x$ to $d$. 
 By applying the inductive hypothesis on every $\varphi[d]$ with $d\in\Delta$
 we have that $\Fmf\models^{\assign_d} \varphi[d]$, for all $d\in\Delta$.
 By semantics of $\forall$,  $\Fmf\models^\assign \forall x\varphi$. 
 As \Fmf was an arbitrary element of $\textit{Pre}(\Imf)$, 
 the argument holds for all  $\Fmf\in \textit{Pre}(\Imf)$. 
%by Lemma~\ref{lem:aux2}.  
\item The remaining cases can be proved by a straightforward application 
of the inductive hypothesis.
\end{itemize} 

\begin{claim2}\label{cl:box4}
For all infinite traces \Imf, all assignments \assign, and
all $\B$-formulas $\varphi$, if for all $\Fmf\in \textit{Pre}(\Imf)$,
  $\Fmf\models^\assign \varphi$ then  
 $\Imf\models^\assign \varphi$.
\end{claim2}
\noindent\textit{Proof of Claim~\ref{cl:box4}}
The proof is by   induction as in Claim~\ref{cl:box1}. 
In the base case 
we have all non-temporal $\B$-formulas (Theorem~\ref{thm:boolean}).
Assume that the claim holds for $\varphi$ and $\psi$.
\begin{itemize}
\item The case for formulas of the form $\B\varphi$ %(and also $\B\varphi$)
is by the semantics of $\B$ 
(since  $\Imf\not\models^\assign \B\varphi$ implies that 
there is  $\Fmf\in \textit{Pre}(\Imf)$ such that 
$\Fmf\not\models^\assign \B\varphi$ for finite traces with 
more than one time point, which contradicts the assumption). 
\item The case for formulas of the form $\forall x\varphi$ is as follows.
Let $\Imf  = (\Delta, \Imc_{n \in [0, \infty)})$ be  an infinite trace.  
%
 Assume 
  $\Fmf\models^\assign \forall x\varphi$, for all $\Fmf\in \textit{Pre}(\Imf)$.  
  By semantics of $\forall$, 
  for all $\Fmf\in \textit{Pre}(\Imf)$ and
  all $d\in\Delta$, $\Fmf\models^{\assign_d} \varphi[d]$. 
 By applying the inductive hypothesis on every $\varphi[d]$ with 
 $d\in\Delta$, 
 we obtain $\Imf\models^{\assign_d} \varphi[d]$, for all $d\in\Delta$.
 %By semantics of $\forall$, 
 So, $\Imf\models^\assign \forall x\varphi$. 
 

\item The case for formulas of the form $\varphi\vee\psi$ is as follows.
Assume that, for all $\Fmf\in \textit{Pre}(\Imf)$, $\Fmf\models^\assign \varphi\vee\psi$ and suppose to the contrary that  
 $\Imf\not\models^\assign \varphi\vee\psi$.
 Then, 
 there are $\Fmf,\Fmf'\in \textit{Pre}(\Imf)$
such that  $\Fmf\not\models^\assign \varphi$
and $\Fmf'\not\models^\assign \psi$ (otherwise we contradict the 
inductive hypothesis). 
 By definition of $\Fmf$ and $\Fmf'$, 
 either $\Fmf'$ is a prefix of $\Fmf$ or vice versa. 
 Assume w.l.o.g. that $\Fmf'$ is a prefix of $\Fmf$.
By Lemma~\ref{lem:aux1}, $\Fmf\not\models^\assign \psi$. 
Then, $\Fmf\not\models^\assign \varphi\vee\psi$,
which  contradicts the assumption that, for all $\Fmf''\in \textit{Pre}(\Imf)$, 
$\Fmf''\models^\assign \varphi\vee\psi$.
%
\item The remaining cases can be proved by a straightforward application 
of the inductive hypothesis. 
\end{itemize}
\end{proof}

%\nb{M: Delete from Th. 26 to 29?}
%
%\begin{restatable}{theorem}{TheoremFexists}\label{thm:fexists}
%	$(i)$
%		If $\p$ and $\psi$ are $\finit{\Rightarrow}{\exists}$, then 	
%		$\exists x \p$,
%		$\forall x \p$ {\color{red}{?}} \nb{M: Check $\forall$},
%		$\p \lor \psi$,
%		$\D \p$
%%		\nb{M: $\forall, \D, \Until$?}
%		are $\finit{\Rightarrow}{\exists}$;
%	$(ii)$
%		if $\p$ and $\psi$ are $\finit{\Leftarrow}{\exists}$, then 	
%		$\exists x \p$, $\forall x \p$, $\p \land \psi$, $\p \lor \psi$
%%		\nb{M: $\B$?}
%%		$\B \p$
%%		\nb{M: Add weak until $\psi \Wuntil \chi$?}
%		are $\finit{\Leftarrow}{\exists}$;
%	$(iii)$
%		if $\p$ and $\psi$ are $\finit{}{\exists}$, then 
%		$\exists x \p$, $\p \lor \psi$
%		are $\finit{}{\exists}$.
%		\nb{M: Check $\forall, \B^{+}$?}
%%		\nb{$\psi \Wuntil^{+} \chi$, $\psi \Wuntil \chi$}
%\end{restatable}
%%\TheoremFexists*
%\begin{proof}
%Let $\Fmf = (\Delta, \Fmc_{n \in [0, l]})$ be a finite trace, and $\assign$ an assignment.
%
%$(i)$
%For $\exists x \p$, suppose that
%$\Fmf \models^{\assign} \exists x \p$.
%By definition, this means
%$\Fmf \models^{\assign'} \p[d]$, for
%some $d \in \Delta$.
%Since $\p$ is $\finit{\Rightarrow}{\exists}$,
%we have:
%for some $d \in \Delta$, $\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign'} \p[d]$.
%Equivalently, 
%$\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign'} \p[d]$, for
%some $d \in \Delta$.
%That is, $\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \exists x \p$.
%
%For $\forall x \p$,
%%\nb{M: Not sure about this part! Check!}
%suppose that
%$\Fmf \models^{\assign} \forall x \p$.
%By definition,
%$\Fmf \models^{\assign'} \p[d]$, for
%all $d \in \Delta$.
%Since $\p$ is $\finit{\Rightarrow}{\exists}$,
%we have:
%for all $d \in \Delta$, $\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign'} \p[d]$.
%Suppose, towards a contradiction, that
%$\forall \Imf \in \Ext(\Fmf). \Imf \models^{\assign'} \lnot \p[\bar{d}]$, for some $\bar{d} \in \Delta$.
%Since by hypothesis $\p$ is $\finit{\Rightarrow}{\exists}$, thanks to Lemma~\ref{lemma:not} we have that $\lnot \p$ is $\finit{\Leftarrow}{\forall}$.
%Thus, from $\forall \Imf \in \Ext(\Fmf). \Imf \models^{\assign'} \lnot \p[\bar{d}]$, for some $\bar{d} \in \Delta$, we have that \nb{M: Why? The quantifier on the assignment is not in the right position} $\Fmf \models^{\assign'} \lnot \p[\bar{d}]$, for some $\bar{d} \in \Delta$.
%That is, $\Fmf \models^{\assign'} \exists x \lnot \p$, contradicting the assumption that $\Fmf \models^{\assign} \forall x \p$.
%Therefore, we have:
%$\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign'} \p[d]$, for
%all $d \in \Delta$.
%Equivalently, $\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \forall x \p$.
%
%
%
%For $\p \lor \psi$,
%suppose $\Fmf \models^{\assign} \p \lor \psi$, that is,
%$\Fmf \models^{\assign} \p$ or $\Fmf \models^{\assign} \psi$.
%By $\finit{\Rightarrow}{\exists}$, we have:
%$\exists \Imf \in \Ext(\Fmf). \Imf \mdl^{\assign} \p$ or $\exists \Imf \in \Ext(\Fmf). \Imf \mdl^{\assign} \psi$.
%Equivalently,
%$\exists \Imf \in \Ext(\Fmf). \Imf \mdl^{\assign} \p \lor \psi$.
%
%
%
%For $\D \p$, suppose $\Fmf \models^{\assign} \D \p$.
%That is,
%$\exists n \in (0, l]: \Fmf, n \mdl^{\assign} \p$.
%The previous step is equivalent to:
%$\Fmf' \mdl^{\assign} \p$,
%where
%$\Fmf' = (\Delta, (\Fmc'_{m})_{m \in [0, l - n]})$ is defined so that, for all $m \in [0, l -n]$, $\Fmc'_{m} = \Fmc_{m + n}$.
%By $\finit{\Rightarrow}{\exists}$, we have:
%$\exists \Imf' \in \Ext(\Fmf'). \Imf' \mdl^{\assign} \p$.
%This last step implies that
%$\exists n \in (0, \infty): \Imf, n \mdl^{\assign} \p$, where $\Imf = (\Delta, (\Imc_{i})_{i \in [0, \infty)})$ is defined as follows:
%$\Imc_{i} = \Fmc_{i}$, for $i \in [0, n]$, and $\Imc_{i} = \Imc'_{i}$, for $i \in (n, \infty)$.
%Thus,
%$\exists \Imf \in \Ext(\Fmf). \exists n \in (0, \infty): \Imf, n \mdl^{\assign} \p$,
%that is:
%$\exists \Imf \in \Ext(\Fmf): \Imf, \mdl^{\assign} \D \p$.
%
%
%$(ii)$
%%Suppose that $\p$ and $\psi$ are $\finit{\Leftarrow}{\exists}$.
%%For all finite traces $\Fmf = (\Delta, \Fmc_{n \in [0, l]})$, and all assignments $\assign$, we show that:
%%\[
%%\Fmf \models^{\assign} \chi \Leftarrow \exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \chi.
%%\]
%For $\exists x \p$, we have that
%$\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \exists x
%\p$ iff
%$\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign'} \p[d]$, for
%some $d \in \Delta$.  By $\finit{\Leftarrow}{\exists}$, we obtain
%$\Fmf \models^{\assign'} \p[d]$, for some $d \in \Delta$.  The
%previous step is equivalent to:
%$\Fmf \models^{\assign} \exists x \p$.
%
%For $\forall x \p$, we have $\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \forall x
%\psi$ iff $\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign'} \psi[d]$, for
%all $d \in \Delta$.
%This last step implies that, for all $d \in \Delta$,
%$\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign'} \psi[d]$.
%By $\finit{\Leftarrow}{\exists}$, we have that, for all $d \in \Delta$,
%$\Fmf \models^{\assign'} \psi[d]$.
%That is, $\Fmf \models^{\assign} \forall x \psi$.
%
%For $\p \land \psi$,
%$\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \p \land \psi$.
%This implies:
%$\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \p$ and
%$\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \psi$.  By
%$\finit{\Leftarrow}{\exists}$, we have that:
%$\Fmf \models^{\assign} \p$ and $\Fmf \models^{\assign} \psi$.
%Equivalently, $\Fmf \models^{\assign} \p \land \psi$.
%
%For $\p \lor \psi$,
%$\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \p \lor \psi$ iff
%$\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \p$ or
%$\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \psi$.  By
%$\finit{\Leftarrow}{\exists}$, we have that:
%$\Fmf \models^{\assign} \p$ or $\Fmf \models^{\assign} \psi$.
%Equivalently, $\Fmf \models^{\assign} \p \lor \psi$.
%
%%For $\B \p$, suppose
%%$\exists \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \B \p$. This means:
%%$\exists \Imf \in \Ext(\Fmf). \forall n \in (0, \infty) \colon \Imf, n
%%\models^{\assign} \p$, iff
%%$\exists \Imf \in \Ext(\Fmf). \forall n \in (0, \infty) \colon \Isf{n}
%%\models^{\assign} \p$,
%%where $\Isf{n}$ is the (infinite) suffix of $\Imf$ starting from $n$.
%%\nb{M: todo: define!}
%%This implies:
%%$\forall n \in (0, l] \colon \exists \Imf \in \Ext(\Fmf). \Isf{n}
%%\models^{\assign} \p$.  By $\finit{\Leftarrow}{\exists}$, we have:
%%$\forall n \in (0, l] \colon \Fmf \models^{\assign} \p$.
%%Equivalently, $\Fmf \models^{\assign} \B \p$.
%
%%For $\D \p$, the proof in $(i)$ works also in the other direction, under the assumption that $\p$ is $\finit{\Leftarrow}{\exists}$.
%
%$(iii)$
%It follows from the proofs of $(i)$ and $(ii)$ that, under the assumption that
%$\p$ and $\psi$ are $\finit{}{\exists}$, also $\exists x \p$, $\forall x \p$\nb{M: Check $\forall$}, $\p \lor \psi$
%%$\p \Until \psi$
%are $\finit{}{\exists}$.
%
%%All the steps in the proofs for $\exists x \p$
%%and $\p \lor \psi$ can be strengthened to `if and only if', under the assumption that $\p$ and $\psi$ are $\finit{}{\exists}$.
%
%\end{proof}
%% WRONG PROOF
%%  For all finite traces $\Fmf = (\Delta, \Fmc_{n \in [0, l]})$, every
%%  $n \in [0, l]$ and all assignments $\assign$, we show that:
%%\[
%%\Fmf, n \models^{\assign} \p \Leftarrow \exists \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \p.
%%\]
%%
%%If $\p = \exists x \psi$, we have that
%%$\exists \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \exists x
%%\psi$ iff
%%$\exists \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \psi[d]$, for
%%some $d \in \Delta$.  By $\finit{\Leftarrow}{\exists}$, we obtain
%%$\Fmf, n \models^{\assign} \psi[d]$, for some $d \in \Delta$.  The
%%previous step is equivalent to:
%%$\Fmf, n \models^{\assign} \exists x \psi$.
%%
%%If $\p = \forall x \psi$, we have
%%$\exists \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \forall x
%%\psi$ iff
%%$\exists \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \psi[d]$, for
%%all $d \in \Delta$.  This last step implies that, for all
%%$d \in \Delta$,
%%$\exists \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \psi[d]$.  By
%%$\finit{\Leftarrow}{\exists}$, we have that, for all $d \in \Delta$,
%%$\Fmf, n \models^{\assign} \psi[d]$.  Equivalently,
%%$\Fmf, n \models^{\assign} \forall x \psi$.
%%
%%
%%If $\p = \psi \land \chi$,
%%$\exists \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \psi \land
%%\chi$ iff
%%$\exists \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \psi$ and
%%$\exists \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \chi$.  By
%%$\finit{\Leftarrow}{\exists}$, we have that:
%%$\Fmf, n \models^{\assign} \psi$ and $\Fmf, n \models^{\assign} \chi$.
%%Equivalently, $\Fmf, n \models^{\assign} \psi \land \chi$.
%%
%%If $\p = \psi \lor \chi$,
%%$\exists \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \psi \lor
%%\chi$ iff
%%$\exists \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \psi$ or
%%$\exists \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \chi$.  By
%%$\finit{\Leftarrow}{\exists}$, we have that:
%%$\Fmf, n \models^{\assign} \psi$ or $\Fmf, n \models^{\assign} \chi$.
%%Equivalently, $\Fmf, n \models^{\assign} \psi \lor \chi$.
%%
%%If $\p = \B \psi$, we have that
%%$\exists \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \B \psi$, iff
%%$\exists \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \B \psi$.  The
%%previous step is equivalent to:
%%$\exists \Imf \in \Ext(\Fmf). \forall m \in (n, \infty) \colon \Imf, m
%%\models^{\assign} \psi$.  This implies:
%%$\forall m \in (n, l] \colon \exists \Imf \in \Ext(\Fmf). \Imf, m
%%\models^{\assign} \psi$.  By $\finit{\Leftarrow}{\exists}$, we have:
%%$\forall m \in (n, l] \colon \Fmf, m \models^{\assign} \psi$.
%%Equivalently, $\Fmf, n \models^{\assign} \B \psi$.
%%
%%
%%All the steps in the proofs for $\exists x \psi$
%%%$\forall x \psi$
%%and $\psi \lor \chi$ can be strengthened to `if and only if', under the assumption that $\psi$ and $\chi$ are $\finit{}{\exists}$.
%
%\begin{restatable}{theorem}{TheoremFforall}\label{thm:fforall}
%	$(i)$
%		If $\p$ and $\psi$ are $\finit{\Rightarrow}{\forall}$, then 	
%		$\exists x \p$, $\forall x \p$, $\p \land \psi$, $\p \lor \psi$
%		$\D \p$ (and thus $\D^{+} \p$)
%%		$\p \Until \psi$
%		are $\finit{\Rightarrow}{\forall}$;
%	$(ii)$
%		if $\p$ and $\psi$ are $\finit{}{\forall}$, then 
%		$\forall x \p$, 
%		\nb{M: Check $\exists, \lor, \D^{+}$?}
%		$\p \land \psi$
%		are $\finit{}{\forall}$.
%%~ %		\nb{M: Check $\exists$, prove $\Until^{+}$?}
%\end{restatable}
%%\TheoremFforall*
%\begin{proof}
%Let $\Fmf = (\Delta, \Fmc_{n \in [0, l]})$ be a finite trace, and $\assign$ an assignment.
%Moreover, for any $n \in [0, l]$, we define
%$\Fsuf{n} = (\Delta, (\Fmc^{n}_{m})_{m \in [0, l - n]})$,
%where:
%$\Fmc^{n}_{m} = \Fmc_{m + n}$, for all $m \in [0,l - n]$.
%
%$(i)$
%For $\exists x \p$, suppose
%$\Fmf \models^{\assign} \exists x \p$, iff
%$\Fmf \models^{\assign'} \p[d]$, for some $d \in \Delta$.  By
%$\finit{\Rightarrow}{\forall}$, we have: for some $d \in \Delta$,
%$\forall \Imf \in \Ext(\Fmf). \Imf \models^{\assign'} \p[d]$.  The
%previous step implies:
%$\forall \Imf \in \Ext(\Fmf). \Imf \models^{\assign'} \p[d]$, for
%some $d \in \Delta$, that is:
%$\forall \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \exists x
%\p$.
%
%For $\forall x \p$, let
%$\Fmf \models^{\assign} \forall x \p$.
%That is,
%$\Fmf \models^{\assign'} \p[d]$, for all $d \in \Delta$.  By
%$\finit{\Rightarrow}{\forall}$, we obtain: for all $d \in \Delta$,
%$\forall \Imf \in \Ext(\Fmf). \Imf \models^{\assign'} \psi[d]$.  The
%previous is equivalent to:
%$\forall \Imf \in \Ext(\Fmf). \Imf \models^{\assign'} \psi[d]$, for
%all $d \in \Delta$, iff
%$\forall \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \forall x
%\psi$.
%
%For $\p \land \psi$, assume $\Fmf \models^{\assign} \p \land \psi$,
%iff $\Fmf \models^{\assign} \p$ and
%$\Fmf \models^{\assign} \psi$.  By $\finit{\Rightarrow}{\forall}$,
%this implies:
%$\forall \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \p$ and
%$\forall \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \psi$.
%Equivalently,
%$\forall \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \p \land
%\psi$.
%
%For $\p \lor \psi$, let
%$\Fmf \models^{\assign} \p \lor \psi$, iff
%$\Fmf \models^{\assign} \p$ or $\Fmf \models^{\assign} \psi$.
%That is, by $\finit{\Rightarrow}{\forall}$,
%$\forall \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \p$ or
%$\forall \Imf \in \Ext(\Fmf).\Imf \models^{\assign} \psi$.  This
%implies that
%$\forall \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \p \lor
%\psi$.
%
%For $\D \p$, let
%$\Fmf \models^{\assign} \D \p$, iff
%$\exists n \in (0, l] \colon \Fmf, n \models^{\assign} \p$.
%The previous step is equivalent to:
%$\exists n \in (0, l] \colon \Fsuf{n} \models^{\assign} \p$.
%By $\finit{\Rightarrow}{\forall}$, we have:
%$\exists n \in (0, l] \colon \forall \Imf \in \Ext(\Fsuf{n}). \Imf \models^{\assign} \psi$.
%This implies that
%$\forall \Imf \in \Ext(\Fmf). \exists n \in (0, \infty) \colon \Imf, n \models^{\assign} \psi$.
%%(the converse is not true).
%Equivalently, 
%$\forall \Imf \in \Ext(\Fmf). \Imf \models^{\assign} \D \psi$.
%
%
%
%%If $\p = \D \psi$,
%%$\Fmf, n \models^{\assign} \D \psi$
%%iff
%%$\exists m \in (n, l] \colon \Fmf, m \models^{\assign} \psi$.
%%As a consequence of $\finit{\Rightarrow}{\forall}$, we have:
%%$\exists m \in (n, l] \colon \forall \Imf \in \Ext(\Fmf). \Imf, m \models^{\assign} \psi$.
%%This implies that
%%$\forall \Imf \in \Ext(\Fmf). \exists m \in (n, \infty) \colon \Imf, m \models^{\assign} \psi$
%%(the converse is not true).
%%Equivalently, 
%%$\forall \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \D \psi$.
%
%%If $\p = \psi \Until \chi$,
%%$\Fmf, n \models^{\assign} \psi \Until \chi$ iff
%%$\exists m \in (n, l] \colon \Fmf, m \models^{\assign} \chi$ and
%%$\forall i \in (m, n) \colon \Fmf, i \models^{\assign} \psi$.  As a
%%consequence of $\finit{\Rightarrow}{\forall}$, we have:
%%$\exists m \in (n, l] \colon \forall \Imf \in \Ext(\Fmf). \Imf, m
%%\models^{\assign} \chi$ and
%%$\forall i \in (m, n) \colon \forall \Imf \in \Ext(\Fmf). \Imf, i
%%\models^{\assign} \psi$.  This implies that
%%$\forall \Imf \in \Ext(\Fmf). \exists m \in (n, \infty) \colon \Imf, m
%%\models^{\assign} \chi$ and
%%$\forall \Imf \in \Ext(\Fmf).\forall i \in (m, n) \colon \Imf, i
%%\models^{\assign} \psi$.  Equivalently,
%%$\forall \Imf \in \Ext(\Fmf). \Imf, n \models^{\assign} \psi \Until
%%\chi$.
%
%$(ii)$
%All the steps in the proofs for $\forall x \p$ and $\p \land \psi$ can be strengthened to `if and only if', under the assumption that $\p$ and $\psi$ are $\finit{}{\forall}$.
%\end{proof}
%
%\begin{restatable}{theorem}{TheoremIexists}\label{thm:iexists}
%	$(i)$
%		If $\p$ and $\psi$ are $\infinit{\Rightarrow}{\exists}$, then 	
%		$\exists x \p$,
%		$\forall x \p$ {\color{red}{?}} \nb{M: Delete $\forall$?},
%		$\p \lor \psi$,
%		$\D \p$
%		(and thus $\D^{+} \p$)
%%		$\p \Until \psi$
%		are $\infinit{\Rightarrow}{\exists}$;
%	$(ii)$
%		if $\p$ and $\chi$ are $\infinit{\Leftarrow}{\exists}$, then 	
%		$\exists x \p$, $\forall x \p$, $\p \land \psi$, $\p \lor \psi$,
%		$\D \p$
%		(and thus $\D^{+} \p$)
%%		$\p \Until \chi$
%		are $\infinit{\Leftarrow}{\exists}$;
%	$(iii)$
%		if $\p$ and $\psi$ are $\infinit{}{\exists}$, then 
%		$\exists x \p$,
%%		$\forall x \psi$,
%%		$\psi \land \chi$, 
%%		\nb{M: Checking my notes $\psi \land \chi$}
%		$\p \lor \psi$,
%		$\D \p$
%		(and thus $\D^{+} \p$)
%%		$\p \Until \psi$
%%		\nb{M: check $\Until$ (my notes) and $\forall$ (counterex)}
%		are $\infinit{}{\exists}$.
%\end{restatable}
%
%%\TheoremIexists*
%\begin{proof}
%Let $\Imf = (\Delta, \Imc_{n \in [0, \infty]})$ be an infinite trace, and $\assign$ an assignment.
%Moreover, for any $n \in \Nbb$, we define
%$\Isf{n} = (\Delta, (\Imc^{n}_{m})_{m \in [0, \infty)})$,
%where:
%$\Imc^{n}_{m} = \Imc_{m + n}$, for all $m \in [0, \infty)$.
%
%
%
%$(i)$
%For $\exists x \p$,
%suppose $\Imf \mdl^{\assign} \exists x \p$.
%This means that, for some $d \in \Delta$,
%$\Imf \mdl^{\assign'} \p[d]$.
%By $\infinit{\Rightarrow}{\exists}$,
%for some $d \in \Delta$,
%$\exists \Fmf \in \Pre(\Imf).\Fmf \mdl^{\assign'} \p[d]$.
%Equivalently,
%$\exists \Fmf \in \Pre(\Imf).\Fmf \mdl^{\assign'} \p[d]$, for some $d \in \Delta$,
%that is,
%$\exists \Fmf \in \Pre(\Imf).\Fmf \mdl^{\assign} \exists x \p$.
%
%For $\forall x \p$, cf. Th.~18(i) \ldots \nb{M: Check/Delete! Discuss counterxample}
%
%For $\p \lor \psi$,
%let $\Imf \mdl^{\assign} \p \lor \psi$.
%That is, $\Imf \mdl^{\assign} \p$ or $\Imf \mdl^{\assign} \p \lor \psi$.
%By $\infinit{\Rightarrow}{\exists}$, we have:
%$\exists \Fmf \in \Pre(\Imf).\Fmf \mdl^{\assign} \p$ or $\exists \Fmf \in \Pre(\Imf).\Fmf \mdl^{\assign} \psi$.
%The previous step is equivalent to:
%$\exists \Fmf \in \Pre(\Imf).\Fmf \mdl^{\assign} \p \lor \psi$.
%
%
%For $\D \p$,
%\nb{M: Check}
%assume that $\Imf \mdl^{\assign} \D \p$.
%By definition, this is equivalent to:
%$\exists n \in (0, \infty): \Imf, n \mdl^{\assign} \p$,
%iff
%$\exists n \in (0, \infty): \Isf{n} \mdl^{\assign} \p$.
%By $\infinit{\Rightarrow}{\exists}$, we obtain:
%$\exists n \in (0, \infty): \exists \Fmf' \in \Pre(\Isf{n}).\Fmf' \mdl^{\assign} \p$.
%Equivalently,
%$\exists n \in (0, \infty): \exists \Fmf \in \Pre(\Imf).\Fmf, n \mdl^{\assign} \p$.
%This means that
%$\exists \Fmf \in \Pre(\Imf).\exists n \in (0, l]: \Fmf, n \mdl^{\assign} \p$, with $l$ being the last time point of $\Fmf$.
%In conclusion,
%$\exists \Fmf \in \Pre(\Imf). \Fmf \mdl^{\assign} \D \p$.
%
%%We show the following claim. 
%%Suppose that, for all infinite traces $\Imf$, all $n \in \Nbb$ and all assignments $\assign$, that:
%%\[
%%\Imf, n \models^{\assign} \chi \Rightarrow \exists \Fmf \in \Prel{n}(\Imf). \Fmf, n \models^{\assign} \chi,
%%\]
%%where
%%$\Prel{n}(\Imf) = \{ \Fmf = (\Delta, (\Fmc)_{m \in [0, l]}) \mid l \geq n \text{ and } \Imf = \Fmf \cdot \Imf', \text{ for some } $\Imf'$ \}$.
%%Then,
%%If $\chi = \exists x \psi$, we have
%%
%%For all infinite traces $\Imf$, all $n \in \Nbb$ and all assignments $\assign$, we show that:
%%\[
%%\Imf, n \models^{\assign} \p \Leftarrow \exists \Fmf \in \Prel{n}(\Imf). \Fmf, n \models^{\assign} \p.
%%\]
%%where
%%$\Prel{n}(\Imf) = \{ \Fmf = (\Delta, (\Fmc)_{m \in [0, l]}) \mid l \geq n \text{ and } \Imf = \Fmf \cdot \Imf', \text{ for some } $\Imf'$ \}$.
%
%$(ii)$
%For $\exists x \p$, we have
%$\exists \Fmf \in \Pre(\Imf). \Fmf \models^{\assign} \exists x \p$
%iff
%$\exists \Fmf \in \Pre(\Imf). \Fmf \models^{\assign'} \p[d]$,
%for some $d \in \Delta$.
%By $\infinit{\Leftarrow}{\exists}$,
%we obtain:
%$\Imf \models^{\assign'} \p[d]$, for some $d \in \Delta$,
%iff
%$\Imf \models^{\assign} \exists x \p$.
%
%
%For $\forall x \p$,
%$\exists \Fmf \in \Pre(\Imf). \Fmf \models^{\assign} \forall x \p$
%iff
%$\exists \Fmf \in \Pre(\Imf). \Fmf \models^{\assign'} \p[d]$,
%for all $d \in \Delta$.
%The previous step implies that,
%for all $d \in \Delta$,
%$\exists \Fmf \in \Pre(\Imf). \Fmf \models^{\assign'} \p[d]$.
%By $\infinit{\Leftarrow}{\exists}$,
%we have:
%for all $d \in \Delta$,
%$\Imf \models^{\assign'} \p[d]$.
%Equivalently,
%$\Imf \models^{\assign} \forall x \p$.
%
%For $\p \land \psi$,
%%\nb{M: Checking my notes}
%we have that
%$\exists \Fmf \in \Pre(\Imf). \Fmf \models^{\assign} \p \land \psi$ iff
%$\exists \Fmf \in \Pre(\Imf). \Fmf \models^{\assign} \p$ and
%$\exists \Fmf \in \Pre(\Imf). \Fmf \models^{\assign} \psi$.  By
%$\infinit{\Leftarrow}{\exists}$, we have:
%$\Imf \models^{\assign} \p$ and $\Imf \models^{\assign} \psi$,
%that is $\Imf \models^{\assign} \p \land \psi$.
%
%For $\p \lor \psi$,
%we have that
%$\exists \Fmf \in \Pre(\Imf). \Fmf \models^{\assign} \p \lor \psi$
%iff
%$\exists \Fmf \in \Pre(\Imf). \Fmf \models^{\assign} \p$ or $\exists \Fmf \in \Pre(\Imf). \Fmf \models^{\assign} \psi$.
%By $\infinit{\Leftarrow}{\exists}$,
%we have:
%$\Imf \models^{\assign} \p$ or $\Imf \models^{\assign} \psi$,
%that is
%$\Imf \models^{\assign} \p \lor \psi$.
%
%
%
%For $\D \p$,
%\nb{M: Check!}
%suppose
%$\exists \Fmf \in \Pre(\Imf). \Fmf \models^{\assign} \D \p$.
%This means
%$\exists \Fmf \in \Pre(\Imf). \exists n \in (0, l]: \Fmf, n \models^{\assign} \p$,
%where $l$ is the last time point of $\Fmf$, iff
%$\exists n \in (0, \infty): \exists \Fmf \in \Pre(\Imf). \Fmf, n \models^{\assign} \p$.
%The previous step is equivalent to:
%$\exists n \in (0, \infty): \exists \Fmf' \in \Pre(\Isf{n}). \Fmf' \models^{\assign} \p$.
%By $\infinit{\Leftarrow}{\exists}$, we have:
%$\exists n \in (0, \infty): \Isf{n} \models^{\assign} \p$, iff
%$\exists n \in (0, \infty): \Imf, n \models^{\assign} \p$.
%Equivalently,
%$\Imf \models^{\assign} \D \p$.
%
%
%
%%If $\p = \D \psi$,
%%$\exists \Fmf \in \Prel{n}(\Imf). \Fmf, n \models^{\assign} \D \psi$
%%iff
%%$\exists \Fmf \in \Prel{n}(\Imf).\exists m \in (n, l] \colon \Fmf, m
%%\models^{\assign} \psi$.  This last step is equivalent to:
%%$\exists m \in (n, \infty) \colon \exists \Fmf \in
%%\Prel{n}(\Imf). \Fmf, m \models^{\assign} \psi$.  Using
%%$\infinit{\Leftarrow}{\exists}$, we have:
%%$\exists m \in (n, \infty) \colon \Imf, m \models^{\assign} \psi$,
%%that is $\Imf, n \models^{\assign} \D \psi$.
%%
%%If $\p = \psi \Until \chi$, we have that:
%%$\exists \Fmf \in \Pre(\Imf). \Fmf, n \models^{\assign} \psi \Until
%%\chi$ iff
%%$\exists \Fmf \in \Pre(\Imf).  \exists m \in (n, l] \colon \Fmf, m
%%\models^{\assign} \chi$ and
%%$\forall i \in (m, n) \colon \Fmf, i \models^{\assign}$.  This last
%%step implies (but is not implied by):
%%$\exists \Fmf \in \Prel(\Imf).\exists m \in (n, l] \colon \Fmf, m
%%\models^{\assign} \chi$ and
%%$\exists \Fmf \in \Prel(\Imf).\forall i \in (m, n) \colon \Fmf, i
%%\models^{\assign} \psi$, and in turn:
%%$\exists m \in (n, \infty) \colon \exists \Fmf \in
%%\Prel{n}(\Imf). \Fmf, m \models^{\assign} \chi$ and
%%$\forall i \in (m, n) \colon \exists \Fmf \in \Prel{n}(\Imf). \Fmf, i
%%\models^{\assign} \psi$.  As a consequence of
%%$\infinit{\Leftarrow}{\exists}$, we have:
%%$\exists m \in (n, \infty) \colon \Imf, m \models^{\assign} \chi$ and
%%$\forall i \in (m, n) \colon \Imf, i \models^{\assign} \psi$.
%%Equivalently, $\Imf, n \models^{\assign} \psi \Until \chi$.
%
%$(iii)$
%It follows from the proofs of $(i)$ and $(ii)$ that, under the assumption that
%$\p$ and $\psi$ are $\infinit{}{\exists}$, also $\exists x \p$, $\p \lor \psi$, $\D \p$
%%$\p \Until \psi$
%are $\infinit{}{\exists}$.
%
%%All the steps in the proofs for $\exists x \psi$, $\psi \lor \chi$ and
%%$\D \psi$ can be strengthened to `if and only if', under the
%%assumption that $\psi$ and $\chi$ are $\infinit{}{\exists}$.
%\end{proof}
%
%\begin{restatable}{theorem}{TheoremIforall}\label{thm:iforall}
%	$(i)$
%		If $\p$ and $\psi$ are $\infinit{\Rightarrow}{\forall}$, then 	
%		$\exists x \p$, $\forall x \p$, $\p \land \psi$, $\p \lor \psi$,
%		$\B \p$
%		(and thus $\B^{+} \p$)
%%		\nb{M: Add weak until $\psi \Wuntil \chi$?}
%		are $\infinit{\Rightarrow}{\forall}$;
%	$(ii)$
%		if $\p$ and $\psi$ are $\infinit{}{\forall}$, then 
%		\nb{M: Check $\exists, \lor$}
%%		$\exists x \psi$,
%		$\forall x \p$, $\p \land \psi$,
%%		$\psi \lor \chi$,
%%		\nb{M: Checking my notes $\psi \lor \chi$}
%		$\B \p$
%		(and thus $\B^{+} \p$)
%		are $\infinit{}{\forall}$.
%%		\nb{M: Check $\exists$}
%\end{restatable}
%%\TheoremIforall*
%\begin{proof}
%
%Let $\Imf = (\Delta, \Imc_{n \in [0, \infty]})$ be an infinite trace, and $\assign$ an assignment.
%Moreover, for any $n \in \Nbb$, let
%$\Isf{n} = (\Delta, (\Imc^{n}_{m})_{m \in [0, \infty)})$,
%be the infinite trace such that:
%$\Imc^{n}_{m} = \Imc_{m + n}$, for all $m \in [0, \infty)$.
%
%
%%For all infinite traces $\Imf$, all $n \in \Nbb$ and all assignments $\assign$, we show that:
%%\[
%%\Imf, n \models^{\assign} \p \Rightarrow \forall \Fmf \in \Prel{n}(\Imf). \Fmf, n \models^{\assign} \p.
%%\]
%%where
%%$\Prel{n}(\Imf) = \{ \Fmf = (\Delta, (\Fmc)_{m \in [0, l]}) \mid l \geq n \text{ and } \Imf = \Fmf \cdot \Imf', \text{ for some } $\Imf'$ \}$.
%
%$(i)$
%For $\exists x \p$,
%let
%$\Imf \models^{\assign} \exists x \p$,
%iff,
%for some $d \in \Delta$,
%$\Imf \models^{\assign'} \p[d]$.
%By $\infinit{\Rightarrow}{\forall}$,
%we have:
%for some $d \in \Delta$,
%$\forall \Fmf \in \Pre(\Imf). \Fmf \models^{\assign'} \p[d]$.
%In turn, this implies
%$\forall \Fmf \in \Pre(\Imf). \Fmf \models^{\assign} \exists x \p$.
%
%
%For $\forall x \p$, suppose $\Imf \models^{\assign} \forall x \p$.
%That is, for all $d \in \Delta$, $\Imf \models^{\assign'} \p[d]$.  By
%$\infinit{\Rightarrow}{\forall}$, we have that, for all
%$d \in \Delta$,
%$\forall \Fmf \in \Pre(\Imf). \Fmf \models^{\assign'} \p[d]$.  This is
%equivalent to:
%$\forall \Fmf \in \Pre(\Imf). \Fmf \models^{\assign'} \p[d]$, for all
%$d \in \Delta$, iff
%$\forall \Fmf \in \Pre(\Imf). \Fmf \models^{\assign} \forall x
%\p$.
%
%
%For $\p \land \psi$, assume
%$\Imf \models^{\assign} \p \land \psi$, iff
%$\Imf \models^{\assign} \p$ and $\Imf \models^{\assign} \psi$.
%By $\infinit{\Rightarrow}{\forall}$, it follows that
%$\forall \Fmf \in \Pre(\Imf). \Fmf \models^{\assign} \p$ and
%$\forall \Fmf \in \Pre(\Imf). \Fmf \models^{\assign} \psi$.
%Equivalently,
%$\forall \Fmf \in \Pre(\Imf). \Fmf \models^{\assign} \p \land
%\psi$.
%
%For $\p \lor \psi$, let
%$\Imf \models^{\assign} \p \lor \psi$, iff
%$\Imf \models^{\assign} \p$ or $\Imf \models^{\assign} \psi$.
%By $\infinit{\Rightarrow}{\forall}$, this implies
%$\forall \Fmf \in \Pre(\Imf). \Fmf \models^{\assign} \p$ or
%$\forall \Fmf \in \Pre(\Imf). \Fmf \models^{\assign} \psi$.
%From this we obtain:
%$\forall \Fmf \in \Pre(\Imf). \Fmf \models^{\assign} \p \lor
%\psi$.
%
%For $\B \p$,
%\nb{M: Check}
%suppose $\Imf \models^{\assign} \B \p$.
%By definition, this is equivalent to:
%$\forall n \in (0, \infty) \colon \Imf, n \models^{\assign} \p$.
%That is,
%$\forall n \in (0, \infty) \colon \Isf{n} \models^{\assign} \p$.
%Since $\p$ is
%$\infinit{\Rightarrow}{\forall}$, we have that
%$\forall n \in (0, \infty) \colon \forall \Fmf' \in \Pre(\Isf{n}).
%\Fmf' \models^{\assign} \p$.
%Equivalently,
%$\forall \Fmf \in \Pre(\Imf): \forall n \in (0, l] \colon
%\Fmf, n \models^{\assign} \psi$, where $l$ is the last time point of $\Fmf$.
%This means:
%$\forall \Fmf \in \Pre(\Imf): \Fmf \models^{\assign} \B \psi$
%
%
%$(ii)$
%All the steps in the proofs for $\forall x \p$, $\p \land \psi$, and $\B \p$
%%and $\B \psi$
%can be strengthened to `if and only if', under the assumption that $\p$ and $\psi$ are $\infinit{}{\forall}$.
%\end{proof}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proofs for Section~\ref{sec:appl}}
%`Applications'
\label{sec:proofappl}
%\nb{M: Rephrased all the proofs, check!}

\subsection{Planning}

For the proofs of the next theorems, we will use the following definitions.
Let $\Sigma$ be a finite subset of $\textsf{N}_{\textsf{P}}$.  
Assume w.l.o.g. that the $\QTLfr{f}{}{}$ formulas we mention in this subsection 
have predicates in $\Sigma$, and that $\Sigma$ contains the end of time predicate $E$.
Given an infinite trace
$\Imf$, the \emph{$\Sigma$-reduct of} $\Imf$
is the infinite trace $\reduct$ coinciding with $\Imf$ on $\Sigma$ and
such that  $X^{\Imc_{{n}\mid_{\Sigma}}} = \eset$, for $X \not \in \Sigma$ and 
$n \in [0, \infty)$.
%~\cite{KonEtAl}.


\begin{restatable}{lemma}{LemmaEndChar}\label{lemma:endchar}
  For every infinite trace $\Imf$, $\Imf \mdl \chi_{f}$ iff
  $\reduct = \FEmfC$, for some finite trace $\Fmf$.
  % \nb{M: Added}O: ok thanks
  % For every infinite trace $\Imf$, $\Imf \mdl \chi_{f}$ iff $\Imf$ is
  % of the form $\FEmf$, for some finite trace $\Fmf$. %\nb{M: Added}O: ok thanks
\end{restatable}
%\LemmaEndChar*
\begin{proof}
%Given a finite trace \Fmf, we may write $\len{\Fmf}$ to denote its \emph{length},
%i.e., $\len{\Fmf} = |(\Fmc_{0}, . . . , \Fmc_{l})| = l + 1$.
($\Leftarrow$) 
If $\reduct = \FEmfC$, 
by Lemma~\ref{lemma:finchar},
$\FEmf \mdl \psif$.
%Thus, in particular,
%$\FEmf \mdl \psi_{f_{2}}$, so that $E^{\FEmc_{n}} = \emptyset$, for all $n \in [0, l]$, and  $E^{\FEmc_{n}} = \Delta$,  for all $n \in [l + 1, \infty)$, where $l$ is the last time point of $\Fmf$.
Moreover, where $l$ is the last time point of $\Fmf$, we have by definition:
for all $n \in [0, l]$, $E^{\FEmc_{n}} = \emptyset$;
for all $n \in [l + 1, \infty)$, $E^{\FEmc_{n}} = \Delta$,
and for every $P \in \NPr \setminus \{E\}$, $P^{\FEmc_{n}} = \eset$.
Thus, for all $n \in (0, \infty)$, for all objects $d$ and all tuples of objects $\bar{d}$ in $\Delta$, we have:
 if $d \in E^{\FEmc_{n}}$, then
 $(d, \bar{d}) \notin P$, for all $P \in \Sigma \setminus \{ E \}$.
Therefore, $\FEmf \mdl \chi_{f_{1}}$, and hence $\FEmf \mdl \chi_{f}$.

($\Rightarrow$) Suppose $\Imf \mdl \chi_{f}$. Since in particular it 
satisfies $\psi_{f}$, by Lemma~\ref{lemma:finchar}, we have that 
$\Imf = \FEImf'$, for some finite trace $\Fmf = (\Delta, (\Fmc_{n})_{n \in [0, l]})$ and some infinite trace $\Imf'$. Thus:
	\[
		E^{\FImc'_{n}} =
			\begin{cases}
				\emptyset, & \text{for all $n \in [0, l]$} \\
				\Delta, & \text{for all } n \in [l + 1, \infty) \\
			\end{cases}
	\]
Since $\Imf \mdl \chi_{f_{1}}$, for all $n \in [l + 1, \infty)$, for all objects $d$ and all tuples of objects $\bar{d}$ in $\Delta$, we have that:
if $d \in E^{\FEmc_{n}} = \Delta$, then $(d, \bar{d}) \notin P$, for all $P \in \Sigma \setminus \{ E \}$.
This is equivalent to $P^{\I_{n}} = \eset$, for all $P \in \Sigma \setminus \{ E \}$.
Therefore, we have that $\reduct = \FEmf$.
\end{proof}



%
\begin{restatable}{lemma}{LemmaEndExtChar}\label{lemma:endextchar}
  Let $\p$ be a $\QTLfr{}{}{}$ formula, $\Fmf$ a finite trace, and $\assign$ an assignment. We have that: $\Fmf \mdl^{\assign} \p \text{ iff \,} \FEmfC \mdl^{\assign} \p\tr$.
\end{restatable}
%\LemmaEndExtChar*
\begin{proof}
By definition of $\FEmf$ and as a consequence of Lemma~\ref{lemma:finextchar}.
\end{proof}



\TheorInsDegEtAlChar*
\begin{proof}
$(\Rightarrow)$ Assume that $\p$ is insensitive. We want to 
prove that, for every infinite trace $\Imf$ and all assignments $\assign$, if $\Imf \mdl^{\assign} \chi_{f}$, then 
$\Imf \mdl^{\assign} \p \leftrightarrow \p\tr$. Suppose $\Imf \mdl^{\assign} \chi_{f}$. 
By Lemma~\ref{lemma:endchar}, $\reduct = \FEmf$, for a finite trace $\Fmf$. 
Moreover, thanks to Lemma~\ref{lemma:endextchar}, $\Fmf \mdl^{\assign} \p$ if and only if $\FEmf \mdl^{\assign} \p\tr$. 
Since $\p$ is by hypothesis insensitive, for every finite 
trace $\Fmf$ and all assignments $\assign$, $\Fmf \mdl^{\assign} \p$ if and only if $\FEmf \mdl^{\assign} \p$.
Thus, 
$\FEmf \mdl^{\assign} \p$ if and only if $\FEmf \mdl^{\assign} \p\tr$.
That is, $\FEmf \mdl^{\assign} \p \leftrightarrow \p\tr$, 
and therefore $\Imf \mdl \p \leftrightarrow \p\tr$ (since all the predicates occurring in $\p,\p\tr$ are in $\Sigma$).

$(\Leftarrow)$ Assume that $\chi_{f} \mdl \p \leftrightarrow \p\tr$. By Lemma~\ref{lemma:endchar}, 
for every infinite trace $\Imf$ and every assignment $\assign$, $\Imf \mdl^{\assign} \chi_{f}$ means that $\reduct = \FEmf$, 
for a finite trace $\Fmf$. Given our assumption, this implies $\FEmf \mdl^{\assign} \p \leftrightarrow \p\tr$, 
that is $\FEmf \mdl^{\assign} \p$ if and only if $\FEmf \mdl^{\assign} \p\tr$, for all assignments ${\assign}$. By Lemma~\ref{lemma:endextchar}, $\FEmf \mdl^{\assign} \p\tr$ 
if and only if $\Fmf \mdl^{\assign} \p$. In conclusion, we obtain that, for all assignments ${\assign}$, $\FEmf \mdl^{\assign} \p$ if and only if $\Fmf \mdl^{\assign} \p$, 
meaning that $\p$ is insensitive.
\end{proof}



\TheorInsDegEtAlPres*
\begin{proof}
Let $\Fmf$ be a finite trace and $\assign$ be an assignment.
For $\lnot \p$, we have that 
$\Fmf \mdl^{\assign} \lnot \p$ iff 
$\Fmf \not \mdl^{\assign} \p$.
Since $\p$ is insensitive by hypothesis, 
this means that $\FEmf \not \mdl^{\assign} \p$.
Therefore, $\lnot \p$ is insensitive as well.
For $\exists x \p$, we have that 
$\Fmf \mdl^{\assign} \exists x \p$ iff 
$\Fmf \mdl^{\assign'} \p[d]$, for some $d \in \Delta$.
Given that $\p$ is insensitive, 
this is equivalent to $\FEmf \mdl^{\assign'} \p[d]$, for some $d \in \Delta$.
That is, $\FEmf \mdl^{\assign} \exists x \p$, and so $\exists x \p$ is insensitive.
For $\p \land \psi$, we have that
$\Fmf \mdl^{\assign} \p \land \psi$ is equivalent to
$\Fmf \mdl^{\assign} \p$ and $\Fmf \mdl^{\assign} \psi$.
Since both $\p$ and $\psi$ are assumed to be insensitive, the previous step is equivalent to:
$\FEmf \mdl^{\assign} \p$ and $\FEmf \mdl^{\assign} \psi$,
i.e.,
$\FEmf \mdl^{\assign} \p \land \psi$.
\end{proof}


\Theoreminsonlyif*
\begin{proof}
The result can be seen as a
consequence of Theorem~\ref{theor:inschar}. 
We provide also a direct proof.
Given a finite trace $\Fmf$ and an assignment $\assign$, if $\Fmf \models^{\assign} \p$ then, as $\p$ is insensitive, $\FEmf \models^{\assign} \p$.
By assumption, $\equivinf{\p}{\psi}$, so $\FEmf \models^{\assign} \psi$.
As $\psi$ is insensitive, $\FEmf \models^{\assign} \psi$ implies $\Fmf \models^{\assign} \psi$.
The converse direction is obtained by swapping $\p$ and $\psi$. 
\end{proof}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%OLD VERSION I2 AND I2 PROOFS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\LemmaEndChar*
%\begin{proof} %\nb{O: changed the proof}
%%\nb{O:moved, small changes for spacing}
%%The function
%%\textit{len} associates to every finite trace $\Fmf$ its \emph{length},
%%i.e., $\textit{len}(\Fmf) = |(\Fmc_{0}, . . . , \Fmc_{l})| = l + 1$.
%Given a finite trace \Fmf, we may write $\len{\Fmf}$ to denote its \emph{length},
%i.e., $\len{\Fmf} = |(\Fmc_{0}, . . . , \Fmc_{l})| = l + 1$.
%%\nb{M: Added}
%%We say that an infinite trace $\Imf$ \emph{is of the form} $\FEmf$, for some finite trace $\Fmf$, if $\Imf_{\mid_{\Sigma(\chi_{f})}}=\FEmf$.
%($\Leftarrow$) 
%If $\reduct = \FEmf$, 
%% \nb{M: Changed with $\reduct$}
%by Lemma~\ref{lemma:finchar},
%%If $\Imf$ is of the form $\FEmf$, by Lemma~\ref{lemma:finchar},
%$\FEmf \mdl \psif$.
%Moreover, by definition, for all $n \geq \len{\Fmf}$:
%%\begin{itemize} 
%%\item[] 
%(i) for all $A \in \NC\setminus \{E\}$, $A^{\FEmc_{n}} = \eset$ and 
%%\item [] 
%(ii)  for all 
%$R \in \NR$, $R^{\FEmc_{n}} = \eset$.
%%\end{itemize}
%By (i), for all $n \geq \len{\Fmf}$:
%$(\bigsqcap_{A \in \Sigma\setminus \{E\}} \!\! \lnot A)^{\FEmc_{n}} = \Delta$. 
%Therefore, for all $n \geq 0$, we have $E^{\FEmc_{n}} \subseteq (\bigsqcap_{A 
%\in \Sigma\setminus \{E\}} \!\! \lnot A)^{\FEmc_{n}}$. Hence, $\FEmf \mdl \chi_{f_{1}}$.
%Similarly, concerning (ii), we have that for all $n \geq \len{\Fmf}$:
%$(\bigsqcap_{R \in \Sigma} \!\! \lnot \exists R. \top)^{\FEmc_{n}} = \Delta$
%and thus, for all $n \geq 0$, $E^{\FEmc_{n}} \sbs (\bigsqcap_{R \in \Sigma} 
%\!\! \lnot \exists R. \top)^{\FEmc_{n}}$, that is $\FEmf \mdl \chi_{f_{2}}$.
%Thus, $\FEmf \mdl \chi_{f}$.
%
%($\Rightarrow$) Suppose $\Imf \mdl \chi_{f}$. Since in particular it 
%satisfies $\psi_{f}$, by Lemma~\ref{lemma:finchar} it is of the form 
%$\FImf'$, and thus there is a $l = \len{\Fmf} - 1$ such that 
%	\[
%		E^{\FImc'_{n}} =
%			\begin{cases}
%				\emptyset, & \text{for all $n \in [0, l]$} \\
%				\Delta, & \text{for all } n \in [l + 1, \infty) \\
%			\end{cases}
%	\]
%Since $\Imf \mdl \chi_{f_{1}}$, we have that for all $n > l$, $E^{\I_{n}} = 
%\Delta \sbs (\bigsqcap_{A \in \Sigma\setminus \{E\}} \!\! \lnot A)^{\I_{n}}$, 
%which is equivalent to $A^{\I_{n}} = \eset$, for all $A \in \Sigma\setminus \{E\}$. Similarly, 
%given that $\Imf \mdl \chi_{f_{2}}$, for all $n > l$, $E^{\I_{n}} = \Delta \sbs 
%(\bigsqcap_{R \in \Sigma} \!\! \lnot \exists R. \top)^{\I_{n}}$, that is 
%$R^{\I_{n}} = \eset$, for every $R \in \Sigma$. Therefore, we have that $\reduct = \FEmf$.
%%\nb{M: Changed with $\reduct$}
%\end{proof}
%
%
%\LemmaEndExtChar*
%\begin{proof}
%By definition of $\FEmf$ and as a consequence of Lemma~\ref{lemma:finextchar}.
%\end{proof}
%
%
%\TheorInsDegEtAlChar*
%\begin{proof}
%Let $C$ be a $\TALCf$ concept.
%$(\Rightarrow)$ Suppose that $C$ is insensitive~\ref{ins:degetal}. 
%We want to prove that, for every infinite trace $\Imf$, if $\Imf \mdl \chi_{f}$, then $\Imf \mdl C \eqv C\tr$. Suppose $\Imf \mdl \chi_{f}$. 
%%\nb{M: Changed with $\reduct$} O: thanks
%By Lemma~\ref{lemma:endchar}, $\reduct = \FEmf$, for some finite trace $\Fmf$. 
%Thanks to Lemma~\ref{lemma:endextchar}, and as a consequence of~\eqref{eq:conc} in Lemma~\ref{lemma:finextchar}, we have that for all finite traces $\Fmf$, $d \in (C)^{\Fmc_{0}}$ iff $d \in (C\tr)^{\FEmc_{0}}$, for every $d \in \Delta$. 
%Since $C$ is by hypothesis insensitive~\ref{ins:degetal}, for 
%every finite trace $\Fmf$, $d \in (C)^{\Fmc_{0}}$ iff $d \in (C)^{\FEmc_{0}}$. 
%Therefore, for every finite trace $\Fmf$ and every $d \in \Delta$, 
%$d \in (C)^{\FEmc_{0}}$ iff $d \in (C\tr)^{\FEmc_{0}}$. Hence, 
%$\FEmf \mdl C \eqv C\tr$, and therefore $\Imf \mdl C \eqv C\tr$ 
%(concept and role names of $C,C\tr$ are in $\Sigma$).
%%\nb{M: Added! Is the `therefore' correct?} O:ok thanks
%
%$(\Leftarrow)$ Assume that $\chi_{f} \mdl C \eqv C\tr$. By Lemma~\ref{lemma:endchar}, 
%for every infinite trace $\Imf$, $\Imf \mdl \chi_{f}$ iff $\reduct = \FEmf$, 
%for a finite trace $\Fmf$. 
%Given our assumption, this implies $\FEmf \mdl C \eqv C\tr$, 
%that is, for all $d \in \Delta$, $d \in (C)^{\FEmc_{0}}$ iff $d \in (C\tr)^{\FEmc_{0}}$. 
%Moreover, as a consequence of Lemma~\ref{lemma:endextchar} and of~\eqref{eq:conc} in Lemma~\ref{lemma:finextchar}, for all finite traces $\Fmf$ and every $d \in \Delta$, $d \in (C)^{\Fmc_{0}}$ iff $d \in (C\tr)^{\FEmc_{0}}$. 
%In conclusion, we have that for all finite traces $\Fmf$ and all $d \in \Delta$, $d \in (C)^{\FEmc_{0}}$ if and only if $d \in (C)^{\Fmc_{0}}$, 
%meaning that $C$ is insensitive~\ref{ins:degetal}.
%
%Let $\p$ be a $\TALCf$ formula.
%$(\Rightarrow)$ Assume that $\p$ is insensitive~\ref{ins:degetal}. We want to 
%prove that, for every infinite trace $\Imf$, if $\Imf \mdl \chi_{f}$, then 
%$\Imf \mdl \p \leftrightarrow \p\tr$. Suppose $\Imf \mdl \chi_{f}$. 
%%\nb{M: Changed with $\reduct$} O: thanks
%By Lemma~\ref{lemma:endchar}, $\reduct = \FEmf$, for a finite trace $\Fmf$. 
%Moreover, thanks to Lemma~\ref{lemma:endextchar}, $\Fmf \mdl \p$ if and only if $\FEmf \mdl \p\tr$. 
%Since $\p$ is by hypothesis insensitive~\ref{ins:degetal}, for every finite 
%trace $\Fmf$, $\Fmf \mdl \p$ if and only if $\FEmf \mdl \p$. Therefore, 
%$\FEmf \mdl \p$ if and only if $\FEmf \mdl \p\tr$. Hence, $\FEmf \mdl \p \leftrightarrow \p\tr$, 
%and therefore $\Imf \mdl \p \leftrightarrow \p\tr$ (concept and role names of $\p,\p\tr$ are in $\Sigma$).
%%\nb{M: Added! Is the `therefore' correct?} O: yes thanks
%
%$(\Leftarrow)$ Assume that $\chi_{f} \mdl \p \leftrightarrow \p\tr$. By Lemma~\ref{lemma:endchar}, 
%for every infinite trace $\Imf$, $\Imf \mdl \chi_{f}$ means that $\reduct = \FEmf$, 
%for a finite trace $\Fmf$. Given our assumption, this implies $\FEmf \mdl \p \leftrightarrow \p\tr$, 
%that is $\FEmf \mdl \p$ if and only if $\FEmf \mdl \p\tr$. By Lemma~\ref{lemma:endextchar}, $\FEmf \mdl \p\tr$ 
%if and only if $\Fmf \mdl \p$. In conclusion, we obtain that $\FEmf \mdl \p$ if and only if $\Fmf \mdl \p$, 
%meaning that $\p$ is insensitive~\ref{ins:degetal}.
%%\nb{M: I am not sure if the structure of the proof is sound. \\ O: This proof is Ok. Just need some polishing}
%\end{proof}
%
%\TheorInsDegEtAlPres*
%\begin{proof}
%%\nb{M: Added! Check!} O:Thanks, I polished a bit
%We   show the statement for concepts (the proofs for formulas are analogous).
%Let $\Fmf$ be a finite trace, and $d \in \Delta^{\Fmf}$.
%For $\lnot C$, we have $d \in (\lnot C)^{\Fmc_{0}}$ iff  
%$d \not \in C^{\Fmc_{0}}$. Since $C$ is insensitive~\ref{ins:degetal} 
%by hypothesis, this means that $d \not \in C^{\FEmc_{0}}$. Therefore, 
%$\lnot C$ is insensitive~\ref{ins:degetal} as well.
%For $\exists R. C$, suppose $d \in (\exists R. C)^{\Fmc_{0}}$. 
%By the semantics of $\TALCf$, 
%there is $e \in C^{\Fmc_{0}}$ such that $(d, e) \in R^{\Fmc_{0}}$. Since $C$ is 
%  insensitive~\ref{ins:degetal}, this is equivalent to $e \in C^{\FEmc_{0}}$, 
%  and (by definition of $\FEmf$) $(d, e) \in R^{\FEmc_{0}}$. Therefore, $\exists R. C$ is 
%  insensitive~\ref{ins:degetal}.
%For $C \sqcap D$, if $d \in (C \sqcap D)^{\Fmc_{0}}$, by the semantics of $\TALCf$, $d \in C^{\Fmc_{0}}$ and 
%$d \in D^{\Fmc_{0}}$. Assuming that both $C$ and $D$ are 
%insensitive~\ref{ins:degetal}, we have $d \in C^{\FEmc_{0}}$ and $d \in D^{\FEmc_{0}}$. 
%Hence, $C \sqcap D$ is insensitive~\ref{ins:degetal}.
%\end{proof}
%
%\TheorInsUsChar*
%\begin{proof}
%Let $C$ be a $\TALCf$ concept. 
%$(\Rightarrow)$ Suppose that $C$ is insensitive~\ref{ins:us}.
%We want to show that, for every infinite trace $\Imf$, if $\Imf \mdl \psif$, then $\Imf \mdl C\tr \sqs C$. 
%If $\Imf \mdl \psif$, by Lemma~\ref{lemma:finchar}, 
%%\nb{M: Re-Changed! using $\Imf = \FImf'$} O: ok thanks!
%$\Imf = \FImf'$, for some finite trace $\Fmf$ and some infinite trace $\Imf'$. 
%As a consequence of~\eqref{eq:conc} in the proof of Lemma~\ref{lemma:finextchar} (for $C$ arbitrary $\TALCf$ concept), we have that for all finite traces $\Fmf$ and all extensions $\FImf'$, $d \in (C)^{\Fmc_{0}}$ iff $d \in (C\tr)^{\FImc'_{0}}$, for every $d \in \Delta$. 
%Since $C$ is, by hypothesis, insensitive~\ref{ins:us}, for 
%all finite traces $\Fmf$, all extensions $\FImf'$, and all $d \in \Delta$, if $d \in (C)^{\Fmc_{0}}$, then $d \in (C)^{\FImc'_{0}}$. 
%Therefore, for every $d \in \Delta$, $d \in (C\tr)^{\FImc'_{0}}$ implies $d \in (C)^{\FImc'_{0}}$, 
%that is $\FImf' \mdl C\tr \sqs C$.
%
%$(\Leftarrow)$ Assume that, for all infinite traces $\Imf$, if $\Imf \mdl \psif$, then $\Imf \mdl C\tr \sqs C$. By Lemma~\ref{lemma:finchar}, $\Imf \mdl \psif$ iff $\Imf$ is of the form $\FImf'$, for some traces $\Fmf$ and $\Imf'$.
%By assumption,
%%\nb{M: Not sure about this step}
%this implies $\FImf' \mdl  C\tr \sqs C$, that is, for every $d \in \Delta$: if $d \in (C\tr)^{\FImc'_{0}}$, then $d \in (C)^{\FImc'_{0}}$.
%Thanks to~\eqref{eq:conc} in the proof of Lemma~\ref{lemma:finextchar}, we have that for all finite traces $\Fmf$ and all extensions $\FImf'$, $d \in (C)^{\Fmc_{0}}$ iff $d \in (C\tr)^{\FImc'_{0}}$, for every $d \in \Delta$.
%In conclusion, we obtain that for all finite traces $\Fmf$, all extensions $\FImf'$, and all $d \in \Delta$, if $d \in (C)^{\Fmc_{0}}$, then $d \in (C)^{\FImc'_{0}}$, that is, $C$ is 
%insensitive~\ref{ins:us}.
%
%Let $\p$ be a $\TALCf$ formula. 
%$(\Rightarrow)$ Assume that $\p$ is insensitive~\ref{ins:us}. 
%%\nb{O: changed `infiniteness' to I2}
%We want to prove that, for every infinite trace $\Imf$, if $\Imf \mdl \psif$, then $\Imf \mdl \p\tr \to \p$. 
%If $\Imf \mdl \psif$, by Lemma~\ref{lemma:finchar}, $\Imf$ is of the form 
%$\FImf'$. By Lemma~\ref{lemma:finextchar}, we have that $\Fmf \mdl \p$ 
%iff $\FImf' \mdl \p\tr$. Since $\p$ is, by hypothesis, insensitive~\ref{ins:us}, for 
%all finite traces $\Fmf$ and all extensions $\FImf'$, if $\Fmf \mdl \p$, 
%then $\FImf' \mdl \p$. Therefore, $\FImf' \mdl \p\tr$ implies $\FImf' \mdl \p$, 
%that is $\FImf' \mdl \p\tr \to \p$.
%
%$(\Leftarrow)$ Assume that, for all infinite traces $\Imf$, if $\Imf \mdl \psif$, then $\Imf \mdl \p\tr \to \p$. By Lemma~\ref{lemma:finchar}, $\Imf \mdl \psif$ iff $\Imf$ is of the form $\FImf'$, for some traces $\Fmf$, $\Imf'$.
%By assumption,
%%\nb{M: Not sure about this step}
%this implies $\FImf' \mdl  \p\tr \to \p$, that is: if $\FImf' \mdl \p\tr$, then $\FImf' \mdl \p$.
%Moreover, by Lemma~\ref{lemma:finextchar}, $\Fmf \mdl \p$ iff $\FImf' \mdl \p\tr$.
%In conclusion, we get that if $\Fmf \mdl \p$, then $\FImf' \mdl \p$, meaning that $\p$ is 
%insensitive~\ref{ins:us}.
%\end{proof}
%
%%\LemmaIns*
%%\begin{proof}
%%	Clearly, $\Fmf, n \mdl \p$ iff $\Fmf', 0 \mdl \p$, with $\Fmf' = (\Delta^{\Fmf}, (\Fmc'_{m})_{m \in [0, l - n]})$ s.t. $\Fmc'_{m} = \Fmc_{n + m}$. Since $\p$ is insensitive to infiniteness, for every extension $\Fmf' \cdot \Imf$ of $\Fmf'$ we have $\Fmf' \cdot \Imf, 0 \mdl \p$, which in turn is equivalent to $\FImf, n \mdl \p$, for every extension $\FImf$ of $\Fmf$.
%%\end{proof}
%
%%\nb{O: added Theo 16 for completeness? \\ M: Done} Many thanks!
%
%
%\TheorInsUsPres*
%\begin{proof} 
%Firstly, we show the following claim. %\nb{O: say something for concepts? \\ M: Added! Check!} Thanks
%
%\smallskip
%
%\noindent
%\textbf{Claim.} 
%\textit{  
%Let $C$ and $\p$ be insensitive~\ref{ins:us} $\TALCf$ concept and formula, respectively, and let
%$\Fmf =(\Delta^{\Fmf}$, $
%(\Fmc_{n})_{n \in [0, l]})$ be a finite trace. Then, for every extension $\FImf$ of $\Fmf$ and every $n \in [0, l]$, we have:
%	\begin{itemize}
%		\item for all $d \in \Delta^{\Fmf}$, if $d \in C^{\Fmc_{n}}$, then $d \in C^{\FImc_{n}}$.
%		\item if $\Fmf, n \mdl \p$, then $\FImf, n \mdl \p$.
%	\end{itemize}
%	}
% 
%\smallskip
%
%\noindent
%\textit{Proof of Claim.} 
%	We consider only $\p$,   the case for $C$ is analogous. Clearly, 
%	$\Fmf, n \mdl \p$ iff $\Fmf', 0 \mdl \p$, with $\Fmf' = (\Delta^{\Fmf}, 
%	(\Fmc'_{m})_{m \in [0, l - n]})$ s.t. $\Fmc'_{m} = \Fmc_{n + m}$. 
%	Since $\p$ is insensitive~\ref{ins:us}, for every 
%	extension $\Fmf' \cdot \Imf$ of $\Fmf'$ we have $\Fmf' \cdot \Imf, 0 \mdl \p$, 
%	which in turn is equivalent to $\FImf, n \mdl \p$, for every extension 
%	$\FImf$ of $\Fmf$. This concludes the proof of the claim.
%
%\smallskip
%%Let $\Fmf$ be a finite trace, and suppose $d \in (\exists R. C)^{\Fmc_{0}}$. By definition, there is $d' \in C)^{\Fmc_{0}}$ s.t. $(d, d') \in R^{\Fmc_{0}}$. Since $C$ is assumed to be insensitive~\ref{ins:us}, we have that for every $\FImf$, $d' \in C^{\FImc_{0}}$, and (by definition of $\FImf$) $(d, d') \in R^{\FImc_{0}}$. Therefore, $\exists R. C$ is~\ref{ins:us}.
%The cases for $\exists R. C$ and $C \sqcap D$ are similar to Theorem~\ref{theor:boolins}, and the proof for $C \U D$ is analogous to $\p \U \psi$ below.
% We show the remaining cases.
%Suppose $\Fmf \mdl \p \land \psi$, that is $\Fmf \mdl \p$ and $\Fmf \mdl \psi$.
%Since both $\p$ and $\psi$ are insensitive~\ref{ins:us}, we have that for every extension 
%$\FImf$, $\FImf \mdl \p$ and $\FImf \mdl \psi$.
%Thus $\FImf \mdl \p \land \psi$, i.e., $\p \land \psi$ is insensitive~\ref{ins:us}.
%Now, assume $\Fmf \mdl \p \U \psi$, for a finite trace $\Fmf = (\Delta^\Fmf, 
%(\Fmc_n)_{n \in [0, l]})$. By definition, there is $n \in (0, l] $ such that $\Fmf, n
% \models \psi$ and $ \Fmf, m \models \p$, for all $m \in (0,n)$. Since $\p$ and 
% $\psi$ are insensitive~\ref{ins:us}, by the   Claim, for every 
% extension $\FImf$, there is $n \in (0, \infty)$ such that $\FImf, n \mdl \p$ and 
% $\FImf, m \mdl \psi$,  for all $m \in (0,n)$. Hence $ \FImf \mdl \p \U \psi$. 
% In conclusion, $\p \U \psi$ is insensitive~\ref{ins:us}.
%\end{proof}
%
%
%
%
%\TheorConcIns*
%\begin{proof}
%%\nb{M: Added! Good? O: yes thanks} 
%We prove the statement only for insensitivity~\ref{ins:us},  
% the case for~\ref{ins:degetal} is similar.  We have that $\lnot C \sqcup D$ is~\ref{ins:us} iff for every finite trace $\Fmf$, every extension $\FImf$, and every $d \in \Delta^{\Fmf}$: if $d \in (\lnot C \sqcup D)^{\Fmc_{0}}$, then $d \in (\lnot C \sqcup D)^{\FImc_{0}}$. 
%This implies that: if $(\lnot C \sqcup D)^{\Fmc_{0}}$ for all $d \in \Delta^{\Fmf}$, then $d \in (\lnot C \sqcup D)^{\FImc_{0}}$ for every $d \in \Delta^{\Fmf}$. 
%Equivalently, if $\Fmf \mdl \top \sqsubseteq \lnot C \sqcup D$, then $\FImf \mdl \top \sqsubseteq \lnot C \sqcup D$. 
%Since $\top \sqsubseteq \lnot C \sqcup D$ is equivalent to $C \sqsubseteq D$, from the previous step we have that $C \sqsubseteq D$ is insensitive~\ref{ins:us}.
%\end{proof}
%
%
%
%
%
%%%% Comparison Insensitivity \cite{DegEtAl} and New Insensitivity: Table with examples
%%
%%\begin{table}
%%\centering
%%\begin{tabular}{ >{\centering}p{5cm} | >{\centering}p{2.5cm} | >{\centering}p{2.5cm}  }
%%Formula  & \ref{ins:degetal} &~\ref{ins:us}
%%\tabularnewline
%%\hline
%%	$\alpha ::= p$ / $\alpha ::= A(a) \mid R(a,b)$ & Y & Y
%%\tabularnewline
%%	$\beta ::= C \sqs D$ \\ ($C, D ::= A \mid \lnot C \mid C \sqcap D \mid \exists R.C $) & -- & Y
%%\tabularnewline
%%	$C \sqs D$ \\ ($C, D$ arbitrary) & -- & N
%%\tabularnewline
%%	$\gamma ::= \alpha \mid \beta \mid \lnot \gamma \mid \gamma_{1} \land \gamma_{2}$ & Y & Y
%%%\tabularnewline
%%%	$\lnot \gamma$ & Y & Y
%%\tabularnewline
%%	$\lnot \p$ ($\p$ insensitive) & Y & N
%%\tabularnewline
%%	$\p \land \psi$ ($\p, \psi$ insensitive) & Y & Y
%%\tabularnewline
%%	$\p \U \psi$ ($\p, \psi$ insensitive) & N & Y
%%\tabularnewline
%%	$\Next \alpha$ & N & Y
%%\tabularnewline
%%	$\Next \lnot \alpha \equiv \lnot \Wnext \alpha$ & N & Y
%%\tabularnewline
%%	$\lnot \Next \alpha \equiv \Wnext \lnot \alpha$ & Y? & Y?
%%\tabularnewline
%%	$\Next^{n} \p$ \\ ($\p$ insensitive, $n < k$, \\ over $\TALCfk$ traces) & Y & Y
%%\tabularnewline
%%	$\Next^{n} \p$ \\ ($\p$ insensitive, $n \geq k$, \\ over $\TALCfk$ traces) & N & Y
%%\tabularnewline
%%	$\D \alpha$ & Y & Y
%%\tabularnewline
%%	$\B \alpha$ & N & N
%%\tabularnewline
%%	$\D \lnot \alpha \equiv \lnot \B \alpha \equiv \top \U \lnot \alpha$ & N & Y
%%\tabularnewline
%%	$\B \lnot \alpha \equiv \lnot \D \alpha \equiv \lnot ( \top \U \alpha)$ & Y & N
%%\tabularnewline
%%	$\D \p$ ($\p$ insensitive) & N & Y
%%\tabularnewline
%%	$\B \p$ ($\p$ insensitive) & N & N
%%\end{tabular}
%%\caption{Comparison of the two insensitivity to infiniteness notions}
%%\label{tab:inscomp}
%%
%%\end{table}
%
%%%% OLD VERSION Table Examples
%%\begin{tabular}{ >{\centering}p{5cm} | >{\centering}p{2.5cm} | >{\centering}p{2.5cm}  }
%%Formula  & \cite{DegEtAl} & Us
%%\tabularnewline
%%\hline
%%	$\alpha = p$ / $\alpha = A(a), R(a,b)$ & Y & Y
%%\tabularnewline
%%	$C \sqs D$ & -- & N (in general / when Y?)
%%\tabularnewline
%%	$\lnot \p,  \p \land \psi$ ($\p, \psi$ insensitive) & Y & Y
%%\tabularnewline
%%	$\p \U \psi$ ($\p, \psi$ insensitive) & N & Y
%%\tabularnewline
%%	$\Next^{n} \p$ ($\p$ insensitive, $n < len(\Fmf)$) & Y? & Y?
%%\tabularnewline
%%	$\Next^{n} \p$ ($\p$ insensitive, $n \geq len(\Fmf)$) & N? & N?
%%\tabularnewline
%%	$\Next \alpha$ & Y? & Y?
%%\tabularnewline
%%	$\Next \lnot \alpha \equiv \lnot \Wnext \alpha$ & N? & Y?
%%\tabularnewline
%%	$\lnot \Next \alpha \equiv \Wnext \lnot \alpha$ & ? & N?
%%\tabularnewline
%%	$\D \p$ ($\p$ insensitive) & N & Y
%%\tabularnewline
%%	$\B \p$ ($\p$ insensitive) & N & N
%%\tabularnewline
%%	$\D \alpha$ & Y & Y
%%\tabularnewline
%%	$\B \alpha$ & N & N
%%\tabularnewline
%%	$\D \lnot \alpha \equiv \lnot \B \alpha \equiv \top \U \lnot \alpha$ & N & Y
%%\tabularnewline
%%	$\B \lnot \alpha \equiv \lnot \D \alpha \equiv \lnot ( \top \U \alpha)$ & Y & N
%%\end{tabular}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Temporal Description Logics}
%\section{Proof of Theorem~\ref{th:fixed}}
%\nb{M: Change Th. nr} O:changed thanks

To prove   Theorem~\ref{th:fixed}  
we use \emph{quasimodels}~\cite{GabEtAl}, which have been used to prove the
satisfiability of various
temporal DLs.
%
Our definitions here are similar to those in Section~\ref{sec:appA}, 
 now adapted to temporal \ALC. 
%In particular, we show that there is a model with at most $k$ time
%points iff there is a quasimodel with a sequence of quasistates of
%length at most $k$.  Then, 
Our upper bound is obtained by a type 
elimination procedure. 
%guessing an
%exponential size sequence of sets of types which serves as a
%certificate for the existence of a quasimodel (and therefore a model)
%for the input formula.
 
\TheorTALCkgComplete*
\begin{proof}
We show   that satisfiability  in \TALCfk restricted to global CIs is in \ExpTime.
Let $\varphi$ be a \TALCfk formula restricted to global CIs.  Assume w.l.o.g. that $\varphi$
does not contain abbreviations (i.e., it only contains the logical
connectives $\neg$, $\sqcap$, $\wedge$, the existential quantifier
$\exists$, and the temporal operator $\Until$).  Let
$\individuals{\varphi}$ be the set of individuals occurring
in~$\varphi$.  Following the notation provided
by~\citeauthor{DBLP:conf/frocos/BaaderBKOT17}~\citeyear{DBLP:conf/frocos/BaaderBKOT17},
denote by $\clf(\varphi)$ the closure under single negation of the set
of all formulas occurring in~$\varphi$.  Similarly, we denote by
$\clc(\varphi)$ the closure under single negation of the set of all
concepts union the concepts $A_{a}, \exists R.A_{a}$, for any
$a\in\individuals{\varphi}$ and $R$ a role occurring in $\varphi$,
where $A_a$ is fresh.
%As usual, the basic elements of our quasimodels are types.
%
A \emph{concept type for $\varphi$} is any subset~$t$ of
$\clc(\varphi)\cup\individuals{\varphi}$ such that:
\begin{enumerate}[label=$\mathbf{T\arabic*}$,leftmargin=*]
  \item\label{ct:neg} $\neg C\in t$ iff $C\not\in t$, for all
    $\neg C\in\clc(\varphi)$;
  \item\label{ct:con} $C\sqcap D\in t$ iff $C,D\in t$, for all
    $C\sqcap D\in\clc(\varphi)$; and
 \item\label{ct:ind} $t$ contains at most one individual name in~$\individuals{\varphi}$.
\end{enumerate}

\noindent
Similarly, we define \emph{formula types} $t\subseteq\clf(\varphi)$ for $\varphi$ with the
  conditions:
\begin{enumerate}[label=$\mathbf{T\arabic*'}$,leftmargin=*]
  \item\label{ft:neg} $\neg\phi\in t$ iff $\phi\not\in t$, for all
    $\neg\phi\in\clf(\varphi)$; and
  \item\label{ft:fcon} $\phi\wedge\psi\in t$ iff $\phi,\psi\in t$, for all
    $\phi\wedge\psi\in\clf(\varphi)$.
\end{enumerate}
We   omit `for $\varphi$'  when there is no risk of confusion. 
A concept type describes one domain element at a single time point,
while a formula type expresses constraints on all domain elements.
%
If $a\in t\cap\individuals{\varphi}$, then $t$ describes a named element. 
We  write $t_a$ to indicate this and call it a \emph{named type}.
%

The next notion captures how sets of types need to be constrained so that 
the DL dimension   is respected. 
%
We say that a pair of concept types $(t,t')$ is \emph{$R$-compatible} if
%\begin{align*}
$\{\neg F\mid \neg \exists
R.F\in t\}\subseteq t'.$ %\nb{A: changed E to F \\O: Ok!}
%\end{align*}
A \emph{quasistate} for~$\varphi$ is a set $S$ of concept or formula types for~$\varphi$ 
such that:
\begin{enumerate}[label=\textbf{Q\arabic*},leftmargin=*]
  \item\label{q:fseg} $S$ contains exactly one formula type~$t_S$;
  \item\label{q:ind} $S$ contains exactly one named type $t_a$ for
    each $a\in\individuals{\varphi}$;
  \item\label{q:gci} for all $C\sqsubseteq D\in\clf(\varphi)$, we have
    $C\sqsubseteq D\in t_S$ iff $C\in t$ implies $D\in t$
    for all concept types $t \in S$;
  \item\label{q:cass} for all $A(a)\in\clf(\varphi)$, we have
    $A(a)\in t_S$ iff $A\in t_a$ %\nb{A: changed C to A \\ O: Ok!};
    \item \label{q:quasi}   $t \in S$ and $\exists R.D \in t$ implies there is $t' \in S$
    such that $D\in t'$ and $(t,t')$ is      $R$-compatible;
    \item \label{q:last} for all $R(a,b)\in\clf(\varphi)$, we have
      $R(a,b)\in t_S$ iff   
     $(t_a,t_b)$ is $R$-compatible. 
\end{enumerate}
 
 A \emph{(concept/formula) run segment} for~$\varphi$ is a finite sequence
$\sigma=\sigma(0)\dots\sigma(n)$ composed exclusively of concept or formula
types, respectively, such that:
\begin{enumerate}[label=\textbf{R\arabic*},leftmargin=*,series=run]
  %\item\label{enu:run1} for
  %  all $\Next \alpha \in \cls(\varphi)$ and all $i\in [0,n)$, $\Next\alpha\in\sigma(i)$ iff $\alpha\in\sigma(i+1)$;
  \item\label{enu:run2} for all $a\in\individuals{\varphi}$ and all $i\in(0,n]$,
    we have $a\in\sigma(0)$ iff $a\in\sigma(i)$;
  \item\label{enu:run3} for all $\alpha\Until\beta\in\cls(\varphi)$ and all $i\in [0,n]$, we
    have ${\alpha\Until\beta} \in\sigma(i)$ iff %(a)\nb{M: Is this a typo? O: Yes thanks}~
    there is
    $j \in (i,n]$ such that $\beta\in\sigma(j)$ and
    $\alpha\in\sigma(m)$ for all $m\in (i,j)$,
\end{enumerate}
%
where \cls is either \clc or \clf (as appropriate), and~\ref{enu:run2} does
not apply to formula run segments. 
%
Intuitively, a concept run segment describes the temporal dimension of 
  a single domain element, whereas a 
formula run segment describes   
constraints on the whole DL interpretation.
 
Finally, a \emph{quasimodel} for~$\varphi$ is a pair 
$(S,\Rmf)$, with $S$   a 
 finite sequence of  quasistates $S(0)S(1)\ldots S(n)$ and $\Rmf$  a non-empty set
of run segments such that:
\begin{enumerate}[label=\textbf{\upshape{M\arabic*}},leftmargin=*]
\item \label{m:formula} $\varphi\in t_S$ where $t_S$ is the formula type 
in $S(0)$;
  \item\label{m:runs} for every   $\sigma\in\Rmf$ and every $i\in [0,n]$,
     $\sigma(i)\in S(i)$; and, conversely, 
 for every  $t\in S(i) $, there is  
    $\sigma\in\Rmf$ with $\sigma(i)=t$.
\end{enumerate}
%
By~\ref{m:runs} and the definition of a quasistate for $\varphi$, \Rmf 
always contains exactly one formula run segment and one named run segment for
each $a\in\individuals{\varphi}$.

Every quasimodel for~$\varphi$ describes an  
interpretation satisfying~$\varphi$ and, conversely,   every such interpretation can be 
abstracted into a quasimodel for~$\varphi$. We formalise this notion for finite traces with 
the following claim. 

%\begin{restatable}{lemma}{Lemmaquasimodel}\label{lem:qm}
 
 \smallskip

\noindent
\textbf{Claim 1.} 
\textit{
  There is a finite trace satisfying $\varphi$ with at most $k$ time
  points iff there is a quasimodel for $\varphi$ with a sequence of
  quasistates of length at most $k$.
  }
  
  \smallskip
%\end{restatable}


%\begin{proof}
%We show   that satisfiability  in \TALCfkg is in \ExpTime.
  
 
Assume w.l.o.g. that  the \TALCfk formula  $\varphi$ restricted to global CIs,
 which 
is  equivalent to a formula of the form $\Tmc\wedge\B(\Tmc)\wedge\phi$ 
where $\phi$ does not contain inclusions and \Tmc is a conjunction of inclusions, 
has
\Tmc  equivalent to $\top\sqsubseteq C_\Tmc$ (and $C_\Tmc$ is of polynomial size 
w.r.t. the size of \Tmc). 
We compute in exponential time w.r.t. 
the size of $\varphi$ the set 
${\sf tp}(\varphi)$ 
of all formula types for $\phi$ 
and the set of all concept types for $\varphi$ satisfying 
the following condition (in addition to \ref{ct:neg}-\ref{ct:ind}):
\begin{enumerate}[label=\textbf{T\arabic*},leftmargin=*,start=4]
  \item\label{ct:global} $C_\Tmc\in t$. 
\end{enumerate}
There is a quasimodel for $\phi$ with all concept types satisfying this last condition  
iff there is a quasimodel for $\varphi$. We formalise this statement with the 
following straightforward claim. 
%\begin{claim}\label{lem:qm-restricted}

\smallskip

\noindent
\textbf{Claim 2.} 
\textit{ 
There is a quasimodel for $\phi$ with all concept types satisfying \ref{ct:global}
iff there is a quasimodel for $\varphi$. }
% 
%\end{claim}

\smallskip

%Denote by  ${\sf tp}(\varphi)$ the set of all such concept and formula types. 
We say that a pair $(t,t')$ of (concept/formula) types is $\U$-\emph{compatible} if: % the following holds:
%
\begin{itemize} 

  \item $\alpha \U \beta \in t$ iff either  $\beta\in t'$  
   or $\{\alpha,\alpha \U \beta\} \subseteq t'$, for all $\alpha\U\beta\in
   \cls(\varphi)$,

\end{itemize}
where \cls is either \clc or \clf (as appropriate).
%
 
Our type elimination algorithm iterates 
over the values in $[1,k-1]$ to determine in exponential time 
in $|k|$, with $k$ given in binary, the length of the sequence of quasistates 
of a quasimodel for $\varphi$, if one exists. 
For each  $l\in [1,k-1]$, the $l$-th iteration starts with sets: $$S_0,\ldots,S_{l-1},S_{l}$$ 
%for a chosen $l\in [1,k-1]$ (this choice can be implemented 
% in exponential time in $|k|$, with $k$ given in binary, 
%by simply iterating over the values in the interval)
and each $S_i$ is initially set to ${\sf
tp}(\varphi)$.  We start by exhaustively eliminating concept   types $t$ from
some $S_i$, with $i \in [0, l]$, if 
  $t$ violates one of the following
conditions:
%, where \ref{te1} is specific for concept types, 
% \ref{te5} is specific for formula types,
%and $\alpha,\beta$ are both concepts or formulas if $t$ is a concept or 
%a formula type (as appropriate):

\begin{enumerate}[label=\bf E\arabic*,leftmargin=*]
    %
  \item \label{te1} for all $\exists R.D \in t$, there is $t'\in S_i$
    such that $D\in t'$ and $(t,t')$ is $R$-compatible;
%
  \item \label{te2} if $i>0$, there is $t' \in S_{i-1}$ such that 
  $(t',t)$ is $\U$-compatible;
%
  \item \label{te3} if $i<l$, there is $t' \in S_{i+1}$ such that 
  $(t,t')$ is $\U$-compatible;
  \item \label{te4} if $i=l$ then there is no $C\U D \in t$.
    %
\end{enumerate}
%
For each $a\in\individuals{\varphi}$, if $t$ is a named type $t_a$
then, in~\ref{te2} and~\ref{te3}, we further require that the
mentioned types in a $\Until$-compatible pair contain $a$.  This phase
of the algorithm stops when no further concept types can be
eliminated.  Next, for each formula type $t$, we say that a function
$f_t$, mapping each $a\in\individuals{\varphi}$ to a named type
containing $a$, is \emph{consistent with $t$} if:
  %\begin{itemize}
  %\item    
  (i) for all  
    $A(a)\in \clf(\varphi)$, 
    $A(a)\in t$ iff $A\in f_t(a)$; and  
   % \item  
    (ii) for all $R(a,b) \in \clf(\varphi)$, 
    $R(a,b) \in t$ iff 
    $(f_t(a),f_t(b))$ is $R$-compatible. 
    We are going to use these functions to construct our quasimodel as follows.
    We first  add to each $S_i$ all $f_t$ consistent with each $t\in S_i$ 
    such that the image of $f_t$ is contained in $S_i$.
    %\end{itemize}
    We then exhaustively eliminate such functions
    $f_t$ %where formula types $t$
    from some $S_i$, with $i \in [0, l]$, if $f_t$ violates one of the
    following conditions:
  \begin{enumerate}[label=$\mathbf{E\arabic*'}$,leftmargin=*]
 %
  %~ \item \label{te11} if $i>0$, there is $f_{t'} \in S_{i-1}$ such that,  
  %~ %$f_{t'}$ consistent with $t'$ with image in $S_{i-1}$ such that, 
  %~ for all $a\in\individuals{\varphi}$, $(f_t(a),f_{t'}(a))$ is $\U$-compatible;
%
  \item \label{te22} if $i<l$, there is $f_{t'} \in S_{i+1}$ such that
    $(t,t')$ is $\U$-compatible and, for all
    $a\in\individuals{\varphi}$, $(f_t(a),f_{t'}(a))$ is
    $\U$-compatible;
    %
  \item \label{te33} if $i=l$ then there is no $\psi\U \psi' \in
    t$. %\nb{A: removed ``where $t$ is the formula type associated with $f_t$''}
%    where $t$ is the formula type associated with $f_t$.
 %
 %~ \item \label{te5} there are $t_a,t_b\in S_i$
    %~ such that, for each $R(a,b) \in t$, $(t_a,t_b)$ is $R$-compatible; 
    %~ also, $t_a$ satisfies the condition that, for all 
    %~ $A(a)\in \clf(\varphi)$, 
    %~ $A(a)\in t$ iff $C\in t_a$, and the same applies for $t_b$. 
    %
\end{enumerate}
  %~ Then, the algorithm exhaustively eliminates 
  %~ formula types $t$ from
%~ some $S_i$, $0\leq i\leq l$ if $t$ violates one of the following
%~ condition:
%~ \begin{enumerate}[label=\bf E\arabic*,leftmargin=*,start=5]
    %~ %
  
    %~ %
%~ \end{enumerate} 
  It remains to ensure   %Conditions~\ref{q:fseg} and~\ref{q:ind}, which 
% 
  that each $S_i$ contains exactly one formula type $t_{i}$ and one
  named type $t_a$ for each $a\in \individuals{\phi}$ (and no
  functions $f_t$).
%
  For this choose any formula type function $f_{t_{0}}$ in $S_0$ such
  that $\phi \in t_{0}$ (if one exists) and remove %\nb{A: added}
  formula types $t'_{0}\neq t_{0}$ from $S_0$.  Then, for each
  $i\in [1,l]$, select a formula type function $f_{t_{i}}\in S_i$ such
  that $({t_{{i-1}}},{t_{i}})$ %\nb{A: added? } Yes thanks
  is $\Until$-compatible and for all $a\in\individuals{\varphi}$,
  $(f_{t_{{i-1}}}(a),f_{t_{i}}(a))$ is $\U$-compatible, removing
  formula types $t'_{i}\neq t_{i}$ from $S_i$, where $f_{t_{i}}$ is
  the selected function.  The existence of such $f_{t_{{i}}}$
  %\nb{A:
  %  $f_{t_{{i-1}}} \to f_{t_{{i}}}$
  %  since we are going forward}
  % $f_{t_{{i-1}}}$
  is ensured by~\ref{te22}. % \ref{te11} and
%
  For each selected   function $f_{t_{i}}$ and each  $a\in\individuals{\varphi}$, with $i\in [1,l]$, 
  %there are $t_a,t_b\in S_i$ satisfying \ref{te5}.
  %Conditions~\ref{q:cass} and~\ref{q:last}, 
  we remove from $S_i$ all named types $t_a$ containing $a$ such that $t_a\neq f_{t_{i}}(a)$.  
  %and remove other $t'_a,t'_b$ from
  %$S_i$. 
  We now have that each $S_i$ contains exactly one formula type
  $t_{i}$ and one named type $t_a$ for each $a\in \individuals{\phi}$.
  Finally, we proceed removing all functions $f_t$.  We have thus
  constructed a sequence of quasistates.  Until concepts/formulas
  $\alpha\U\beta$ are satisfied thanks to the \U-compatibility
  conditions and the fact that there are no expressions of the form
  $\alpha\U\beta$ in concept/formula types in the last quasistate.
 
  This last step does not affect Conditions \ref{te1}-\ref{te4} (in
  particular~\ref{te1}) for the remaining concept types since for each
  named type there is an unnamed (concept) type which is the result of
  removing the individual name from it, and if the named type was not
  removed during type elimination then the corresponding unnamed type
  was also not removed.
  %
  If the algorithm succeeds on these steps with a surviving concept
  type $t \in S_0$ and a formula type $t_{S_0}$ in $S_0$ such that
  $\phi \in t_{S_0}$ then it returns `satisfiable'.  Otherwise, it
  increments $l$ or returns `unsatisfiable' if $l=k-1$ (i.e., there
  are no further iterations).
%\begin{restatable}{lemma}{Lemmacorrectness}

\smallskip

\noindent
\textbf{Claim 3.}  \textit{ The type elimination algorithm returns
  `satisfiable' iff there is a quasimodel for $\varphi$. }

\smallskip

\noindent
\textit{Proof of Claim 3.}  For $(\Rightarrow)$, let
$S^*=S_0^*,\ldots,S_l^*$ be the result of the type elimination
procedure.  Define $(S^*,\Rmf)$ with \Rmf as the set of sequences
$\sigma$ of (concept/formula) types such that, for all $i \in [0,l]$:
%
\begin{enumerate}%[itemindent=1em]
\item $\sigma(i) \in S^*_i$, and %\nb{A: added} 
for every $t\in S^*_i$,
  there is $\sigma\in\Rmf$ with $\sigma(i)=t$;
  \item for all $a\in\individuals{\varphi}$,
    we have $a\in\sigma(0)$ iff $a\in\sigma(i)$;
  \item for all $\alpha\Until\beta\in\cls(\varphi)$, we
    have $\alpha\Until\beta\in\sigma(i)$ iff there is
    $j \in (i,l]$ such that $\beta\in\sigma(j)$ and
    $\alpha\in\sigma(n)$ for all $n\in (i,j)$. 
\end{enumerate}
%
where \cls is either \clc or \clf (as appropriate).
%
We now argue that $(S^*,\Rmf)$ is a quasimodel for $\phi$.  We first
argue that $S^*$ is a sequence of quasistates for $\phi$.  \ref{te1}
ensures Condition~\ref{q:quasi}, while Condition~\ref{q:gci} is
satisfied since $\phi$ does not have concept inclusions.
%   (this is captured by \ref{ct:global}). 
For Conditions~\ref{q:cass} and~\ref{q:last}, we have the fact that
named types are taken from functions consistent with the formula
types.
%\ref{te5}. 
The last step of our algorithm consists in eliminating formula and
named types so that we satisfy Conditions~\ref{q:fseg}
and~\ref{q:ind}.  Thus, $S^*$ is a sequence of quasistates for $\phi$.
%
Concerning %\nb{A: paragraph changed, check!} 
the construction of $\Rmf$, Point~2 can be
enforced thanks to our selection procedure for named types, while
Point~3
 is a consequence of 
 \begin{itemize}
\item Conditions~\ref{te2}, \ref{te3} and \ref{te4}, for concept types; and
% while for formula types
%is a consequence of
\item Conditions~\ref{te22} and~\ref{te33}, for formula types, 
together with the selection procedure.
\end{itemize}
%
  Points 2 and 3 coincide with Conditions~\ref{enu:run2}
and~\ref{enu:run3}, so \Rmf is a set of run segments for $\phi$.
Finally, when the algorithm returns `satisfiable' then
Condition~\ref{m:formula} holds, while Point 1 ensures that
Condition~\ref{m:runs} holds.
%
% The algorithm only returns `satisfiable' if Condition~\ref{m:formula}
% holds.
%
% Finally, Point 1 above together with Conditions \ref{te2}, \ref{te3} 
% and \ref{te4} (and our selection procedure for named types) ensure that Condition~\ref{m:runs} holds.    
Thus, $(S^*,\Rmf)$ is a quasimodel for $\phi$.  Since 
it satisfies Condition~\ref{ct:global}, by Claim~2, there is
 a quasimodel for $\varphi$. 
  
 For the other direction $(\Leftarrow)$, assume there is a quasimodel
 for $\varphi$. By Claim~2, this implies the existence of a quasimodel
 $(S',\Rmf)$ for $\phi$ satisfying Condition~\ref{ct:global}. Assume
 $S'$ is of the form $S'_0 \ldots S'_{l-1} S'_l$, for some
 $l\in [1,k-1]$.  Let $S_0^*,\ldots,S_l^*$ be the result of the type
 elimination at the $l$-th iteration. Since $(S',\Rmf)$ is a
 quasimodel, each concept type satisfies~\ref{te1}.  Moreover,
 Conditions~\ref{te2}-\ref{te4} are consequences of the existence of
 run segments through each type (by~\ref{m:runs}).
%Since no unnamed concept type in $S_i'$ violates~\ref{te1}-\ref{te4}, 
 Then, for all unnamed (concept) types $t$, if $t\in S'_i$ then
 $t\in S_i^*$, $i \in [0,l]$.  If $t$ is a formula type or a named
 type then $t\in S'_i$ does not necessarily imply that $t\in S_i^*$,
 $i \in [0,l]$.  However, the existence of such types implies that the
 algorithm should find a sequence of functions $f_t$ satisfying
 \ref{te22} and \ref{te33} which is then used to select formula and
 named types satisfying the quasimodel conditions.  In particular, the
 selection procedure will select a function $f_{t_0}$ associated with
 a formula type $t_0\in S_0^*$ containing $\phi$.  So there is a
 surviving formula type in $S_0^*$ containing $\phi$.  If the formula
 contains individuals, then the named types in the image of the
 selected function are in $S_0^*$ and the algorithm returns
 `satisfiable'. Otherwise, since $(S',\Rmf)$ is a quasimodel, there is
 an unnamed concept type $t\in S'_0$ which is also in $ S_0^*$ by
 definition of our type elimination procedure for unnamed concept
 types.
%Observe that since   formula types do  not contain concept inclusions, 
%all conditions are checked locally, within concept types only. 
%
 
This finishes the proof of Claim~3.
%
%\qed
%\end{proof}

\smallskip

We now argue that our type elimination algorithm runs in exponential time. 
Since there are polynomially many individuals (w.r.t. the size of $\phi$) 
occurring in $\phi$, 
the number of functions $f_t$ consistent with a formula type is exponential.
As the number of (concept/formula) types is exponential 
the total number of functions and types to consider is exponential.  
%The
%maintained sets of (concept/formula) types and functions 
%have initally exponential size and 
In every
step some concept type or function is eliminated (by~\ref{te1}-\ref{te4} 
or by~\ref{te22}-\ref{te33}, respectively). Conditions~\ref{te1}-\ref{te4} 
and~\ref{te22}-\ref{te33} can
clearly be checked in exponential time. Also, the selection procedure 
of functions  for each $S_i$, which determine the formula and named types in 
the result of the algorithm,
%contains exactly one formula type 
%and 
%one named type for each individual name in $\individuals{\varphi}$ 
can also be checked in exponential time since 
we can pick any function in $S_{i+1}$  satisfying the $\Until$-compatibility relation, which is 
a local condition.  
%~ Finally,  after we decide on the formula type, 
%~ we can select named  types by first
%~ removing named  types not satisfying condition \ref{te5} and then 
%~ choosing any successor satisfying the $\Until$-compatibility relation, 
%~ for each individual name in $\individuals{\varphi}$. 
As this can also be implemented in exponential time, 
we finish our proof.
\end{proof}
 %we thus conclude:
We leave satisfiability   in \TALCf \emph{restricted to global CIs},  
analogously defined as the fragment % \TALCfg 
of \TALCf with only formulas of the form 
$\Tmc\wedge\B(\Tmc)\wedge\phi$, as an open problem. 
It is known that the complexity of the satisfiability problem 
in this fragment over infinite traces is 
\ExpTime-complete~\cite{LutEtAl,DBLP:conf/frocos/BaaderBKOT17}.
%~ \footnote{In~\cite[Theorem~3]{LutEtAl} 
%~ the authors show that satisfiability 
  %~ in  LTL$_\ALC$ 
%~ w.r.t. TBoxes with constant domains is \ExpTime-complete. 
%~ An argument  in~\cite[Theorem 1]{DBLP:conf/frocos/BaaderBKOT17} extends this result 
%~ to  \TALC formulas, which include assertions.}. 
Though, the end of time formula $\psi_{f}$ is not expressible in this fragment. %~\TALCfg. 
We cannot use the same strategy  of defining 
a translation for the semantics based on infinite traces, as we 
did in Section~`Satisfiability over Finite Traces' %~\ref{sec:tdlf-to-tdl}. 
The upper bound in~\cite{LutEtAl} 
is based on type elimination. 
The main difficulty of devising a type elimination procedure %for \TALCfg 
  is that the number of time points 
is not fixed and the argument in~\cite{LutEtAl} 
showing that there is a quasimodel iff there 
is a quasimodel $(S,\Rmf)$ such that 
 $S(i+1)\subseteq S(i)$, for all $i\geq 0$, is not applicable 
 to finite traces. A type with a concept equivalent to $\neg\Next \top$ 
 can only be in the last quasistate of the quasimodel. So it is not clear 
 whether one can show that if there is a quasimodel then there is a quasimodel 
 with an exponential sequence of quasistates, as in Theorem~\ref{th:fixed}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ijcai19"
%%% End:


==> 3.1-axioms.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Axiomatisation of the monodic fragment}
\label{sec:axioms}

%\nb{M: working here}

We axiomatise the monodic fragment of first-order temporal logic on finite traces, based on the language $\QTLfr{\Until}{}{\monodic}$.
%
Let $\monod$ be the smallest set $\Lambda$ of $\QTLfr{\Until}{}{\monodic}$ formulas that contains all the substitution instances of the following axiom schemata and is closed under the inference rules listed below.

%\noindent
%\newline
\subsubsection*{Axiom schemata \textnormal{(over $\QTLfr{\Until}{}{\monodic}$ formulas)}}
%
\begin{align}
& \text{Axiom schemata of first-order logic (FOL)}, \notag \\
%$\textbf{QL}$},
& \B (\p \to \psi) \to (\B \p \to \B \psi), \label{eq:boxK} \\
& \Wnext (\p \to \psi) \to (\Wnext \p \to \Wnext \psi), \label{eq:wnextK} \\
& \Wnext \p \leftrightarrow \B \bot \lor \Next \p, \label{eq:wnextdef} \\
& \B \p \leftrightarrow \Wnext \p \land \Wnext \B \p, \label{eq:boxdef} \\
& \B (\p \to \Wnext \p) \to \Wnext (\p \to \Box \p), \label{eq:boxwnexttrcl} \\
& \p \Until \psi \to \D \psi, \label{eq:untiltodiam} \\
& \p \Until \psi \leftrightarrow \Next \psi \lor \Next(\p \land \p \Until \psi), \label{eq:untildef} \\
& \Wnext \forall x \p \leftrightarrow \forall x \Wnext \p, \label{eq:wnextbarcan} \\
& \D^{+} \B \bot. \label{eq:endoftime}
\end{align}

%\noindent
%\newline
\subsubsection*{Inference rules \textnormal{(over $\QTLfr{\Until}{}{\monodic}$ formulas)}}
%
\begin{align}
& \text{Inference rules of FOL},\notag \\
%$\textbf{QL}$}
& \text{if $\p \in \Lambda$, then $\B \p \in \Lambda$}.\label{eq:boxNec}
\end{align}

If $\p \in \monod$, we say that $\p$ is $\monod$ \emph{derivable}, and we write $\vdash_{\monod} \p$ (or simply $\vdash \p$).
%
We have that the following formulas are derivable, and the following rule holds, in $\monod$ (cf. Appendix~\ref{sec:app_der}):
%
\begin{align}
%\label{eq:nexttownext}
%& \vdash \Next \p \to \Wnext \p, \\
\label{eq:lastequiv}
& \vdash \Box \bot \leftrightarrow \lnot \Next \top, \\ 
\label{eq:wnextand}
& \vdash \Wnext (\p \land \psi) \leftrightarrow \Wnext \p \land \Wnext \psi, \\ 
%& \vdash_{\monod} \Next (\p \lor \psi) \leftrightarrow \Next \p \lor \Next \psi \\
\label{eq:nextand}
& \vdash \Next (\p \land \psi) \leftrightarrow \Next \p \land \Next \psi, \\
%\label{eq:nextor}
%& \vdash \Next (\p \lor \psi) \leftrightarrow \Next \p \lor \Next \psi, \\
\label{eq:wnextor}
& \vdash \Wnext (\p \lor \psi) \leftrightarrow \Wnext \p \lor \Wnext \psi, \\ 
\label{eq:untiltotop}
& \vdash \p \Until \psi \rightarrow \Diamond \top, \\ 
\label{eq:wnextNec}
& \text{if $\p \in \monod$, then $\Wnext \p \in \monod$}.
\end{align}
%\nb{M: todo fix~$(\ref{eq:nextand})$}






%Given the class\nb{M: is it a set?} $\Cmc^{f}$ of all finite traces,
Finally,
%given the class $\mathbb{F}$ of all finite traces,
we define the set
%\begin{align*}
$\QLog = \{ \p \in \QTL \mid \p \text{ valid on finite traces} \}$.
%\QLog = \{ \p \in \QTL \mid & \ \Fmf, n \models^{\assign} \p, \text{ for all } \Fmf \in \mathbb{F}, \text{ all instants } n \text{ in } \Fmf,
%\\ & \text{ and all assignments } \assign \text{ in } \Fmf \}
%\end{align*}
%\begin{align*}
%\QLog = \{ \p \in \QTL \mid & \ \Fmf, n \models^{\assign} \p, \text{ for all finite traces } \Fmf, \text{ all instants } n \text{ in } \Fmf, \\
%& \text{ and all assignments } \assign \text{ in } \Fmf \}
%%& \text{ and all assignments } \assign \text{ in } \Delta^\Fmf \}
%%\QLog{\Cmc^{f}} = \{ \p \in \QTL \mid & \ \Fmf, n \models^{\assign} \p, \text{ for all } \Fmf = (\Delta^\Fmf, (\Fmc_n)_{n \in [0, l]}), \text{ with } \Fmf \in \Cmc^{f} \text{ all } n \in [0, l], \\
%%& \text{ and all assignments } \assign \text{ in } \Delta^\Fmf \}
%\end{align*}
%for every finite trace $\Fmf = (\Delta^\Fmf, (\Fmc_n)_{n \in [0, l]})$, every $n \in [0, l]$, and every assignment $\assign$, $\Fmf, n \models^{\assign} \p$.
%
%
We now prove that the axiom system introduced above is sound and complete, by adapting techniques used in~\cite[Theorem 11.71]{GabEtAl}.
%(and introduced in references therein).
%which in turn uses techniques introduced in~\cite{WolZak1}.\nb{M: todo fix ref}


%%% BEGIN THEOREM
\begin{theorem}

For every $\QTLfr{\Until}{}{\monodic}$ formula $\p$, we have:
\[
	\vdash_{\monod} \p \text{\quad iff \quad}
	\p \in \QLog
%	\QLog{\Cmc^{f}}
\]
\end{theorem}
\begin{proof}
Soundness ($\Rightarrow$)
\nb{M: todo add/check}
is straightforward.
To prove completeness ($\Leftarrow$), we show that if $\not\vdash \lnot \p$, i.e., if $\p$ is \emph{consistent with $\monod$}, then $\p$ is satisfied at some time point of a finite trace.
%
We can assume w.l.o.g.~that $\p$ is a sentence, since $\p\{x_{1}, \ldots, x_{n}\} \in \QLog$ implies $\forall x_{1} \ldots \forall x_{n} \p\{x_{1}, \ldots, x_{n}\} \in \QLog$.
%
Thus, by showing that $\vdash \forall x_{1} \ldots \forall x_{n} \p\{x_{1}, \ldots, x_{n}\}$, we also obtain that $\vdash \p\{x_{1}, \ldots, x_{n}\}$, since $\monod$ contains the
%$\textbf{QL}$  (first-order logic)
axiom schemata of FOL.
%We will use the quasimodel technique to construct such models.

For a $\QTLfr{\Until}{}{\monodic}$ sentence $\p$, let
$\sub(\p)$ and $\con(\p)$
be, respectively, the sets of all subformulas and constants in $\p$.
Moreover, we define
\nb{M: to check}
\[
\sub_{\Wnext \lnot}(\p) = \sub(\p) \cup \{ \lnot \psi \mid \psi \in \sub(\p) \} \cup
\{ \Wnext \psi \mid \psi \in \sub(\p) \} \cup \{ \Wnext \lnot \psi \mid \psi \in \sub(\p) \}, 
\]
and let 
$\sub_{n}(\p)$ be the subset of $\sub_{\Wnext \lnot}(\p)$ that contains formulas having at most $n$ free variables.
Finally, $\sub_{x}(\p) = \{ \psi\{x / y\} \mid \psi\{y\} \in \sub_{1}(\p) \}$, where $x$ is a variable not occurring in $\p$.
%
A \emph{type} for $\p$ is a Boolean saturated subset $\tp$ of $\sub_{x}(\p)$, that is:
\begin{itemize}
\item $\psi_1 \wedge \psi_2 \in t$ iff
$\psi_1 \in t$ and $\psi_2\in t$, for every 
$\psi_1\wedge \psi_2 \in {\sf sub}_x(\varphi)$; 
\item $\neg\psi \in t$ iff  $\psi\notin t$, 
for every 
$\neg \psi  \in {\sf sub}_x(\varphi)$.
\end{itemize}
%
Given a type $t$ and a constant $c \in \con(\p)$, we call the pair $(c, t)$
%called
an \emph{indexed type for $\p$} (indexed by $c$).
%denoted by $\tp^{c}$.


A pair $\Cmf = (T_{\Cmf}, T_{\Cmf}^{\con})$ is a \emph{state candidate for $\p$} if $T_{\Cmf}$ is a non-empty set of types for $\p$ such that, for all $t, t' \in T_{\Cmf}$, $t \cap \sub_{0}(\p) = t' \cap \sub_{0}(\p)$, and $T_{\Cmf}^{\con} \subseteq \con(\p) \times T_{\Cmf}$ is a set of indexed types such that, for each $c \in \con(\p)$, there exists a unique $t \in T_{\Cmf}$ with $(c, t) \in T_{\Cmf}^{\con}$.
Indexed types $(c, \tp) \in \settp^{\con}_{\stcand}$ will be denoted by $\tp^{c}_{\stcand}$.
%
Given a state candidate $\Cmf$, we define
%\nb{M: abbreviate $\bigwedge_{\psi(x)\in t} 
%\psi(x) \mapsto t$?}
$${\sf real}_\Cmf := \bigwedge_{t\in \Cmf} \exists x \bigwedge_{\psi\{x\}\in t} 
\psi\{x\}\wedge\forall x \bigvee_{t\in \Cmf}\bigwedge_{\psi\{x\}\in t}\psi\{x\}\wedge\bigwedge_{t^c_{\Cmf} \in \Cmf}\bigwedge_{\psi\{x\}\in t^c_{\Cmf}}\psi\{c/x\}.$$
%
We say that $\Cmf$ is \emph{consistent} if the sentence ${\sf real}_\Cmf$ is consistent with $\monod$.
%
In the rest of this section, with an abuse of notation, we will often refer to
$\bigwedge_{\psi\{x\}\in t} \psi\{x\}$
simply by
$\tp$.

A pair $(t_{1}, t_{2})$ of types for $\p$ is \emph{suitable} if the formula
%\[
	$t_{1} \land \Wnext t_{2}$
%	:= \bigwedge_{\psi(x) \in t_{1}} \psi(x) \land \Wnext \bigwedge_{\psi'(x) \in t_{2}} \psi'(x)
%\]
is consistent with $\monod$.
%
We observe that, if $(t_{1}, t_{2})$ is suitable, then
%both $t_{1}$ and $t_{2}$ are consistent with $\monod$.
$t_{1}$ is consistent with $\monod$.
%and either $t_{2}$ is consistent with $\monod$, or
%$\last$
%%$\B \bot$
%is (or both).
%\nb{M: remove?}
%
A pair $(\Cmf_{1}, \Cmf_{2})$ of state candidates is \emph{suitable} if the formula ${\sf real_{\Cmf_{1}}} \land \Wnext {\sf real_{\Cmf_{2}}}$ is consistent with $\monod$.
%
Again, if $(\Cmf_{1}, \Cmf_{2})$ is suitable, then $\Cmf_{1}$ is consistent.
%with $\monod$.
%%and either $\Cmf_{2}$ is consistent with $\monod$, or
%%$\last$
%%%$\B \bot$
%%is (or both).
%%\nb{M: remove?}
%

Let $\seqcand = (\Cmf_{n} = (T_{n}, T_{n}^{\con}) \mid n \in [0, l] )$, with $l \in \mathbb{N}$, be a finite sequence of state candidates for $\p$. 
%
A \emph{run} through $\mathbf{q}$ is a function $r$ assigning every $n \in [0, l]$ to a type $r(n)$ in $T_{n}$.
%
We call $r$ \emph{coherent and saturated} if the following conditions hold:
\begin{itemize}
	\item $(r(n), r(n+1))$ are suitable for $n \in [0, l)$;
	\item $r(l)$ is consistent with $\monod$;\nb{M: to check}
%	and no formulas of the form $\p \Until \psi$ are in $r(l)$;
	\item $\chi \Until \psi \in r(n)$ iff there exists $m > n$ such that $\psi \in r(m)$ and, for every $i \in (n, m)$, $\chi \in r(i)$.
\end{itemize}

A \emph{$\monod$-quasimodel} for $\p$ is a pair
$\quasimod = (\seqcand, \runs)$,
where $\seqcand = (\Cmf_{n} \mid n \in [0, l])$, with $l \in \mathbb{N}$, is a sequence of state candidates for $\p$ such that:
\begin{enumerate}
	\item $\p \in t$, for some $n \in [0, l]$ and $t \in T_{n}$;
	\item $(\Cmf_{n}, \Cmf_{n+1})$ are suitable, for all $n \in [0, l)$;
	\item $\Cmf_{l}$ is consistent;\nb{M: to check}
%	(and no $t \in T_{l}$ contains formulas of the form $\p \Until \psi$\nb{M: redundant, given Conditions 4, 5 below?});
\end{enumerate}
and $\runs$ is a set of coherent and saturated runs through $\seqcand$ satisfying the following conditions:
\begin{enumerate}
	\item[(4)] for every $c \in \con(\p)$, the function $r_{c}$ defined by $r_{c}(n) = t$, for $(c, t) \in T^{\con}_{n}$, with $n \in [0, l]$, is a run in $\runs$;
	\item[(5)] for every $n \in [0, l]$ and every $t$ in $T_{n}$, there exists a run $r$ in $\runs$ such that $r(n) = t$.
\end{enumerate}


The next lemma states that the existence of a quasimodel for a formula $\p$ implies satisfiability of $\p$ on finite traces, and it is an adaptation of~\cite[Lemma 11.72]{GabEtAl} to the case of finite traces.
%
%%% BEGIN LEMMA 1
\begin{lemma}
For a $\QTLfr{\Until}{}{\monodic}$ sentence $\p$, if there is a $\monod$-quasimodel
%$\quasimod = (\seqcand, \runs)$
for $\p$, then $\p$ is satisfiable on finite traces.
\end{lemma}
%\nb{M: todo add proof?}
%
%\begin{proof}
%%Suppose that $\quasimod = (\seqcand, \runs)$ is a $\monod$-quasimodel for $\p$, with $\seqcand = (\Cmf_{n} \mid n \in [0, l])$.
%%
%%
%\end{proof}
%%% END LEMMA 1



We now show that, for any $\QTLfr{\Until}{}{\monodic}$ sentence $\p$, being consistent with $\monod$ implies the existence of a $\monod$-quasimodel for $\p$.

%%% BEGIN LEMMA 2
\begin{lemma}
\label{lem:consquasimod}
%For every $\QTLfr{\Until}{}{\monodic}$ sentence $\p$ consistent with $\monod$, there is a $\monod$-quasimodel for $\p$.
If a $\QTLfr{\Until}{}{\monodic}$ sentence $\p$ is consistent with $\monod$, then there is a $\monod$-quasimodel for $\p$.
\end{lemma}
%
\begin{proof}

We show first the following preliminary claims.


%%% BEGIN CLAIM 1
\begin{claim}%\hfill
\label{claim:suitablepair}
The following statements hold.
\begin{itemize}

	\item[($i$)] Given a suitable pair of types $(\tp_{1}, \tp_{2})$ for $\p$, we have that:
		\begin{itemize}
%			\item for every $\Wnext \psi \in \sub_{x}\p$, $\Wnext \psi \in \tp_{1}$ implies $\last \in  \tp_{1}$ or $\psi \in \tp_{2}$;\nb{M: to fix}
			\item for every $\Next \psi \in \sub_{x}\p$, $\Next \psi \in \tp_{1}$ implies $\psi \in \tp_{2}$;
			\item for every $\chi \Until \psi \in \sub_{x}\p$, $\chi \Until \psi \in \tp_{1}$ implies $\psi \in \tp_{2}$, or $\chi \in \tp_{2}$ and $\chi \Until \psi \in \tp_{2}$.
		\end{itemize}
	\item[($ii$)] Given a suitable pair of state candidates $(\stcand_{1}, \stcand_{2})$, with $\stcand_{1} = (\settp_{1}, \setindtp_{1}), \stcand_{2} = (\settp_{2}, \setindtp_{2})$, we have that:
		\begin{itemize}
			\item for every $\tp_1 \in \settp_1$, there exists a $\tp_2 \in \settp_2$ such that $(\tp_1, \tp_2)$ is suitable;
			\item for every $\tp_2 \in \settp_2$, there exists a $\tp_1 \in \settp_1$ such that $(\tp_1, \tp_2)$ is suitable;
			\item for every $c \in \con(\p)$, the pair $(\tp^{c}_{\stcand_1}, \tp^{c}_{\stcand_2})$ is suitable.
		\end{itemize}
\end{itemize}
\end{claim}
%
\begin{proof}

$(i)$ Suppose towards a contradiction that $\Next \psi \in \tp_{1}$, but $\psi \not \in \tp_{2}$. Therefore, $\lnot \psi \in \tp_{2}$.
Since $\tp_{1} \land \Wnext \tp_{2}$ is consistent with $\monod$, by~$(\ref{eq:wnextand})$ and~$(\ref{eq:nextand})$, the formula
$\Next \psi \land \Wnext \lnot \psi$
is consistent with $\monod$.
Thus, by~$(\ref{eq:wnextdef})$, 
$\Next \psi \land (\Box \bot \lor \Next \lnot \psi)$
is consistent with $\monod$.
This implies that $\Next \psi \land \Next \lnot \psi$ is consistent with $\monod$, or $\Next \psi \land \Box \bot$ is.
In the former case, by
%~$(\ref{eq:nexttownext})$ and
definition of $\Wnext$, we have that $\Wnext \psi \land \lnot \Wnext \psi$ is consistent with $\monod$, which is impossible.
In the latter case, by FOL and~$(\ref{eq:lastequiv})$, we obtain that $\Next (\psi \land \top) \land \lnot \Next \top$ is consistent with $\monod$, and this, by~$(\ref{eq:nextand})$, implies that $\Next \top \land \lnot \Next \top$ is consistent with $\monod$, which is again impossible.

Now suppose that $\chi \Until \psi \in \tp_{1}$.
By~$(\ref{eq:untildef})$, $(\ref{eq:nextand})$ and consistency of~$\tp_{1}$, we have either $\Next \psi \in \tp_{1}$, or $\Next \chi, \Next(\chi \Until \psi) \in \tp_{1}$.
Given what we have just shown for the previous point above, this implies either $\psi \in \tp_{2}$, or $\chi, \chi \Until \psi \in \tp_{2}$.

$(ii)$ Suppose towards a contradiction that there is $\tp_{1} \in \settp_{1}$ such that none of the pairs $(\tp_{1}, \tp_{2})$, for $\tp_{2} \in \settp_{2}$ is suitable.
It follows that
\begin{align*}
& \vdash \bigwedge_{t_{2} \in \settp_{2}} \lnot (\tp_{1} \land \Wnext \tp_{2}), \\
& \vdash \bigwedge_{t_{2} \in \settp_{2}} (\tp_{1} \to \lnot \Wnext \tp_{2}), \\
& \vdash \tp_{1} \to \bigwedge_{t_{2} \in \settp_{2}} \lnot \Wnext \tp_{2}, \\
& \vdash \exists x \tp_{1} \to \exists x \bigwedge_{t_{2} \in \settp_{2}} \lnot \Wnext \tp_{2}, \\
%& \vdash \lnot (\exists x \tp_{1} \land \lnot \exists x \bigwedge_{t_{2} \in \settp_{2}} \lnot \Wnext \tp_{2}) \\
& \vdash \lnot (\exists x \tp_{1} \land \forall x \bigvee_{t_{2} \in \settp_{2}} \Wnext \tp_{2}), \\
& \vdash \lnot (\exists x \tp_{1} \land \Wnext \forall x \bigvee_{t_{2} \in \settp_{2}} \tp_{2}), \text{ by~$(\ref{eq:wnextbarcan})$ and $(\ref{eq:wnextor})$},
\end{align*}
contrary to $(\stcand_{1}, \stcand_{2})$ being suitable.

Now suppose towards a contradiction that there is $\tp_{2} \in \settp_{2}$ such that none of the pairs $(\tp_{1}, \tp_{2})$, for $\tp_{1} \in \settp_{1}$, is suitable. We have:
\begin{align*}
& \vdash \bigwedge_{t_{1} \in \settp_{1}} \lnot (\tp_{1} \land \Wnext \tp_{2}), \\
& \vdash \bigwedge_{t_{1} \in \settp_{1}} (\Wnext \tp_{2} \to \lnot \tp_{1}), \\
& \vdash \Wnext \tp_{2} \to \bigwedge_{t_{1} \in \settp_{1}} \lnot \tp_{1}, \\
& \vdash \Wnext \tp_{2} \to \lnot \bigvee_{t_{1} \in \settp_{1}}  \tp_{1}, \\
& \vdash \exists x  \Wnext \tp_{2} \to \exists x \lnot \bigvee_{t_{1} \in \settp_{1}} \tp_{1}, \\
%& \vdash \lnot (\exists x \tp_{1} \land \lnot \exists x \bigwedge_{t_{2} \in \settp_{2}} \lnot \Wnext \tp_{2}) \\
& \vdash \lnot (\exists x \Wnext \tp_{2}  \land \forall x \bigvee_{t_{1} \in \settp_{1}} \tp_{1}),
\end{align*}
contrary to $(\stcand_{1}, \stcand_{2})$ being suitable.
%\nb{M: to check}

Finally, assume that $c \in \con(\p)$. We have that $\tp^{c}_{\stcand_{1}} \land \Wnext \tp^{c}_{\stcand_{2}}$ is consistent with $\monod$, and so $(\tp^{c}_{\stcand_{1}}, \tp^{c}_{\stcand_{2}})$ is suitable.
%\nb{M: to check}

\end{proof}
%%% END CLAIM 2

A \emph{pointed state candidate} for $\p$ is a pair $\ptcand = (\stcand, \tp)$, where $\stcand = (\settp, \settp^{\con})$ is a state candidate for $\p$ and $\tp$ is a type in $\settp$.
%
We say that $\ptcand = (\stcand, \tp)$ is \emph{consistent} if the formula $\real_{\stcand} \land \tp$ is consistent with $\monod$.
%
A pair $(\ptcand_1, \ptcand_2)$ of pointed state candidates $\ptcand_1 = (\stcand_1, \tp_1), \ptcand_2 = (\stcand_2, t_2)$ for $\p$ is called \emph{suitable}, written $\ptcand_1 \prec \ptcand_2$,
\nb{M: to check/fix - use `$\preceq$'?}
if the formula $\real_{\stcand_1} \land \tp_1 \land \Wnext (\real_{\stcand_2} \land \tp_2)$ is consistent with $\monod$.
%
Given a $c \in \con (\p)$, a pair $\ptcand_1 = (\stcand_1, \tp_1), \ptcand_2 = (\stcand_2, t_2)$ of pointed state candidates for $\p$ is called \emph{suitable for $c$}, written $\ptcand_1 \prec_{c} \ptcand_2$, if $\ptcand_1 \prec \ptcand_2$, $\tp^{c}_{1} \in \settp^{\con}_{1}$ and $\tp^{c}_{2} \in \settp^{\con}_{2}$, where $\stcand_{i} = (\settp_{i}, \settp^{\con}_{i})$, $i \in \{1,2\}$.




%%% BEGIN CLAIM 2
\begin{claim}%\hfill
\label{claim:conspointstcand}

The following statements hold.

\begin{itemize}
	\item[($i$)] There is a consistent state candidate $\stcand = (\settp, \settp^{\con})$ for $\p$ such that $\p \in \tp$ for all $\tp \in \settp$.
	\item[($ii$)] For every consistent pointed state candidate $\ptcand_1 = (\stcand_1, \tp_1)$ for $\p$, there is a
	\nb{M: to check/fix - add `consistent'?}
	pointed state candidate $\ptcand_2 = (\stcand_2, \tp_2)$ such that $\ptcand_1 \prec \ptcand_2$.
	\item[($iii$)] Let $c \in \con(\p)$. For every consistent pointed state candidate for $\p$ of the form $\ptcand_1 =  (\stcand_1, \tp_1)$ and every state candidate $\stcand_2$ such that the pair $(\stcand_1, \stcand_2)$ is suitable, we have $\ptcand \prec_c \ptcand_2$ for $\ptcand_2 = (\stcand_2, \tp_2)$.
\end{itemize}

\end{claim}
%
\begin{proof}
We define the disjunction $\pi_{\p} = \bigvee_{(\stcand, \tp)}(\real_{\stcand} \land \tp)$, where $(\stcand, \tp)$ are pointed state candidate for $\p$.
%
We then substitute subformulas of $\pi_{\p}$ of the form $\Next \psi, \Wnext \psi, \Box \psi, \chi \Until \psi$ that are not in the scope of another temporal operator with unary predicate symbols or propositional variables. The resulting sentence $\overline{\pi_{\p}}$ is true in all
%(classical)
first-order structures. Since $\monod$ contains the axiom schemata and rules of
FOL,
%{\bf QL},
%classical first-order logic,
by
G\"{o}del
completeness theorem we obtain\nb{M: to check}
\begin{equation}
\label{eq:monodp}
\vdash \pi_{\p}.
\end{equation}

%\begin{itemize}

%	\item[$(i)$]
$(i)$
	Since $\p$ is consistent with $\monod$, from~$(\ref{eq:monodp})$ we obtain that $\pi_{\p} \land \p$ is consistent with $\monod$. This implies that there is a disjunct $\real_{\stcand} \land \tp$ of $\pi_{\p}$ such that $\real_{\stcand} \land \tp \land \p$ is also consistent with $\monod$, and so $\p \in \tp$ (otherwise, we would have $\p \not \in \tp$, i.e., $\lnot \p \in \tp$, and $\real_{\stcand} \land \tp \land \p$ would not be consistent).
	Since $\p$ is a sentence, and all $\tp$ in $\stcand$ agree on $\sub_{0}(\p)$, for all types $\tp'$ of $\stcand$ we have $\p \in \tp'$.
	
%	\item[$(ii)$]
	$(ii)$
	By~$(\ref{eq:wnextNec})$ and~$(\ref{eq:monodp})$, we have $\vdash \Wnext \pi_{\p}$. Hence,
	$\real_{\stcand_{1}} \land \tp_{1} \land \Wnext \pi_{\p}$ is consistent with $\monod$, that is,
	$\not \vdash \lnot (\real_{\stcand_{1}} \land \tp_{1} \land \Wnext \pi_{\p})$.
	This means
	$\not \vdash \lnot \real_{\stcand_{1}} \lor \lnot \tp_{1} \lor \lnot \Wnext \bigvee_{(\stcand, \tp)}(\real_{\stcand} \land \tp)$,
	and, by~$(\ref{eq:wnextor})$, that
	$\not \vdash \lnot \real_{\stcand_{1}} \lor \lnot \tp_{1} \lor \lnot \bigvee_{(\stcand, \tp)} \Wnext(\real_{\stcand} \land \tp)$.
	Thus, there are a state candidate $\stcand_{2} = (\settp_{2}, \setindtp_{2})$ and a type $\tp_{2} \in \settp_{2}$ such that the formula
	$\real_{\stcand_{1}} \land \tp_{1} \land \Wnext (\real_{\stcand_{2}} \land \tp_{2})$
	is consistent with $\monod$.
	\nb{M: to check/fix - show that $\stcand_{2}$ is consistent? In case $\stcand_{1}$ contains $\Box \bot$, we can take $\stcand_{2} = \stcand_{1}$}
	
%	\item[$(iii)$]
	$(iii)$
	Let $c \in \con(\p)$, $\ptcand_{1} = (\stcand_{1}, \tp^{c}_{\stcand_{1}})$, and suppose that the pair $(\stcand_{1}, \stcand_{2})$ is suitable. Now consider $\ptcand_{2} = (\stcand_2, \tp^{c}_{\stcand_{2}})$. If $\ptcand_1 \not \prec_{c} \ptcand_2$, we have:
	\begin{align}
		& \vdash \real_{\stcand_{1}} \land \tp^{c}_{\stcand_{1}} \to \lnot \Wnext (\real_{\stcand_{2}} \land \tp^{c}_{\stcand_{2}}), \text{ by definition of $\ptcand_{1} \not \prec_{c} \ptcand_{2}$}; \\
		&  \vdash \real_{\stcand_{1}} \land \tp^{c}_{\stcand_{1}}\{ c / x \} \to \lnot \Wnext (\real_{\stcand_{2}} \land \tp^{c}_{\stcand_{2}}\{ c / x \}), \text{ by FOL}; \\
%		classical first-order logic
		&  \vdash \real_{\stcand_{1}} \to \lnot \Wnext \real_{\stcand_{2}}, \text{ by definition of $\real_{\stcand_{i}}$}.
	\end{align}
This contradicts the fact that $(\stcand_{1}, \stcand_{2})$ is suitable. Thus, $\ptcand_1 \prec_{c} \ptcand_2$.
%\end{itemize}
\end{proof}
%%% END CLAIM 2


Let $(\ptcand_{0}, \ldots, \ptcand_{n})$ be a sequence of pointed state candidates
for $\p$, with
$\ptcand_{0} = (\stcand_{0}, \tp_{0})$
and $\chi \Until \psi \in \tp_{0}$.
We say that $\chi \Until \psi$ is \emph{realised} in $\tp_{0}$ (or that the sequence \emph{realises} $\chi \Until \psi$ in $\tp_{0}$) if
$\ptcand_{0} \prec \ldots \prec \ptcand_{n}$
and
there is $k \in (0, n]$, such that $\psi \in \tp_{k}$ and, for all $i \in (0, k)$, $\chi \in \tp_{i}$.
%
In this case, given $c \in \con(\p)$, if
$\ptcand_{0} \prec_{c} \ldots \prec_{c} \ptcand_{n}$,
we say that $\chi \Until \psi$ is \emph{$c$-realised} in $\tp_{0}$
(or that the sequence \emph{$c$-realises} $\chi \Until \psi$ $\tp_{0}$).

%%% BEGIN CLAIM 3
\begin{claim}
\label{claim:ptstcandseq}
Given a consistent pointed stated candidate $\ptcand_{0} = (\stcand_{0}, \tp_{0})$ and a formula $\chi \Until \psi \in \tp_{0}$, there is a sequence $(\ptcand_{0}, \ldots, \ptcand_{n})$ realising $\chi \Until \psi$ in $t_{0}$. Moreover, if $\tp_{0} = \tp^{c}_{\stcand_{0}}$, there is a sequence $(\ptcand_{0}, \ldots, \ptcand_{n})$ that $c$-realises $\chi \Until \psi$ in $t_{0}$.

\end{claim}
%
\begin{proof}

Towards a contradiction, suppose otherwise: there are a consistent pointed state candidate
$\ptcand_{0} = (\stcand_{0}, \tp_{0})$
and a formula
$\chi \Until \psi \in \tp_{0}$
such that no sequence
$(\ptcand_{0}, \ldots, \ptcand_{n})$
realises
$\chi \Until \psi$ in $t_{0}$.
%
Let $\Kmc$ be the set of all pointed state candidates $\ptcand$ such that there are $n \in \mathbb{N}$, $n \geq 1$, and pointed state candidates $\ptcand_{1}, \ldots, \ptcand_{n}$ with
\[
\ptcand_{0} \prec \ptcand_{1} \prec \ldots \prec \ptcand_{n} \quad \text{and} \quad \ptcand_{n} = \ptcand.
\]
Consider the disjunction
\[
	\vartheta = \bigvee_{(\stcand, \tp) \in \Kmc} (\real_{\stcand} \land \tp),
\]
which is not nullary since $\Kmc$ is non-empty, by Claim~$\ref{claim:conspointstcand}$.

First, we claim that
\begin{equation}
\label{eq:thetatonotpsi}
	\vdash_{\monod} \vartheta \to \lnot \psi
\end{equation}
To see this, suppose otherwise, towards a contradiction. We have that $\vartheta \land \psi$ is consistent with $\monod$, and thus
$\bigvee_{(\stcand, \tp) \in \Kmc} (\real_{\stcand} \land \tp \land \psi)$
is consistent with $\monod$ as well.
This means, in particular, that $\psi \in \tp$ (otherwise, we have that $\lnot \psi \in \tp$, and $\real_{\stcand} \land \tp \land \psi$ cannot be consistent).
Hence, we have a sequence $\ptcand_{0} \prec \ptcand_{1} \prec \ldots \prec \ptcand_{n}$ such that $n \in \mathbb{N}, n \geq 1$, $\ptcand_{i} = (\stcand_{i}, \tp_{i})$ and $\psi \in \tp_{n}$.
Since all pairs $(t_{i}, t_{i + 1}), 0 \leq i < n$, are suitable, by Claim~\ref{claim:suitablepair}, Point $(i)$, we have that the sequence $\ptcand_{0} \ldots \ptcand_{n}$ realises $\chi \Until \psi$ in $\tp_{0}$, contradicting our assumption.
Thus, $(\ref{eq:thetatonotpsi})$ holds.
%

Now, we claim that
\begin{equation}
\label{eq:thetatownexttheta}
	\vdash_{\monod} \vartheta \to \Wnext \vartheta
\end{equation}
Indeed, if this does not hold, then
$\vartheta \land \lnot \Wnext \vartheta$ is consistent with $\monod$.
Thus, there is
$\ptcand = (\stcand, \tp) \in \Kmc$
such that
$\real_{\stcand} \land \tp \land \lnot \Wnext \vartheta$ is consistent with $\monod$,
%or equivalently (given that $\Wnext \vartheta$ abbreviates $\lnot \Next \lnot \vartheta$),
%such that $\real_{\stcand} \land \tp \land \Next \lnot \vartheta$ is consistent with $\monod$.
or equivalently, by~$(\ref{eq:wnextor})$ and definition of $\vartheta$,
\nb{M: to check}
such that
$\real_{\stcand} \land \tp \land \bigwedge_{(\stcand, \tp) \in \Kmc} \lnot \Wnext  (\real_{\stcand} \land \tp)$ is consistent with $\monod$.
By Claim~\ref{claim:conspointstcand}, Point~$(ii)$, since $\ptcand$ is consistent, there is a pointed state candidate $\ptcand' = (\stcand', \tp')$ such that $\ptcand \prec \ptcand'$.
Therefore, $\ptcand' \in \Kmc$, and thus $\real_{\stcand} \land \tp \land \Wnext(\real_{\stcand'} \land \tp')$ is consistent with $\monod$.
This contradicts the consistency of
$\real_{\stcand} \land \tp \land \bigwedge_{(\stcand, \tp) \in \Kmc} \lnot \Wnext  (\real_{\stcand} \land \tp)$,
and so~$(\ref{eq:thetatownexttheta})$ holds.

From~$(\ref{eq:thetatonotpsi})$, by $(\ref{eq:boxNec})$ and $(\ref{eq:boxK})$, we obtain
\begin{equation}
\label{eq:boxthetatoboxnotpsi}
	\vdash \Box \vartheta \to \Box \lnot \psi,
\end{equation}
while from~$(\ref{eq:thetatownexttheta})$ we get:
\begin{align*}
	& \vdash \Box (\vartheta \to \Wnext \vartheta), \hfill \text{by~$(\ref{eq:boxNec})$}, \\
	& \vdash \Wnext (\vartheta \to \Box \vartheta), \hfill \text{by~$(\ref{eq:boxwnexttrcl})$}, \\
	& \vdash \Wnext \vartheta \to \Wnext \Box \vartheta, \hfill \text{by~$(\ref{eq:wnextK})$}, \\
	& \vdash \Wnext \vartheta \to \Box \vartheta, \hfill \text{by~$(\ref{eq:boxdef})$}, \\
	& \vdash \vartheta \to (\lnot \psi \land \Box \lnot \psi), \hfill \text{by~$(\ref{eq:thetatonotpsi}), (\ref{eq:thetatownexttheta})$ and $(\ref{eq:boxthetatoboxnotpsi})$}.
\end{align*}

Now take $\ptcand_{1} = (\stcand_{1}, \tp_{1})$ from $\Kmc$ such that $\ptcand_{0} \prec \ptcand_{1}$.
Since
$\real_{\stcand_{1}} \land \tp_{1}$ is a disjunct of $\vartheta$, we have
\[
	\vdash \real_{\stcand_{1}} \land \tp_{1} \to (\lnot \psi \land \Box \lnot \psi),
\]
from which, by~$(\ref{eq:wnextNec})$, $(\ref{eq:wnextK})$, $(\ref{eq:wnextand})$ and $(\ref{eq:boxdef})$, we obtain
\[
	\vdash \Wnext (\real_{\stcand_{1}} \land \tp_{1}) \to \Box \lnot \psi
\]
and therefore
\begin{equation}
\label{eq:realtoboxnotpsi}
	\vdash (\real_{\stcand_{0}} \land \tp_{0} \land \Wnext (\real_{\stcand_{1}} \land \tp_{1})) \to \Box \lnot \psi
\end{equation}
On the other hand, by $\chi \Until \psi \in \tp_{0}$ and~$(\ref{eq:untiltodiam})$, we have
\[
	\vdash (\real_{\stcand_{0}} \land \tp_{0} \land \Wnext (\real_{\stcand_{1}} \land \tp_{1})) \to \D \psi
\]
contrary to~$(\ref{eq:realtoboxnotpsi})$ and the fact that $\ptcand_{0} \prec \ptcand_{1}$.

The existence of a $c$-realising sequence, for each $c \in \con(\p)$, is proved analogously.
%\nb{M: to check}
\qedhere
\end{proof}
%%% END CLAIM 3


The following claim shows that, given a sequence of suitable pointed state candidates, there exists a finite subsequence such that the last pointed state candidate is suitable and does not contain any formula of the form $\chi \Until \psi$.

%%%% BEGIN CLAIM 4 (OLD VERSION)
\begin{claim}
\label{claim:finseq}
\nb{M: to check}
Given
%a consistent pointed state candidate
%$\ptcand_{0} = (\stcand_{0}, \tp_{0})$
%and
a sequence of pointed state candidates
$\ptcand_{0} \prec \ldots \prec \ptcand_{i} \prec \ptcand_{i + 1} \prec \ldots$,
there is a sequence
$\ptcand_{0} \prec \ldots \prec \ptcand_{n}$,
%$( (\stcand_{0}, \tp_{0}), \ldots, (\stcand_{l}, \tp_{l}) )$
with
$n \geq 1$ and 
$\ptcand_{n} = (\stcand_{n}, \tp_{n})$ consistent, such that there is no formula $\chi \Until \psi \in \tp_{n}$.
\end{claim}
%%
\begin{proof}
%
\nb{M:  to check}
Towards a contradiction, suppose otherwise:
there exist
%a consistent pointed state candidate
%$\ptcand_{0} = (\stcand_{0}, \tp_{0})$
%and
a sequence
$\ptcand_{0} \prec \ldots \prec \ptcand_{i} \prec \ptcand_{i + 1} \prec \ldots$
such that for all sequences
$\ptcand_{0} \prec \ldots \prec \ptcand_{n}$,
with $n \geq 1$ and $\ptcand_{n} = (\stcand_{n}, \tp_{n})$ consistent,
we have a formula
$\chi \Until \psi \in \tp_{n}$.
%%
%
Let $\Kmc$ be the set of all pointed state candidates $\ptcand$ such that there are $n \in \mathbb{N}$, $n \geq 1$, and pointed state candidates $\ptcand_{1}, \ldots, \ptcand_{n}$ such that
\[
\ptcand_{0} \prec \ptcand_{1} \prec \ldots \prec \ptcand_{n} \quad \text{and} \quad \ptcand_{n} = \ptcand, \ \text{with $\ptcand_{n}$ consistent},
\]
and consider the disjunction\nb{M: to check/fix - is this non-empty? cf. addition of `consistent' to Claim 12}
\[
	\vartheta = \bigvee_{(\stcand, \tp) \in \Kmc} (\real_{\stcand} \land \tp).
\]
%\nb{M: to check}
%Let the set $\Kmc$ and the formula $\vartheta$ be defined as in the proof of Claim~\ref{claim:ptstcandseq} above.
%%except that $n \geq 0$.
Since, by assumption, there are formulas of the form $\chi \Until \psi$ such that $\chi \Until \psi \in \tp_{n}$, for all $\ptcand_{n} \in \Kmc$, we have by
%$(\ref{eq:untiltodiam})$
%and
$(\ref{eq:untiltotop})$
%classical first-order logic
that
\begin{equation}
\label{eq:varthetatodiamondtop}
	\vdash_{\monod} \vartheta \to \Diamond \top,
\end{equation}
and thus, by $(\ref{eq:boxNec})$ and $(\ref{eq:boxK})$,
\begin{equation}
\label{eq:varthetatoboxdiamondtop}
	\vdash_{\monod} \Box \vartheta \to \Box \Diamond \top,
\end{equation}
Moreover, as in the proof of Claim~\ref{claim:ptstcandseq} above (by~$(\ref{eq:thetatownexttheta})$ and the fact that $\vdash_{\monod}  \Wnext \vartheta \to \Box \vartheta$), we have that
\begin{equation}
\label{eq:varthetatoboxvartheta}
	\vdash_{\monod} \vartheta \to \Box \vartheta.
\end{equation}
Therefore, from~$(\ref{eq:varthetatoboxdiamondtop})$ and~$(\ref{eq:varthetatoboxvartheta})$, we obtain 
\begin{equation}
\label{eq:varthetatoboxdiamtop}
	\vdash_{\monod} \vartheta \to \Box \Diamond \top.
\end{equation}
%
Take $\ptcand_{1} = (\stcand_{1}, \tp_{1})$ from $\Kmc$ such that $\ptcand_{0} \prec \ptcand_{1}$.
Since $\real_{\stcand_{1}} \land t_{1}$ is a disjunct of $\vartheta$,
%and since by assumption there is a formula of the form $\chi \Until \psi \in \tp_{1}$,
by
%%$(\ref{eq:untiltotop})$,
$(\ref{eq:varthetatodiamondtop})$
and
$(\ref{eq:varthetatoboxdiamtop})$
%%$(\ref{eq:untiltodiam})$
%and propositional reasoning
we have also that
%\[
%	\vdash_{\monod} \real_{\stcand_{1}} \land t_{1} \to \Diamond \top \land \Box \Diamond \top.
%\]
%By~$(\ref{eq:wnextNec})$, $(\ref{eq:wnextK})$, $(\ref{eq:wnextand})$ and $(\ref{eq:boxdef})$, we obtain
%\[
%	\vdash \Wnext (\real_{\stcand_{1}} \land \tp_{1}) \to \Box \Diamond \top
%\]
%We now claim that
%\[
%	\vdash \real_{\stcand_{0}} \land \tp_{0} \land \Wnext (\real_{\stcand_{1}} \land \tp_{1}) \to \Diamond \top.
%\]
%To see this, suppose otherwise. We have that $\real_{\stcand_{0}} \land \tp_{0} \land \Wnext (\real_{\stcand_{1}} \land \tp_{1}) \land \Box \bot$ is consistent, hence by~$(\ref{})$ also $\real_{\stcand_{0}} \land \tp_{0} \land \lnot \chi \Until \psi$ is consistent, with $\chi \Until \psi \in \tp_{1}$. However, since $\chi \Until \psi \in \tp_{1}$, we have aldo that $\vdash \real_{\stcand_{0}} \land \tp_{0} \land \Wnext (\real_{\stcand_{1}} \land \tp_{1}) \to \chi \Until \psi$
%
%\ldots
%Thus
\[
	\vdash_{\monod} \real_{\stcand_{1}} \land \tp_{1}
%	\land \Wnext (\real_{\stcand_{1}} \land \tp_{1})
	\to \Box^{+} \Diamond \top.
\]
However, this entails a contradiction, since $\ptcand_{1}$ is assumed to be consistent and, by~$(\ref{eq:endoftime})$, we have
\[
	\vdash_{\monod} \real_{\stcand_{1}} \land t_{1} \to \Diamond^{+} \Box \bot.
\]
\end{proof}
%%%% END CLAIM 4 (OLD VERSION)

%%% BEGIN CLAIM 4

%\nb{M: alternative version}
%\begin{claim}
%Given a consistent state candidate
%$\stcand_{0}$,
%there is a sequence
%$\stcand_{0}, \ldots, \stcand_{l}$
%such that:
%$(i)$ for all $i \in [0, l-1)$, the pairs $(\stcand_{i}, \stcand_{i+1})$ are suitable;
%$(ii)$ $\stcand_{l}$ is consistent;
%and
%$(iii)$ no type in $\stcand_{l}$ contains formulas of the form $\chi \Until \psi$.
%%and
%%$(iv)$ some type in $\stcand_{l}$ contains the formula $\Box \bot$.
%\end{claim}
%\begin{proof}
%%
%%Since $\ptcand_{n} = (\stcand_{n}, \tp_{n})$ is consistent, by Claim~\ref{claim:ptstcandseq},
%%there is a sequence $(\ptcand_{n}, \ldots, \ptcand_{n'})$ realising $\chi \Until \psi$ in $\tp_n$.
%%Therefore, $\ptcand_{n} \prec \ldots \prec \ptcand_{n'}$, and thus by assumption we have that there is a formula $\chi' \Until \psi' \in \tp_{n'}$.
%%We can assume that $\ptcand_{n'}$ is consistent, for otherwise, given that $( \ptcand_{n' - 1}, \ptcand_{n})$ is suitable, we have that $\ptcand_{n' - 1}$ is consistent, and thus by assumption there would be a formula $\chi' \Until \psi' \in \tp_{n' - 1}$.
%%By repeating the same reasoning, we can construct an infinite sequence of pointed state candidates \ldots
%%%Since the pairs $(\ptcand_{i}, \ptcand_{i + 1})$ are all suitable, for $i \in [0, n)$, we have in particular that $\Wnext (\real_{\stcand_n} \land \tp_n)$ is consistent with $\monod$.
%%%%and thus, by (\ldots add axioms\ldots), that
%%%%%$\Wnext \tp_n$ is consistent  with $\monod$. This implies that
%%%%%$\last$ is consistent with $\monod$, or that
%%%%$\ptcand_{n}$ is consistent with $\monod$.
%%%%%
%%%%%
%%%%%%By construction, we have that the pairs $( (\stcand_{n}, \tp_{n}), (\stcand_{n+1}, \tp_{n+1}) )$ are suitable for all $n$.
%%%%%%\ldots\nb{M: working here}
%%%%%%
%%%%%%\ldots
%%%%%%
%%%%%%Show that it follows that $\Box^{+} \Diamond \top$ is consistent with $\monod$, contradicting the fact that $\vdash \Diamond^{+} \Box \bot$, by $(\ref{eq:endoftime})$.
%
%\end{proof}


%Given a consistent pointed state candidate
%$\ptcand_{0} = (\stcand_{0}, \tp_{0})$,
%there is a sequence
%$\ptcand_{0} \prec \ldots \prec \ptcand_{n}$
%%$( (\stcand_{0}, \tp_{0}), \ldots, (\stcand_{l}, \tp_{l}) )$
%such that no type in $\stcand_{l}$ contains formulas of the form $\chi \Until \psi$.

%For every consistent pointed stated candidate $\ptcand_{0} = (\stcand_{0}, \tp_{0})$ and every formula $\chi \Until \psi \in \tp_{0}$, there is a sequence $(\ptcand_{0}, \ldots, \ptcand_{n})$ realising $\chi \Until \psi$ in $t_{0}$. Moreover, if $\tp_{0} = \tp^{c}_{\stcand_{0}}$, there is a sequence $(\ptcand_{0}, \ldots, \ptcand_{n})$ that $c$-realises $\chi \Until \psi$ in $t_{0}$.

We are now ready to complete the proof of the lemma.
%
By Claim~\ref{claim:conspointstcand}~$(i)$, there is a consistent pointed state candidate $(\stcand_{0}, \tp_{0})$ such that $\p \in \tp_{0}$. $\stcand_{0}$ will be the initial state candidate in the sequence
\[
	\seqcand = (\stcand_{i} = (\settp_{i}, \settp^{\con}_{i}) \mid i \in [0, l]), \text{ for some $l \in \mathbb{N}$,}
\]
of state candidates for the quasimodel $\quasimod = (\seqcand, \runs)$ we want to construct.

Firstly, we consider a $\tp \in \settp_{0}$ and $\chi \Until \psi \in \tp$.
%
(If no type in $\stcand_{0}$ contains formulas of the form $\chi \Until \psi$, we just take the 
%(one element)
sequence $(\stcand_{0}, \stcand_{1})$, where $\stcand_{1} = \stcand_{0}$).
We have that the pointed state candidate $(\stcand_{0}, \tp)$ is consistent.
Thus, by Claim~\ref{claim:ptstcandseq}, there is a sequence
\begin{equation}
\label{eq:firstseq}
( (\stcand_{0}, \tp), (\stcand_{0}, \tp_{1}), \ldots, (\stcand_{k}, \tp_{k}) )
\end{equation}
of pointed state candidates realising $\chi \Until \psi$ in $\tp$.

As a next step, we consider another (if any) formula $\chi' \Until \psi'$ not realised in this sequence.
By Claim~\ref{claim:suitablepair}~$(i)$, we have that $\chi', \chi' \Until \psi' \in \tp_{k}$.
Again, thanks to Claim~\ref{claim:ptstcandseq}, we can extend~$(\ref{eq:firstseq})$ to
\begin{equation}
\label{eq:secondseq}
( (\stcand_{0}, \tp), (\stcand_{0}, \tp_{1}), \ldots, (\stcand_{k}, \tp_{k}), \ldots, (\stcand_{m}, \tp_{m}) )
\end{equation}
realising $\chi'\Until\psi'$ in $\tp$.
Proceeding analogously for every formula of the form $\chi \Until \psi$ in $\tp$, we can construct another sequence that extends~$(\ref{eq:secondseq})$ and realises $\chi \Until \psi$ in $\tp$.
With a small abuse of notation, we denote such a sequence again by $(\ref{eq:secondseq})$,
%Let~$(\ref{eq:secondseq})$ be such a sequence.

Then, we consider another type $\tp' \in \settp_{0}$.
By Claim~\ref{claim:conspointstcand}~$(ii)$, there are types $\tp'_{i} \in \settp_{i}$, $i \leq m$, such that
$(\stcand_{0}, \tp') \prec (\stcand_{1}, \tp'_{1}) \prec \ldots \prec (\stcand_{m}, \tp'_{m})$.
We extend the sequence
$(\stcand_{0}, \tp'), (\stcand_{1}, \tp'_{1}), \ldots, (\stcand_{m}, \tp'_{m})$
to a sequence realising all formulas of the form $\chi \Until \psi$ in $\tp'$, as done above.
After that, we consider another type $\tp'' \in \settp_{0}$, and proceed similarly, until all types are exhausted and we have a sequence
$(\stcand_{0}, \ldots, \stcand_{n})$
of state candidates.
%


Now we consider constants.
Suppose $c \in \con(\p)$, and $\chi \Until \psi \in \tp^{c}_{\stcand_{0}}$.
By Claim~\ref{claim:conspointstcand}~$(iii)$, we have
$(\stcand_{0}, \tp^{c}_{\stcand_{0}}) \prec_{c} (\stcand_{1}, \tp^{c}_{\stcand_{1}}) \prec_{c} \ldots \prec_{c} (\stcand_{n}, \tp^{c}_{\stcand_{n}})$.
If $\chi \Until \psi$ is not $c$-realised by the sequence
\begin{equation}
\label{eq:thirdseq}
(\stcand_{0}, \tp^{c}_{\stcand_{0}}), (\stcand_{1}, \tp^{c}_{\stcand_{1}}), \ldots, (\stcand_{n}, \tp^{c}_{\stcand_{n}})
\end{equation}
in $\tp^{c}_{\stcand_{0}}$, then $\chi, \chi \Until \psi \in \tp^{c}_{\stcand_{n}}$.

By Claim~\ref{claim:ptstcandseq}, we can extend~$(\ref{eq:thirdseq})$ to
\begin{equation*}
\label{eq:fourthseq}
(\stcand_{0}, \tp^{c}_{\stcand_{0}}), (\stcand_{1}, \tp^{c}_{\stcand_{1}}), \ldots, (\stcand_{n}, \tp^{c}_{\stcand_{n}}), \ldots, (\stcand_{n'}, \tp^{c}_{\stcand_{n'}})
\end{equation*}
$c$-realising $\chi \Until \psi$ in $\tp^{c}_{\stcand_{0}}$.
Next, we take another $d \in \con(\p)$ and $\chi' \Until \psi' \in \tp^{d}_{\stcand_{0}}$ which is not $d$-realised by the sequence
\begin{equation}
\label{eq:fifthseq}
(\stcand_{0}, \tp^{d}_{\stcand_{0}}), (\stcand_{1}, \tp^{d}_{\stcand_{1}}), \ldots, (\stcand_{n}, \tp^{d}_{\stcand_{n}}), \ldots, (\stcand_{n'}, \tp^{d}_{\stcand_{n'}})
\end{equation}
We extend~$(\ref{eq:fifthseq})$ so that $\chi' \Until \psi'$ is $d$-realised by the new sequence.
After that, we consider another $e \in \con(\p)$ and $\chi'' \Until \psi'' \in \tp^{e}_{\stcand_{0}}$, and go on as before.
We proceed similarly until all constants $c \in \con(\p)$ and all $\chi \Until \psi \in \tp^{c}_{\stcand_{0}}$ are exhausted, and we have a sequence
$(\stcand_{0}, \ldots, \stcand_{p})$
of state candidates for $\p$.
Then, we consider the types and indexed types from $\stcand_{p}$ and construct a sequence
$(\stcand_{p}, \ldots, \stcand_{p'})$
as if $\stcand_{p}$ were $\stcand_{0}$.
After that, we repeat the procedure for $\stcand_{p'}$, and so on.
%

%\nb{M: working here}
\nb{M: to check/fix}
It follows from Claim~\ref{claim:finseq} that, proceeding in this way, we can obtain a finite sequence 
${\bf q} = ( \stcand_{i} \mid i \in [0, l] )$ so that $\stcand_{l}$ is consistent and no type in $\stcand_{l}$ contains formulas of the form $\p \Until \psi$.
%
%Let ${\bf q} = ( \stcand_{i} \mid i \in [0, l] )$ be the resulting finite sequence
%%(constructed in Claim~\ref{claim:finseq})
%so that no type in $\stcand_{l}$ contains formulas of the form $\p \Until \psi$.
%
By Claim~\ref{claim:suitablepair}, it can be seen that $\quasimod = (\seqcand, \runs_{\seqcand})$ is a quasimodel for $\p$, where $\runs_{\seqcand}$ is the set of all coherent and saturated runs through $\seqcand$.
%
\end{proof}
%%% END LEMMA 2
%
%
%
\end{proof}
%%% END THEOREM



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ijcai19"
%%% End:

==> macros_old.tex <==

%%% SIDE COMMENTS ENVIRONMENT

\marginparwidth=15mm
\newcommand{\nb}[1]{\textcolor{red}{$|$}\mbox{}\marginpar
%{\scriptsize\raggedright\textcolor{red}{#1}}
{\parbox{16mm}{\scriptsize\textcolor{red}{\raggedright #1}}}
}


%%% PARAGRAPH ENVIRONMENT

\newcommand{\mypar}[1]{\medskip\noindent\textbf{#1.}}


%%% USEFUL SHORTCUTS / NOTATION

\newcommand{\e}{\emph}

\newcommand{\p}{\varphi}
\newcommand{\q}{\psi}
\newcommand{\s}{\sigma}

\newcommand{\eset}{\emptyset}
\newcommand{\mdl}{\models}
\newcommand{\Int}{\ensuremath{\mathcal{I}}\xspace}

\newcommand{\sbs}{\subseteq}
\newcommand{\sqs}{\sqsubseteq}

\newcommand{\lp}{{\langle}}
\newcommand{\rp}{{\rangle}}

\newcommand{\tr}{^{\dagger}}
%\newcommand{\trx}{^{\dagger_{x}}}
%\newcommand{\try}{^{\dagger_{y}}}
\newcommand{\ttr}{^{\ddagger}}
\newcommand{\startr}{^{\star}}

\newcommand{\assign}{\ensuremath{\mathfrak{a}}\xspace}


%%% VARIA

\newcommand{\eqv}{\ensuremath{\doteq}\xspace}

\newcommand{\reduct}{\ensuremath{\Imf_{\mid_{\Sigma}}}\xspace}
\newcommand{\len}[1]{\ensuremath{{\sf len}(#1)}\xspace}

\newcommand{\ass}[2]{\ensuremath{(#1 : #2)}\xspace}

\newcommand{\last}{\ensuremath{\textit{last}}\xspace}

\newcommand{\Pre}{\ensuremath{\textit{Pre}}\xspace}
\newcommand{\Prel}[1]{\ensuremath{\Pre_{l \geq #1}}\xspace}

\newcommand{\Ext}{\ensuremath{\textit{Ext}}\xspace}

\newcommand{\satfin}[1]{\ensuremath{\textsc{sat}_{f}(#1)}\xspace}
\newcommand{\satinf}[1]{\ensuremath{\textsc{sat}_{i}(#1)}\xspace}

\newcommand{\equivfin}[2]{\ensuremath{#1 \equiv_{\Fmf} #2}\xspace}
\newcommand{\equivinf}[2]{\ensuremath{#1  \equiv_{\Imf} #2}\xspace}
%\newcommand{\equivfin}[2]{\ensuremath{\textsc{equ}_{f}(#1, #2)}\xspace}
%\newcommand{\equivinf}[2]{\ensuremath{\textsc{equ}_{i}(#1, #2)}\xspace}


\newcommand{\Isf}[1]{\ensuremath{\Imf^{#1}}\xspace}
%\newcommand{\Isf}[1]{\ensuremath{\Imf^{\mid^{#1}}}\xspace}

\newcommand{\Fsuf}[1]{\ensuremath{\Fmf^{#1}}\xspace}




%%% LOGICAL OPERATORS

\renewcommand{\U}{\ensuremath{\mathbin{\mathcal{U}}}\xspace}
\newcommand{\Until}{\ensuremath{\mathbin{\mathcal{U}}}\xspace}
\newcommand{\Since}{\ensuremath{\mathbin{\mathcal{S}}}\xspace}
\newcommand{\Wuntil}{\ensuremath{\mathbin{\mathcal{W}}}\xspace}

%\newcommand{\Next}{\ensuremath{\ocircle}}
\newcommand{\Next}{{\ensuremath{\raisebox{0.25ex}{\text{\scriptsize{$\bigcirc$}}}}}}
\newcommand{\nxt}{{\ensuremath{\raisebox{0.25ex}{\text{\scriptsize{$\bigcirc$}}}}}}
\newcommand{\Of}{\ocircle_{F}}
\newcommand{\Op}{\ocircle_{P}}
\newcommand{\Wnext}{\CIRCLE}

\newcommand{\D}{\Diamond}
\newcommand{\Df}{\D_{F}}
\newcommand{\Dp}{\Diamond_{P}}
\newcommand{\Dplus}{\ensuremath{\Diamond^{+}}\xspace}
\newcommand{\Uplus}{\ensuremath{\U^{+}}\xspace}
\newcommand{\B}{\Box}
\newcommand{\Bf}{\B_{F}}
\newcommand{\Bp}{\Box_{P}}

\newcommand{\Bast}{\boxast}

\newcommand{\monodic}{\ensuremath{\mathop{\ooalign{$\Box$ \cr \kern0.55ex \raisebox{0.2ex}{\scalebox{0.5}{$1$}}}\rule{0pt}{1.5ex} \kern-0.7ex}}\xspace}
%\newcommand{\monodic}{\ensuremath{(\textsf{m})}\xspace}


%%% LOGICS


%%% DESCRIPTION LOGICS


%%% LANGUAGES
\newcommand{\DL}{\ensuremath{\text{DL}}\xspace}
\newcommand{\DLs}{\ensuremath{\text{DLs}}\xspace}
\newcommand{\DLite}{\textsl{DL-Lite}\xspace}


\newcommand{\DLitea}{\ensuremath{\DLite_{\alpha}}}
\newcommand{\DLiteb}{\ensuremath{\DLite_\textit{bool}}}
\newcommand{\DLitek}{\ensuremath{\DLite_\textit{krom}}}
\newcommand{\DLitec}{\ensuremath{\DLite_\textit{core}}}

\newcommand{\ALC}{\ensuremath{\smash{\mathcal{ALC}}}\xspace}
\newcommand{\ALCQI}{\ensuremath{\mathcal{ALCQI}}}
\newcommand{\DLR}{\ensuremath{\mathcal{DLR}}}



%%% CONCEPTS

\newcommand{\NC}{\ensuremath{{\sf N_C}}\xspace}
\newcommand{\NI}{\ensuremath{{\sf N_I}}\xspace}
\newcommand{\NR}{\ensuremath{{\sf N_R}}\xspace}
\newcommand{\NPr}{\ensuremath{\textsf{N}_{\textsf{P}}\xspace}}


%%% QUASI-MODELS & REDUCTS

\newcommand{\nnf}{\ensuremath{\mathsf{nnf}}\xspace}
\newcommand{\cl}{\ensuremath{\mathsf{cl}}\xspace}

\newcommand{\clu}{\ensuremath{\cl^{\mathsf{u}}}\xspace}
\newcommand{\clc}{\ensuremath{\cl^{\mathsf{c}}}\xspace}
\newcommand{\clf}{\ensuremath{\cl^{\mathsf{f}}}\xspace}
\newcommand{\cls}{\ensuremath{\cl^\ast}\xspace}
\newcommand{\csub}{\ensuremath{\mathsf{csub}}\xspace}
\newcommand{\fsub}{\ensuremath{\mathsf{fsub}}\xspace}
\newcommand{\const}{\ensuremath{\ell_{\varphi}}\xspace}
\newcommand{\runSegments}[1]{\ensuremath{\mathsf{rs}(#1)}\xspace}
\newcommand{\roleConstraints}[1]{\ensuremath{\mathsf{rc}(#1)}\xspace}
\newcommand{\individuals}[1]{\NI(#1)}
\newcommand{\types}[1]{\mathsf{tp}(#1)}
\newcommand{\typesc}[1]{\mathsf{tp^{c}}(#1)}
\newcommand{\typesf}[1]{\mathsf{tp^{f}}(#1)}
\newcommand{\typescF}[1]{\mathsf{tp^{c}_{\Fmf}}(#1)}
\newcommand{\typesfF}[1]{\mathsf{tp^{f}_{\Fmf}}(#1)}
\newcommand{\quasistates}[1]{\mathsf{qs}(#1)}
\newcommand{\roles}[1]{\mathsf{rol}(#1)}
\newcommand{\rs}[1]{\ensuremath{\Rmc_{#1}}\xspace}



%%% MODAL LOGICS


%%%%%% FRAMES AND MODELS

\newcommand{\FrL}{\ensuremath{\smash{\mathsf{Fr}\mathbf{L}}}\xspace}


%%%%%% MODAL LANGUAGES

\newcommand{\ML}{\ensuremath{\smash{\mathcal{ML}}}\xspace}
\newcommand{\QML}{\ensuremath{\smash{\mathcal{QML}}}\xspace}

\newcommand{\MLALC}{\ensuremath{\smash{\ML_{\mathcal{ALC}}}}\xspace}

\newcommand{\MLALCdes}{\ensuremath{\smash{\ML^{\defdes}_{\mathcal{ALC}}}}\xspace}

\newcommand{\MLnALC}[1]{\ensuremath{\smash{\ML^{#1}_{\mathcal{ALC}}}}\xspace}




%%% MODAL SYSTEMS

\newcommand{\EALC}{\ensuremath{\smash{\mathbf{E}_{\mathcal{ALC}}}}\xspace}
\newcommand{\MALC}{\ensuremath{\smash{\mathbf{M}_{\mathcal{ALC}}}}\xspace}
\newcommand{\KALC}{\ensuremath{\smash{\mathbf{K}_{\mathcal{ALC}}}}\xspace}
\newcommand{\KtwoALC}{\ensuremath{\smash{\mathbf{K}^{2}_{\mathcal{ALC}}}}\xspace}
\newcommand{\KthreeALC}{\ensuremath{\smash{\mathbf{K}^{3}_{\mathcal{ALC}}}}\xspace}

\newcommand{\KnALC}[1]{\ensuremath{\smash{\mathbf{K}^{#1}_{\mathcal{ALC}}}}\xspace}

\newcommand{\SfiveALCQI}{\ensuremath{\textbf{S5}_{\mathcal{ALCQI}}}}


%%% TEMPORAL LOGICS

\newcommand{\LTL}{\ensuremath{\textsl{LTL}}\xspace}
\newcommand{\LTLf}{\ensuremath{\LTL^{f}}\xspace}

\newcommand{\RVLTL}{\ensuremath{\textsl{RV-LTL}}\xspace}


\newcommand{\QTL}{\ensuremath{\mathcal{QT\!L}}\xspace}

\newcommand{\QTLfr}[3]{\ensuremath{{\textsl{T}_{\Until}^{\ #1}\mathcal{QL}^{#2}_{#3}}}\xspace}
%\newcommand{\QTLfr}[3]{\ensuremath{\mathcal{\QTL}^{#1}_{#2}{#3}}\xspace}

\newcommand{\QTLn}[1]{\ensuremath{\smash{\QTL_{#1}}}\xspace}
%\newcommand{\QTLi}{{\ensuremath{\QTL^{1}}}}
%\newcommand{\QTLii}{{\ensuremath{\QTL^{2}}}}
%\newcommand{\QTLn}{{\ensuremath{\QTL^{n}}}}

\newcommand{\QTLm}{{\ensuremath{\QTL(\textsf{m})}}}
%\newcommand{\QTLiim}{{\ensuremath{\QTL^{2}(\textsf{m})}}}

\newcommand{\QTLf}{{\ensuremath{\QTL^{f}}}}
\newcommand{\QTLfn}[1]{\ensuremath{\smash{\QTL^{f}_{#1}}}\xspace}
%\newcommand{\QTLfi}{{\ensuremath{\QTL_{f}^{1}}}}
%\newcommand{\QTLfii}{{\ensuremath{\QTL_{f}^{2}}}}
%\newcommand{\QTLfn}{{\ensuremath{\QTL_{f}^{n}}}}

\newcommand{\QTLfm}{{\ensuremath{\QTLf(\textsf{m})}}}
\newcommand{\QTLfnm}{{\ensuremath{\QTLfn(\textsf{m})}}}
%\newcommand{\QTLfiim}{{\ensuremath{\QTL_{f}^{2}(\textsf{m})}}}

\newcommand{\QTLk}{{\ensuremath{\QTL^{k}}}}
\newcommand{\QTLkn}[1]{\ensuremath{\smash{\QTL^{k}_{#1}}}\xspace}



\newcommand{\TDL}{\ensuremath{\text{TDL}}\xspace}
\newcommand{\TDLs}{\ensuremath{\text{TDLs}}\xspace}
\newcommand{\TDLite}{\ensuremath{\textit{TDL-Lite}}\xspace}
\newcommand{\TDLitef}{\ensuremath{\textsl{TDL-Lite}_{\textit{f}}}\xspace}


\newcommand{\TuDLite}[2]{\ensuremath{\textsl{T}_{\Until}\DLite^{#1}_{#2}}\xspace}
\newcommand{\TfDLite}[1]{\ensuremath{\textsl{T}^{f}_{\Until}\DLite_{#1}}\xspace}
\newcommand{\TkDLite}[1]{\ensuremath{\textsl{T}^{k}_{\Until}\DLite_{#1}}\xspace}

%\newcommand{\TDLiteb}{\ensuremath{T_{\Until}\DLite_{bool}}\xspace}
%\newcommand{\TfDLiteb}{\ensuremath{T^{f}_{\Until}\DLite_{bool}}\xspace}
%\newcommand{\TkDLiteb}{\ensuremath{T^{k}_{\Until}\DLite_{bool}}\xspace}

\newcommand{\TusDLf}{\textsl{T}_{\mathcal{US}}\textit{DL}_{\textit{f}}}

\newcommand{\TALC}{\ensuremath{\smash{\textsl{T}_{\U}{\mathcal{ALC}}}}\xspace}
\newcommand{\TALCQI}{\ensuremath{\smash{\textsl{T}_{\U}{\mathcal{ALCQI}}}}}

\newcommand{\TALCf}{\ensuremath{\smash{\textsl{T}^{f}_{\U}{\mathcal{ALC}}}}\xspace}

\newcommand{\TALCk}{\ensuremath{\smash{\textsl{T}^{k}_{\U}{\mathcal{ALC}}}}\xspace}
\newcommand{\TALCfk}{\ensuremath{\smash{\textsl{T}^{k}_{\U}{\mathcal{ALC}}}}\xspace}

\newcommand{\TALCfg}{\ensuremath{\smash{\textsl{T}^{f}_{\U}(\textsf{g}){\mathcal{ALC}}}}\xspace}
\newcommand{\TALCfkg}{\ensuremath{\smash{\textsl{T}^{k}_{\U}(\textsf{g}){\mathcal{ALC}}}}\xspace}

\newcommand{\TALCfB}{\ensuremath{\smash{\textsl{T}^{f}_{\Box}{\mathcal{ALC}}}}\xspace}

\newcommand{\TuALC}[1]{\ensuremath{\smash{\textsl{T}^{#1}_{\U}{\mathcal{ALC}}}}\xspace}


%%% FINITE VS INFINITE TRACES

\newcommand{\finit}[2]{\ensuremath{\smash{\textsf{F}_{#1 #2}}}\xspace}
\newcommand{\infinit}[2]{\ensuremath{\smash{\textsf{I}_{#1 #2}}}\xspace}


%%% DEFINITE DESCRIPTIONS

\newcommand{\defdes}{\ensuremath{\smash{\textit{\riota}}}\xspace}




%%% COMPLEXITY CLASSES

\newcommand{\ACz}{{\ensuremath{\textsc{AC}^0}}}
\newcommand{\LogSpace}{\textsc{LogSpace}}
\newcommand{\NLogSpace}{\textsc{NLogSpace}}
\newcommand{\PTime}{\textsc{PTime}}
\newcommand{\NP}{\textsc{NP}}
\newcommand{\PSpace}{\textsc{PSpace}}
\newcommand{\ExpTime}{\textsc{ExpTime}}
\newcommand{\NExpTime}{\textsc{NExpTime}}
\newcommand{\ExpSpace}{\textsc{ExpSpace}}
\newcommand{\expsp}{\textsc{ExpSpace}}



%%% SANS-SERIF LETTERS

\newcommand{\Asf}{\ensuremath{\textsf{A}}\xspace}
\newcommand{\Bsf}{\ensuremath{\textsf{B}}\xspace}
\newcommand{\Csf}{\ensuremath{\textsf{C}}\xspace}
\newcommand{\Dsf}{\ensuremath{\textsf{D}}\xspace}
\newcommand{\Esf}{\ensuremath{\textsf{E}}\xspace}
\newcommand{\Fsf}{\ensuremath{\textsf{F}}\xspace}



%%% FRAKTUR LETTERS

\newcommand{\Amf}{\ensuremath{\mathfrak{A}}\xspace}
\newcommand{\Bmf}{\ensuremath{\mathfrak{B}}\xspace}
\newcommand{\Cmf}{\ensuremath{\mathfrak{C}}\xspace}
\newcommand{\Dmf}{\ensuremath{\mathfrak{D}}\xspace}
\newcommand{\Emf}{\ensuremath{\mathfrak{E}}\xspace}
\newcommand{\Fmf}{\ensuremath{\mathfrak{F}}\xspace}
\newcommand{\Gmf}{\ensuremath{\mathfrak{G}}\xspace}
\newcommand{\Hmf}{\ensuremath{\mathfrak{H}}\xspace}
\newcommand{\Imf}{\ensuremath{\mathfrak{I}}\xspace}
\newcommand{\Jmf}{\ensuremath{\mathfrak{J}}\xspace}
\newcommand{\Kmf}{\ensuremath{\mathfrak{K}}\xspace}
\newcommand{\Lmf}{\ensuremath{\mathfrak{L}}\xspace}
\newcommand{\Mmf}{\ensuremath{\mathfrak{M}}\xspace}
\newcommand{\Nmf}{\ensuremath{\mathfrak{N}}\xspace}
\newcommand{\Omf}{\ensuremath{\mathfrak{O}}\xspace}
\newcommand{\Pmf}{\ensuremath{\mathfrak{P}}\xspace}
\newcommand{\Qmf}{\ensuremath{\mathfrak{Q}}\xspace}
\newcommand{\Rmf}{\ensuremath{\mathfrak{R}}\xspace}
\newcommand{\Smf}{\ensuremath{\mathfrak{S}}\xspace}
\newcommand{\Tmf}{\ensuremath{\mathfrak{T}}\xspace}
\newcommand{\Umf}{\ensuremath{\mathfrak{U}}\xspace}
\newcommand{\Vmf}{\ensuremath{\mathfrak{V}}\xspace}
\newcommand{\Wmf}{\ensuremath{\mathfrak{W}}\xspace}
\newcommand{\Xmf}{\ensuremath{\mathfrak{X}}\xspace}
\newcommand{\Ymf}{\ensuremath{\mathfrak{Y}}\xspace}
\newcommand{\Zmf}{\ensuremath{\mathfrak{Z}}\xspace}

\newcommand{\FEmf}{\ensuremath{\Fmf \cdot_{E} \Emf}\xspace}
\newcommand{\FEmfC}{\ensuremath{\Fmf \cdot_{E} \Emf}\xspace}
\newcommand{\FImf}{\ensuremath{\Fmf \cdot \Imf}\xspace}
\newcommand{\FEImf}{\ensuremath{\Fmf \cdot_{E} \Imf}\xspace}


%%% MATHCAL LETTERS

\newcommand{\Amc}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\Bmc}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\Cmc}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\Dmc}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\Emc}{\ensuremath{\mathcal{E}}\xspace}
\newcommand{\Fmc}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\Gmc}{\ensuremath{\mathcal{G}}\xspace}
\newcommand{\Hmc}{\ensuremath{\mathcal{H}}\xspace}
\newcommand{\Imc}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\Jmc}{\ensuremath{\mathcal{J}}\xspace}
\newcommand{\Kmc}{\ensuremath{\mathcal{K}}\xspace}
\newcommand{\Lmc}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\Mmc}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\Nmc}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\Omc}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\Pmc}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\Qmc}{\ensuremath{\mathcal{Q}}\xspace}
\newcommand{\Rmc}{\ensuremath{\mathcal{R}}\xspace}
\newcommand{\Smc}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\Tmc}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\Umc}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\Vmc}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\Wmc}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\Xmc}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\Ymc}{\ensuremath{\mathcal{Y}}\xspace}
\newcommand{\Zmc}{\ensuremath{\mathcal{Z}}\xspace}

\newcommand{\FEmc}{\ensuremath{\Fmc \cdot_{E} \Emc}}
\newcommand{\FImc}{\ensuremath{\Fmc \cdot \Imc}}
\newcommand{\FEImc}{\ensuremath{\Fmc \cdot_{E} \Imc}\xspace}



%%% BLACKBOARD LETTERS 

\newcommand{\Abl}{\ensuremath{\mathbb{A}}\xspace}
\newcommand{\Bbl}{\ensuremath{\mathbb{B}}\xspace}
\newcommand{\Cbl}{\ensuremath{\mathbb{C}}\xspace}
\newcommand{\Dbl}{\ensuremath{\mathbb{D}}\xspace}
\newcommand{\Ebl}{\ensuremath{\mathbb{E}}\xspace}
\newcommand{\Fbl}{\ensuremath{\mathbb{F}}\xspace}
\newcommand{\Gbl}{\ensuremath{\mathbb{G}}\xspace}
\newcommand{\Hbl}{\ensuremath{\mathbb{H}}\xspace}
\newcommand{\Ibl}{\ensuremath{\mathbb{I}}\xspace}
\newcommand{\Jbl}{\ensuremath{\mathbb{J}}\xspace}
\newcommand{\Kbl}{\ensuremath{\mathbb{K}}\xspace}
\newcommand{\Lbl}{\ensuremath{\mathbb{L}}\xspace}
\newcommand{\Mbl}{\ensuremath{\mathbb{M}}\xspace}
\newcommand{\Nbl}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\Obl}{\ensuremath{\mathbb{O}}\xspace}
\newcommand{\Pbl}{\ensuremath{\mathbb{P}}\xspace}
\newcommand{\Qbl}{\ensuremath{\mathbb{Q}}\xspace}
\newcommand{\Rbl}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\Sbl}{\ensuremath{\mathbb{S}}\xspace}
\newcommand{\Tbl}{\ensuremath{\mathbb{T}}\xspace}
\newcommand{\Ubl}{\ensuremath{\mathbb{U}}\xspace}
\newcommand{\Vbl}{\ensuremath{\mathbb{V}}\xspace}
\newcommand{\Wbl}{\ensuremath{\mathbb{W}}\xspace}
\newcommand{\Xbl}{\ensuremath{\mathbb{X}}\xspace}
\newcommand{\Ybl}{\ensuremath{\mathbb{Y}}\xspace}
\newcommand{\Zbl}{\ensuremath{\mathbb{Z}}\xspace}



%%% BOLDFACE LETTERS

\newcommand{\Abf}{\ensuremath{\mathbf{A}}\xspace}
\newcommand{\Bbf}{\ensuremath{\mathbf{B}}\xspace}
\newcommand{\Cbf}{\ensuremath{\mathbf{C}}\xspace}
\newcommand{\Dbf}{\ensuremath{\mathbf{D}}\xspace}
\newcommand{\Ebf}{\ensuremath{\mathbf{E}}\xspace}
\newcommand{\Fbf}{\ensuremath{\mathbf{F}}\xspace}
\newcommand{\Gbf}{\ensuremath{\mathbf{G}}\xspace}
\newcommand{\Hbf}{\ensuremath{\mathbf{H}}\xspace}
\newcommand{\Ibf}{\ensuremath{\mathbf{I}}\xspace}
\newcommand{\Jbf}{\ensuremath{\mathbf{J}}\xspace}
\newcommand{\Kbf}{\ensuremath{\mathbf{K}}\xspace}
\newcommand{\Lbf}{\ensuremath{\mathbf{L}}\xspace}
\newcommand{\Mbf}{\ensuremath{\mathbf{M}}\xspace}
\newcommand{\Nbf}{\ensuremath{\mathbf{N}}\xspace}
\newcommand{\Obf}{\ensuremath{\mathbf{O}}\xspace}
\newcommand{\Pbf}{\ensuremath{\mathbf{P}}\xspace}
\newcommand{\Qbf}{\ensuremath{\mathbf{Q}}\xspace}
\newcommand{\Rbf}{\ensuremath{\mathbf{R}}\xspace}
\newcommand{\Sbf}{\ensuremath{\mathbf{S}}\xspace}
\newcommand{\Tbf}{\ensuremath{\mathbf{T}}\xspace}
\newcommand{\Ubf}{\ensuremath{\mathbf{U}}\xspace}
\newcommand{\Vbf}{\ensuremath{\mathbf{V}}\xspace}
\newcommand{\Wbf}{\ensuremath{\mathbf{W}}\xspace}
\newcommand{\Xbf}{\ensuremath{\mathbf{X}}\xspace}
\newcommand{\Ybf}{\ensuremath{\mathbf{Y}}\xspace}
\newcommand{\Zbf}{\ensuremath{\mathbf{Z}}\xspace}

\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}} 
\newcommand{\Nbb}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\Zbb}{\ensuremath{\mathbb{Z}}\xspace}

%%% USELESS

\newcommand{\A}{\ensuremath{\mathcal{A}}}
\newcommand{\K}{\ensuremath{\mathcal{K}}}
\newcommand{\I}{\ensuremath{\mathcal{I}}}
\newcommand{\T}{\ensuremath{\mathcal{T}}}
%
%\newcommand{\QT}{Q_\T}
%\newcommand{\QA}{Q_\A}
%
%\newcommand{\TuDLbn}{\ensuremath{\smash{\textsl{T}_{\mathcal{US}}\DLbn}}}%
%\newcommand{\TuDLcn}{\ensuremath{\smash{\textsl{T}_{\mathcal{US}}\DLcn}}}%
%
%\newcommand{\TdDLan}{\ensuremath{\smash{\textsl{T}_{F\!P}\DLan}}}%
%\newcommand{\TdDLbn}{\ensuremath{\smash{\textsl{T}_{F\!P}\DLbn}}}%
%\newcommand{\TdDLkn}{\ensuremath{\smash{\textsl{T}_{F\!P}\DLkn}}}%
%\newcommand{\TdDLcn}{\ensuremath{\smash{\textsl{T}_{F\!P}\DLcn}}}%
%
%\newcommand{\TdDLaHN}{\ensuremath{\smash{\textsl{T}_{\U\!\S}\rDLaHN}}}%
%\newcommand{\TdDLbHN}{\ensuremath{\smash{\textsl{T}_{\U\!\S}\rDLbHN}}}%
%\newcommand{\TdDLkHN}{\ensuremath{\smash{\textsl{T}_{\U\!\S}\rDLkHN}}}%
%\newcommand{\TdDLcHN}{\ensuremath{\smash{\textsl{T}_{\U\!\S}\rDLcHN}}}%
%
%\newcommand{\TdxDLan}{\ensuremath{\smash{\textsl{T}_{F\!P\!X}\DLan}}}
%\newcommand{\TdxDLbn}{\ensuremath{\smash{\textsl{T}_{F\!P\!X}\DLbn}}}%
%\newcommand{\TdxDLkn}{\ensuremath{\smash{\textsl{T}_{F\!P\!X}\DLkn}}}%
%\newcommand{\TdxDLcn}{\ensuremath{\smash{\textsl{T}_{F\!P\!X}\DLcn}}}%
%
%\newcommand{\zSVDLan}{\ensuremath{\smash{\textsl{T}_{U}\DLan}}}%
%\newcommand{\zSVDLb}{\ensuremath{\smash{\textsl{T}_{U}\DLbn}}}%
%\newcommand{\zSVDLk}{\ensuremath{\smash{\textsl{T}_{U}\DLkn}}}%
%\newcommand{\zSVDLc}{\ensuremath{\smash{\textsl{T}_{U}\DLcn}}}%
%
%\newcommand{\TxDLbn}{\ensuremath{\smash{\textsl{T}^{\,\ast}_{X}\DLbn}}}%
%\newcommand{\TdrDLbn}{\ensuremath{\smash{\textsl{T}^{\,\ast}_{F\!P}\DLbn}}}%
%\newcommand{\TurDLbn}{\ensuremath{\smash{\textsl{T}^{\,\ast}_{U}\DLbn}}}%
%
%\newcommand{\TdxrDLcn}{\ensuremath{\smash{\textsl{T}^{\,\ast}_{F\!P\!X}\DLcn}}}%
%\newcommand{\TdxrDLkn}{\ensuremath{\smash{\textsl{T}^{\,\ast}_{F\!P\!X}\DLkn}}}%


